LibraGrad: Balancing Gradient Flow for Universally Better Vision Transformer Attributions

Why do gradient-based explanations struggle with Transformers, and how can we improve them? We identify gradient flow imbalances in Transformers that violate FullGrad-completeness, a critical property for attribution faithfulness that CNNs naturally possess. To address this issue, we introduce LibraGrad -- a theoretically grounded post-hoc approach that corrects gradient imbalances through pruning and scaling of backward paths, without changing the forward pass or adding computational overhead. We evaluate LibraGrad using three metric families: Faithfulness, which quantifies prediction changes under perturbations of the most and least relevant features; Completeness Error, which measures attribution conservation relative to model outputs; and Segmentation AP, which assesses alignment with human perception. Extensive experiments across 8 architectures, 4 model sizes, and 4 datasets show that LibraGrad universally enhances gradient-based methods, outperforming existing white-box methods -- including Transformer-specific approaches -- across all metrics. We demonstrate superior qualitative results through two complementary evaluations: precise text-prompted region highlighting on CLIP models and accurate class discrimination between co-occurring animals on ImageNet-finetuned models -- two settings on which existing methods often struggle. LibraGrad is effective even on the attention-free MLP-Mixer architecture, indicating potential for extension to other modern architectures. Our code is freely available at https://github.com/NightMachinery/LibraGrad.

==> files/ds2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
% Method & ImageNet & ImageNet-Hard & MURA & Oxford-IIIT Pet & Avg. \\
Method & \makecell{ImageNet} & \makecell{ImageNet-\\Hard} & MURA & \makecell{Oxford-\\IIIT Pet} & \textit{Avg.} \\
\cmidrule(r){1-1}
% \cmidrule(lr){2-5}
\cmidrule(r){2-5}
% \cmidrule(l){6-6}
\cmidrule{6-6}
Random & 26.5 & 52.4 & 15.1 & 13.7 & 26.9 \\
RawAtt & 44.6 & 65.9 & 24.8 & 37.2 & 43.1 \\
Attn. Rollout & 35.4 & 62.2 & 21.5 & 21.2 & 35.1 \\
AliLRP & 33.3 & 64.1 & 19.2 & 19.0 & 33.9 \\
AttnLRP & 38.5 & 70.8 & 22.8 & 30.3 & 40.6 \\
DecompX & 37.8 & 67.7 & 21.6 & 22.5 & 37.4 \\
Int. Gradients & 35.4 & 66.6 & 23.8 & 20.7 & 36.6 \\
\midrule
\IxG{}  & 34.4 & 67.6 & 25.5 & 20.4 & 37.0 \\
% \textbf{Libra \IxG{} }
\textbf{\dittoLibra{}}
& 38.6 & 68.8 & 21.6 & 23.5 & 38.1 \\
\midrule
AttCAT & 46.9 & 82.3 & 31.1 & 37.3 & 49.4 \\
% \textbf{Libra AttCAT}
\textbf{\dittoLibra{}}
& \underline{63.5} & \underline{87.3} & \underline{40.9} & \underline{55.3} & \underline{61.8} \\
\midrule
GenAtt & 58.2 & 81.3 & 30.0 & 44.1 & 53.4 \\
% \textbf{Libra GenAtt}
\textbf{\dittoLibra{}}
& 61.6 & 82.8 & 30.1 & 46.5 & 55.2 \\
\midrule
TokenTM & 56.8 & 79.3 & 28.0 & 44.0 & 52.0 \\
% \textbf{Libra TokenTM}
\textbf{\dittoLibra{}}
& 59.1 & 80.0 & 28.0 & 45.4 & 53.1 \\
\midrule
GradCAM+ & 45.6 & 75.8 & 24.0 & 32.6 & 44.5 \\
% \textbf{Libra GradCAM+}
\textbf{\dittoLibra{}}
& 61.4 & 83.4 & 34.7 & 47.8 & 56.8 \\
\midrule
HiResCAM & 45.4 & 74.2 & 22.2 & 18.0 & 39.9 \\
% \textbf{Libra HiResCAM}
\textbf{\dittoLibra{}}
& 56.7 & 79.7 & 30.1 & 39.4 & 51.5 \\
\midrule
XGradCAM+ & 38.6 & 72.1 & 23.7 & 33.2 & 41.9 \\
% \textbf{Libra XGradCAM+}
\textbf{\dittoLibra{}}
& \textbf{63.9} & 84.7 & 36.6 & 52.6 & 59.4 \\
\midrule
FullGrad+ & 44.2 & 80.1 & 32.8 & 35.3 & 48.1 \\
% \textbf{Libra FullGrad+}
\textbf{\dittoLibra{}}
& 63.1 & \textbf{87.6} & \textbf{43.2} & \textbf{57.3} & \textbf{62.8} \\
\bottomrule
\end{tabular}
\caption{Cross-dataset analysis of Most-Influential-First Deletion (MIF) Accuracy evaluated using predicted labels on ViT-B. All standard deviations were bounded by 0.1 (omitted for brevity).}
\label{across_models_ds2_MIF_1p_accuracy_m_2}
\end{table}


==> files/tables_v1/across_models/depth/LIF_1p_AOPC/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ViT-Tiny & ViT-Small & ViT-Base & ViT-Large & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 79.0 \textcolor{gray}{±0.2} & 81.8 \textcolor{gray}{±0.2} & 85.8 \textcolor{gray}{±0.2} & 83.7 \textcolor{gray}{±0.2} & 82.6 \textcolor{gray}{±0.2} \\
RawAtt & 85.6 \textcolor{gray}{±0.2} & 87.2 \textcolor{gray}{±0.2} & 87.6 \textcolor{gray}{±0.1} & 81.5 \textcolor{gray}{±0.1} & 85.5 \textcolor{gray}{±0.2} \\
Attention Rollout & 84.3 \textcolor{gray}{±0.2} & 82.4 \textcolor{gray}{±0.3} & 86.0 \textcolor{gray}{±0.2} & 81.9 \textcolor{gray}{±0.2} & 83.7 \textcolor{gray}{±0.2} \\
AliLRP & 92.6 \textcolor{gray}{±0.2} & 85.8 \textcolor{gray}{±0.2} & 89.3 \textcolor{gray}{±0.2} & 85.9 \textcolor{gray}{±0.2} & 88.4 \textcolor{gray}{±0.2} \\
AttnLRP & 93.2 \textcolor{gray}{±0.2} & 92.8 \textcolor{gray}{±0.2} & 90.8 \textcolor{gray}{±0.1} & 91.3 \textcolor{gray}{±0.2} & 92.1 \textcolor{gray}{±0.2} \\
DecompX & 93.1 \textcolor{gray}{±0.2} & 90.3 \textcolor{gray}{±0.2} & 90.6 \textcolor{gray}{±0.1} & 89.3 \textcolor{gray}{±0.2} & 90.8 \textcolor{gray}{±0.2} \\
Integrated Gradients & 88.8 \textcolor{gray}{±0.2} & 90.1 \textcolor{gray}{±0.2} & 91.3 \textcolor{gray}{±0.1} & 88.4 \textcolor{gray}{±0.2} & 89.6 \textcolor{gray}{±0.2} \\
\midrule
\IxG{}  & 88.3 \textcolor{gray}{±0.2} & 87.8 \textcolor{gray}{±0.3} & 90.2 \textcolor{gray}{±0.1} & 86.7 \textcolor{gray}{±0.1} & 88.2 \textcolor{gray}{±0.2} \\
\textbf{Libra \IxG{} } & 93.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+6.3\%}) & 89.6 \textcolor{gray}{±0.2} (\textcolor{blue}{+2.1\%}) & 91.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.2\%}) & 90.2 \textcolor{gray}{±0.2} (\textcolor{blue}{+4.0\%}) & 91.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+3.4\%}) \\
\midrule
AttCAT & 95.3 \textcolor{gray}{±0.2} & 95.6 \textcolor{gray}{±0.2} & 96.6 \textcolor{gray}{±0.2} & 92.6 \textcolor{gray}{±0.2} & 95.0 \textcolor{gray}{±0.2} \\
\textbf{Libra AttCAT} & \underline{98.1} \textcolor{gray}{±0.2} (\textcolor{blue}{+2.9\%}) & \underline{97.8} \textcolor{gray}{±0.2} (\textcolor{blue}{+2.3\%}) & \underline{99.2} \textcolor{gray}{±0.1} (\textcolor{blue}{+2.7\%}) & \underline{97.1} \textcolor{gray}{±0.2} (\textcolor{blue}{+4.8\%}) & \underline{98.0} \textcolor{gray}{±0.2} (\textcolor{blue}{+3.2\%}) \\
\midrule
GenAtt & 93.5 \textcolor{gray}{±0.2} & 92.9 \textcolor{gray}{±0.2} & 94.6 \textcolor{gray}{±0.1} & 91.5 \textcolor{gray}{±0.2} & 93.1 \textcolor{gray}{±0.2} \\
\textbf{Libra GenAtt} & 92.2 \textcolor{gray}{±0.2} (\textcolor{coral}{-1.4\%}) & 92.7 \textcolor{gray}{±0.2} (\textcolor{coral}{-0.2\%}) & 94.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.2\%}) & 92.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.5\%}) & 92.9 \textcolor{gray}{±0.2} (\textcolor{coral}{-0.2\%}) \\
\midrule
TokenTM & 91.3 \textcolor{gray}{±0.2} & 90.8 \textcolor{gray}{±0.2} & 93.3 \textcolor{gray}{±0.1} & 90.3 \textcolor{gray}{±0.2} & 91.4 \textcolor{gray}{±0.2} \\
\textbf{Libra TokenTM} & 90.5 \textcolor{gray}{±0.2} (\textcolor{coral}{-0.9\%}) & 90.8 \textcolor{gray}{±0.2} (+0.0\%) & 93.5 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.2\%}) & 90.8 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.6\%}) & 91.4 \textcolor{gray}{±0.2} (+0.0\%) \\
\midrule
GradCAM+ & 84.3 \textcolor{gray}{±0.2} & 88.1 \textcolor{gray}{±0.2} & 91.5 \textcolor{gray}{±0.2} & 91.0 \textcolor{gray}{±0.2} & 88.7 \textcolor{gray}{±0.2} \\
\textbf{Libra GradCAM+} & 89.6 \textcolor{gray}{±0.2} (\textcolor{blue}{+6.2\%}) & 93.7 \textcolor{gray}{±0.2} (\textcolor{blue}{+6.4\%}) & 96.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.2\%}) & 92.7 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.8\%}) & 93.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+4.9\%}) \\
\midrule
HiResCAM & 71.3 \textcolor{gray}{±0.2} & 78.7 \textcolor{gray}{±0.3} & 91.7 \textcolor{gray}{±0.2} & 74.2 \textcolor{gray}{±0.3} & 79.0 \textcolor{gray}{±0.2} \\
\textbf{Libra HiResCAM} & 86.2 \textcolor{gray}{±0.2} (\textcolor{blue}{+20.8\%}) & 91.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+15.7\%}) & 94.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.8\%}) & 88.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+18.6\%}) & 89.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+13.8\%}) \\
\midrule
XGradCAM+ & 86.4 \textcolor{gray}{±0.2} & 89.5 \textcolor{gray}{±0.2} & 86.6 \textcolor{gray}{±0.2} & 90.1 \textcolor{gray}{±0.2} & 88.2 \textcolor{gray}{±0.2} \\
\textbf{Libra XGradCAM+} & 91.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+6.3\%}) & 94.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+5.2\%}) & 96.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+11.6\%}) & 93.7 \textcolor{gray}{±0.2} (\textcolor{blue}{+3.9\%}) & 94.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+6.7\%}) \\
\midrule
FullGrad+ & 93.5 \textcolor{gray}{±0.2} & 94.3 \textcolor{gray}{±0.2} & 95.0 \textcolor{gray}{±0.2} & 91.8 \textcolor{gray}{±0.2} & 93.7 \textcolor{gray}{±0.2} \\
\textbf{Libra FullGrad+} & \textbf{99.2} \textcolor{gray}{±0.2} (\textcolor{blue}{+6.1\%}) & \textbf{97.9} \textcolor{gray}{±0.2} (\textcolor{blue}{+3.8\%}) & \textbf{99.6} \textcolor{gray}{±0.1} (\textcolor{blue}{+4.8\%}) & \textbf{97.4} \textcolor{gray}{±0.2} (\textcolor{blue}{+6.0\%}) & \textbf{98.5} \textcolor{gray}{±0.2} (\textcolor{blue}{+5.2\%}) \\
\bottomrule
\end{tabular}
\caption{How Least-Influential-First Deletion (LIF) AOPC evaluated using predicted labels varies with different model sizes.}
\label{across_models_depth_LIF_1p_AOPC_m_2}
\end{table}


==> files/tables_v1/across_models/depth/LIF_1p_accuracy/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ViT-Tiny & ViT-Small & ViT-Base & ViT-Large & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 58.6 \textcolor{gray}{±0.1} & 66.5 \textcolor{gray}{±0.1} & 73.3 \textcolor{gray}{±0.1} & 70.2 \textcolor{gray}{±0.1} & 67.1 \textcolor{gray}{±0.1} \\
RawAtt & 67.3 \textcolor{gray}{±0.1} & 72.8 \textcolor{gray}{±0.1} & 76.2 \textcolor{gray}{±0.1} & 67.6 \textcolor{gray}{±0.1} & 71.0 \textcolor{gray}{±0.1} \\
Attention Rollout & 65.4 \textcolor{gray}{±0.1} & 67.3 \textcolor{gray}{±0.1} & 73.8 \textcolor{gray}{±0.1} & 68.3 \textcolor{gray}{±0.1} & 68.7 \textcolor{gray}{±0.1} \\
AliLRP & 73.0 \textcolor{gray}{±0.1} & 70.6 \textcolor{gray}{±0.1} & 77.8 \textcolor{gray}{±0.1} & 72.5 \textcolor{gray}{±0.1} & 73.5 \textcolor{gray}{±0.1} \\
AttnLRP & 74.3 \textcolor{gray}{±0.1} & 77.3 \textcolor{gray}{±0.1} & 78.7 \textcolor{gray}{±0.1} & 77.6 \textcolor{gray}{±0.1} & 77.0 \textcolor{gray}{±0.1} \\
DecompX & 74.8 \textcolor{gray}{±0.1} & 75.3 \textcolor{gray}{±0.1} & 79.1 \textcolor{gray}{±0.1} & 75.8 \textcolor{gray}{±0.1} & 76.3 \textcolor{gray}{±0.1} \\
Integrated Gradients & 66.9 \textcolor{gray}{±0.1} & 73.9 \textcolor{gray}{±0.1} & 78.0 \textcolor{gray}{±0.1} & 73.5 \textcolor{gray}{±0.1} & 73.1 \textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 69.0 \textcolor{gray}{±0.1} & 72.1 \textcolor{gray}{±0.1} & 77.3 \textcolor{gray}{±0.1} & 72.8 \textcolor{gray}{±0.1} & 72.8 \textcolor{gray}{±0.1} \\
\textbf{Libra \IxG{} } & 74.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+8.4\%}) & 74.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.0\%}) & 80.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.8\%}) & 76.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.4\%}) & 76.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.1\%}) \\
\midrule
AttCAT & 74.8 \textcolor{gray}{±0.1} & 78.5 \textcolor{gray}{±0.1} & 82.5 \textcolor{gray}{±0.1} & 77.5 \textcolor{gray}{±0.1} & 78.3 \textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \underline{77.9} \textcolor{gray}{±0.1} (\textcolor{blue}{+4.2\%}) & \textbf{81.0} \textcolor{gray}{±0.1} (\textcolor{blue}{+3.2\%}) & \underline{86.7} \textcolor{gray}{±0.1} (\textcolor{blue}{+5.1\%}) & \underline{82.2} \textcolor{gray}{±0.1} (\textcolor{blue}{+6.1\%}) & \underline{81.9} \textcolor{gray}{±0.1} (\textcolor{blue}{+4.6\%}) \\
\midrule
GenAtt & 76.2 \textcolor{gray}{±0.1} & 79.1 \textcolor{gray}{±0.1} & 84.0 \textcolor{gray}{±0.1} & 78.2 \textcolor{gray}{±0.1} & 79.4 \textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 74.6 \textcolor{gray}{±0.1} (\textcolor{coral}{-2.1\%}) & 79.0 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.1\%}) & 84.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.4\%}) & 78.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.7\%}) & 79.2 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.2\%}) \\
\midrule
TokenTM & 74.2 \textcolor{gray}{±0.1} & 77.2 \textcolor{gray}{±0.1} & 83.1 \textcolor{gray}{±0.1} & 77.3 \textcolor{gray}{±0.1} & 77.9 \textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 73.7 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.6\%}) & 77.1 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.1\%}) & 83.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.1\%}) & 77.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.7\%}) & 78.0 \textcolor{gray}{±0.1} (+0.0\%) \\
\midrule
GradCAM+ & 65.1 \textcolor{gray}{±0.1} & 71.9 \textcolor{gray}{±0.1} & 78.5 \textcolor{gray}{±0.1} & 76.8 \textcolor{gray}{±0.1} & 73.1 \textcolor{gray}{±0.1} \\
\textbf{Libra GradCAM+} & 70.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+7.8\%}) & 78.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+8.4\%}) & 84.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+8.3\%}) & 79.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.0\%}) & 78.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+6.8\%}) \\
\midrule
HiResCAM & 48.3 \textcolor{gray}{±0.1} & 62.8 \textcolor{gray}{±0.1} & 79.5 \textcolor{gray}{±0.1} & 59.3 \textcolor{gray}{±0.1} & 62.5 \textcolor{gray}{±0.1} \\
\textbf{Libra HiResCAM} & 68.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+40.8\%}) & 76.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+21.2\%}) & 82.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+4.0\%}) & 73.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+24.4\%}) & 75.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+20.3\%}) \\
\midrule
XGradCAM+ & 66.7 \textcolor{gray}{±0.1} & 73.5 \textcolor{gray}{±0.1} & 73.3 \textcolor{gray}{±0.1} & 75.7 \textcolor{gray}{±0.1} & 72.3 \textcolor{gray}{±0.1} \\
\textbf{Libra XGradCAM+} & 72.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+9.0\%}) & 78.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+6.8\%}) & 85.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+16.6\%}) & 80.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.6\%}) & 79.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+9.5\%}) \\
\midrule
FullGrad+ & 73.4 \textcolor{gray}{±0.1} & 77.6 \textcolor{gray}{±0.1} & 81.6 \textcolor{gray}{±0.1} & 76.8 \textcolor{gray}{±0.1} & 77.4 \textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & \textbf{78.8} \textcolor{gray}{±0.1} (\textcolor{blue}{+7.3\%}) & \textbf{81.0} \textcolor{gray}{±0.1} (\textcolor{blue}{+4.4\%}) & \textbf{87.0} \textcolor{gray}{±0.0} (\textcolor{blue}{+6.6\%}) & \textbf{82.6} \textcolor{gray}{±0.1} (\textcolor{blue}{+7.6\%}) & \textbf{82.4} \textcolor{gray}{±0.1} (\textcolor{blue}{+6.5\%}) \\
\bottomrule
\end{tabular}
\caption{How Least-Influential-First Deletion (LIF) Accuracy evaluated using predicted labels varies with different model sizes.}
\label{across_models_depth_LIF_1p_accuracy_m_2}
\end{table}


==> files/tables_v1/across_models/depth/LIF_gt_AOPC/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ViT-Tiny & ViT-Small & ViT-Base & ViT-Large & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 82.8 \textcolor{gray}{±0.2} & 84.1 \textcolor{gray}{±0.2} & 87.5 \textcolor{gray}{±0.2} & 85.4 \textcolor{gray}{±0.2} & 84.9 \textcolor{gray}{±0.2} \\
RawAtt & 88.1 \textcolor{gray}{±0.2} & 89.4 \textcolor{gray}{±0.2} & 89.2 \textcolor{gray}{±0.1} & 83.3 \textcolor{gray}{±0.2} & 87.5 \textcolor{gray}{±0.2} \\
Attention Rollout & 87.2 \textcolor{gray}{±0.2} & 84.8 \textcolor{gray}{±0.2} & 87.9 \textcolor{gray}{±0.2} & 84.1 \textcolor{gray}{±0.2} & 86.0 \textcolor{gray}{±0.2} \\
AliLRP & 95.0 \textcolor{gray}{±0.3} & 88.2 \textcolor{gray}{±0.2} & 90.9 \textcolor{gray}{±0.2} & 87.7 \textcolor{gray}{±0.2} & 90.4 \textcolor{gray}{±0.2} \\
AttnLRP & 95.6 \textcolor{gray}{±0.2} & 94.6 \textcolor{gray}{±0.2} & 92.4 \textcolor{gray}{±0.2} & 92.9 \textcolor{gray}{±0.2} & 93.8 \textcolor{gray}{±0.2} \\
DecompX & 95.4 \textcolor{gray}{±0.2} & 92.2 \textcolor{gray}{±0.2} & 92.2 \textcolor{gray}{±0.2} & 91.0 \textcolor{gray}{±0.2} & 92.7 \textcolor{gray}{±0.2} \\
Integrated Gradients & 96.3 \textcolor{gray}{±0.2} & 95.4 \textcolor{gray}{±0.2} & 95.7 \textcolor{gray}{±0.2} & 93.3 \textcolor{gray}{±0.2} & 95.2 \textcolor{gray}{±0.2} \\
\midrule
\IxG{}  & 90.8 \textcolor{gray}{±0.2} & 90.0 \textcolor{gray}{±0.3} & 91.8 \textcolor{gray}{±0.2} & 88.4 \textcolor{gray}{±0.2} & 90.3 \textcolor{gray}{±0.2} \\
\textbf{Libra \IxG{} } & 96.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+6.2\%}) & 92.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+2.1\%}) & 93.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.4\%}) & 92.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+4.0\%}) & 93.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+3.4\%}) \\
\midrule
AttCAT & 98.0 \textcolor{gray}{±0.2} & 97.7 \textcolor{gray}{±0.2} & 98.4 \textcolor{gray}{±0.2} & 94.3 \textcolor{gray}{±0.2} & 97.1 \textcolor{gray}{±0.2} \\
\textbf{Libra AttCAT} & \underline{100.8} \textcolor{gray}{±0.2} (\textcolor{blue}{+2.9\%}) & \underline{100.0} \textcolor{gray}{±0.2} (\textcolor{blue}{+2.4\%}) & \underline{100.8} \textcolor{gray}{±0.2} (\textcolor{blue}{+2.4\%}) & \underline{98.5} \textcolor{gray}{±0.2} (\textcolor{blue}{+4.5\%}) & \underline{100.0} \textcolor{gray}{±0.2} (\textcolor{blue}{+3.0\%}) \\
\midrule
GenAtt & 95.4 \textcolor{gray}{±0.2} & 94.7 \textcolor{gray}{±0.2} & 95.7 \textcolor{gray}{±0.2} & 92.8 \textcolor{gray}{±0.2} & 94.6 \textcolor{gray}{±0.2} \\
\textbf{Libra GenAtt} & 94.3 \textcolor{gray}{±0.2} (\textcolor{coral}{-1.1\%}) & 94.5 \textcolor{gray}{±0.2} (\textcolor{coral}{-0.2\%}) & 96.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.3\%}) & 93.2 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.5\%}) & 94.5 \textcolor{gray}{±0.2} (\textcolor{coral}{-0.1\%}) \\
\midrule
TokenTM & 93.4 \textcolor{gray}{±0.2} & 92.7 \textcolor{gray}{±0.2} & 94.4 \textcolor{gray}{±0.1} & 91.6 \textcolor{gray}{±0.2} & 93.0 \textcolor{gray}{±0.2} \\
\textbf{Libra TokenTM} & 92.7 \textcolor{gray}{±0.2} (\textcolor{coral}{-0.7\%}) & 92.8 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.1\%}) & 94.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.2\%}) & 92.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.5\%}) & 93.0 \textcolor{gray}{±0.2} (+0.0\%) \\
\midrule
GradCAM+ & 88.6 \textcolor{gray}{±0.2} & 90.5 \textcolor{gray}{±0.2} & 93.5 \textcolor{gray}{±0.2} & 92.9 \textcolor{gray}{±0.2} & 91.4 \textcolor{gray}{±0.2} \\
\textbf{Libra GradCAM+} & 93.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+5.2\%}) & 96.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+6.1\%}) & 98.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+4.9\%}) & 94.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.6\%}) & 95.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+4.4\%}) \\
\midrule
HiResCAM & 76.6 \textcolor{gray}{±0.3} & 81.8 \textcolor{gray}{±0.3} & 93.3 \textcolor{gray}{±0.2} & 76.7 \textcolor{gray}{±0.2} & 82.1 \textcolor{gray}{±0.3} \\
\textbf{Libra HiResCAM} & 90.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+17.7\%}) & 93.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+14.1\%}) & 96.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+3.0\%}) & 90.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+17.3\%}) & 92.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+12.5\%}) \\
\midrule
XGradCAM+ & 90.5 \textcolor{gray}{±0.3} & 91.8 \textcolor{gray}{±0.2} & 88.9 \textcolor{gray}{±0.3} & 92.1 \textcolor{gray}{±0.2} & 90.8 \textcolor{gray}{±0.2} \\
\textbf{Libra XGradCAM+} & 95.5 \textcolor{gray}{±0.2} (\textcolor{blue}{+5.6\%}) & 96.5 \textcolor{gray}{±0.2} (\textcolor{blue}{+5.1\%}) & 98.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+10.8\%}) & 95.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+3.5\%}) & 96.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+6.2\%}) \\
\midrule
FullGrad+ & 96.3 \textcolor{gray}{±0.2} & 96.3 \textcolor{gray}{±0.2} & 96.6 \textcolor{gray}{±0.2} & 93.8 \textcolor{gray}{±0.2} & 95.7 \textcolor{gray}{±0.2} \\
\textbf{Libra FullGrad+} & \textbf{101.8} \textcolor{gray}{±0.2} (\textcolor{blue}{+5.7\%}) & \textbf{100.1} \textcolor{gray}{±0.2} (\textcolor{blue}{+4.0\%}) & \textbf{101.2} \textcolor{gray}{±0.2} (\textcolor{blue}{+4.8\%}) & \textbf{98.9} \textcolor{gray}{±0.2} (\textcolor{blue}{+5.4\%}) & \textbf{100.5} \textcolor{gray}{±0.2} (\textcolor{blue}{+4.9\%}) \\
\bottomrule
\end{tabular}
\caption{How Least-Influential-First Deletion (LIF) AOPC evaluated using ground-truth labels varies with different model sizes.}
\label{across_models_depth_LIF_gt_AOPC_m_2}
\end{table}


==> files/tables_v1/across_models/depth/LIF_gt_accuracy/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ViT-Tiny & ViT-Small & ViT-Base & ViT-Large & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 49.2 \textcolor{gray}{±0.1} & 57.7 \textcolor{gray}{±0.1} & 65.2 \textcolor{gray}{±0.1} & 62.9 \textcolor{gray}{±0.1} & 58.8 \textcolor{gray}{±0.1} \\
RawAtt & 55.2 \textcolor{gray}{±0.1} & 63.9 \textcolor{gray}{±0.1} & 67.5 \textcolor{gray}{±0.1} & 60.3 \textcolor{gray}{±0.1} & 61.7 \textcolor{gray}{±0.1} \\
Attention Rollout & 54.4 \textcolor{gray}{±0.1} & 58.6 \textcolor{gray}{±0.1} & 65.9 \textcolor{gray}{±0.1} & 61.9 \textcolor{gray}{±0.1} & 60.2 \textcolor{gray}{±0.1} \\
AliLRP & 63.1 \textcolor{gray}{±0.1} & 62.5 \textcolor{gray}{±0.1} & 69.9 \textcolor{gray}{±0.1} & 65.4 \textcolor{gray}{±0.1} & 65.2 \textcolor{gray}{±0.1} \\
AttnLRP & 63.2 \textcolor{gray}{±0.1} & 68.4 \textcolor{gray}{±0.1} & 71.0 \textcolor{gray}{±0.1} & 70.3 \textcolor{gray}{±0.1} & 68.2 \textcolor{gray}{±0.1} \\
DecompX & 63.3 \textcolor{gray}{±0.1} & 66.5 \textcolor{gray}{±0.1} & 71.1 \textcolor{gray}{±0.1} & 68.8 \textcolor{gray}{±0.1} & 67.4 \textcolor{gray}{±0.1} \\
Integrated Gradients & 64.0 \textcolor{gray}{±0.1} & 69.6 \textcolor{gray}{±0.1} & 74.4 \textcolor{gray}{±0.1} & 71.1 \textcolor{gray}{±0.1} & 69.8 \textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 58.6 \textcolor{gray}{±0.1} & 64.2 \textcolor{gray}{±0.1} & 69.9 \textcolor{gray}{±0.1} & 65.8 \textcolor{gray}{±0.1} & 64.6 \textcolor{gray}{±0.1} \\
\textbf{Libra \IxG{} } & 65.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+11.3\%}) & 66.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.4\%}) & 72.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.7\%}) & 70.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+6.6\%}) & 68.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+6.1\%}) \\
\midrule
AttCAT & 66.5 \textcolor{gray}{±0.1} & 71.9 \textcolor{gray}{±0.1} & 76.8 \textcolor{gray}{±0.1} & 71.8 \textcolor{gray}{±0.1} & 71.7 \textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \underline{69.5} \textcolor{gray}{±0.1} (\textcolor{blue}{+4.5\%}) & \underline{74.2} \textcolor{gray}{±0.1} (\textcolor{blue}{+3.3\%}) & \underline{80.2} \textcolor{gray}{±0.1} (\textcolor{blue}{+4.5\%}) & \underline{76.3} \textcolor{gray}{±0.1} (\textcolor{blue}{+6.2\%}) & \underline{75.0} \textcolor{gray}{±0.1} (\textcolor{blue}{+4.6\%}) \\
\midrule
GenAtt & 63.6 \textcolor{gray}{±0.1} & 69.6 \textcolor{gray}{±0.1} & 74.8 \textcolor{gray}{±0.1} & 70.0 \textcolor{gray}{±0.1} & 69.5 \textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 62.3 \textcolor{gray}{±0.1} (\textcolor{coral}{-2.0\%}) & 69.5 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.2\%}) & 75.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.4\%}) & 70.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.3\%}) & 69.4 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.1\%}) \\
\midrule
TokenTM & 61.2 \textcolor{gray}{±0.1} & 67.4 \textcolor{gray}{±0.1} & 73.5 \textcolor{gray}{±0.1} & 68.9 \textcolor{gray}{±0.1} & 67.7 \textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 60.8 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.6\%}) & 67.4 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.1\%}) & 73.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.1\%}) & 69.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.8\%}) & 67.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.1\%}) \\
\midrule
GradCAM+ & 57.9 \textcolor{gray}{±0.1} & 65.0 \textcolor{gray}{±0.1} & 72.0 \textcolor{gray}{±0.1} & 70.5 \textcolor{gray}{±0.1} & 66.3 \textcolor{gray}{±0.1} \\
\textbf{Libra GradCAM+} & 61.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+7.0\%}) & 70.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+8.9\%}) & 78.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+8.3\%}) & 72.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.9\%}) & 70.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+6.7\%}) \\
\midrule
HiResCAM & 42.4 \textcolor{gray}{±0.1} & 55.8 \textcolor{gray}{±0.1} & 71.9 \textcolor{gray}{±0.1} & 53.6 \textcolor{gray}{±0.1} & 55.9 \textcolor{gray}{±0.1} \\
\textbf{Libra HiResCAM} & 60.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+41.5\%}) & 68.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+22.6\%}) & 75.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.1\%}) & 67.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+25.7\%}) & 67.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+21.3\%}) \\
\midrule
XGradCAM+ & 59.5 \textcolor{gray}{±0.1} & 66.3 \textcolor{gray}{±0.1} & 67.0 \textcolor{gray}{±0.1} & 69.5 \textcolor{gray}{±0.1} & 65.6 \textcolor{gray}{±0.1} \\
\textbf{Libra XGradCAM+} & 64.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+8.3\%}) & 71.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+7.7\%}) & 78.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+16.6\%}) & 73.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.7\%}) & 71.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+9.6\%}) \\
\midrule
FullGrad+ & 64.5 \textcolor{gray}{±0.1} & 70.3 \textcolor{gray}{±0.1} & 75.2 \textcolor{gray}{±0.1} & 71.5 \textcolor{gray}{±0.1} & 70.4 \textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & \textbf{70.2} \textcolor{gray}{±0.1} (\textcolor{blue}{+8.8\%}) & \textbf{74.4} \textcolor{gray}{±0.1} (\textcolor{blue}{+5.9\%}) & \textbf{80.6} \textcolor{gray}{±0.1} (\textcolor{blue}{+7.1\%}) & \textbf{76.8} \textcolor{gray}{±0.1} (\textcolor{blue}{+7.5\%}) & \textbf{75.5} \textcolor{gray}{±0.1} (\textcolor{blue}{+7.3\%}) \\
\bottomrule
\end{tabular}
\caption{How Least-Influential-First Deletion (LIF) Accuracy evaluated using ground-truth labels varies with different model sizes.}
\label{across_models_depth_LIF_gt_accuracy_m_2}
\end{table}


==> files/tables_v1/across_models/depth/MIF_1p_AOPC/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ViT-Tiny & ViT-Small & ViT-Base & ViT-Large & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 20.7 \textcolor{gray}{±0.2} & 18.6 \textcolor{gray}{±0.2} & 14.2 \textcolor{gray}{±0.2} & 15.8 \textcolor{gray}{±0.2} & 17.3 \textcolor{gray}{±0.2} \\
RawAtt & 44.8 \textcolor{gray}{±0.3} & 41.2 \textcolor{gray}{±0.3} & 27.9 \textcolor{gray}{±0.3} & 25.3 \textcolor{gray}{±0.2} & 34.8 \textcolor{gray}{±0.3} \\
Attention Rollout & 39.8 \textcolor{gray}{±0.3} & 28.8 \textcolor{gray}{±0.2} & 21.2 \textcolor{gray}{±0.2} & 18.3 \textcolor{gray}{±0.3} & 27.0 \textcolor{gray}{±0.3} \\
AliLRP & 39.3 \textcolor{gray}{±0.2} & 26.2 \textcolor{gray}{±0.3} & 19.1 \textcolor{gray}{±0.2} & 19.2 \textcolor{gray}{±0.2} & 26.0 \textcolor{gray}{±0.2} \\
AttnLRP & 44.3 \textcolor{gray}{±0.3} & 35.2 \textcolor{gray}{±0.2} & 23.4 \textcolor{gray}{±0.2} & 27.6 \textcolor{gray}{±0.3} & 32.6 \textcolor{gray}{±0.3} \\
DecompX & 44.8 \textcolor{gray}{±0.3} & 33.6 \textcolor{gray}{±0.2} & 22.8 \textcolor{gray}{±0.2} & 25.3 \textcolor{gray}{±0.3} & 31.6 \textcolor{gray}{±0.3} \\
Integrated Gradients & 33.3 \textcolor{gray}{±0.2} & 29.3 \textcolor{gray}{±0.3} & 21.4 \textcolor{gray}{±0.2} & 21.9 \textcolor{gray}{±0.2} & 26.5 \textcolor{gray}{±0.2} \\
\midrule
\IxG{}  & 31.8 \textcolor{gray}{±0.2} & 25.0 \textcolor{gray}{±0.3} & 20.2 \textcolor{gray}{±0.2} & 19.6 \textcolor{gray}{±0.2} & 24.2 \textcolor{gray}{±0.2} \\
\textbf{Libra \IxG{} } & 44.0 \textcolor{gray}{±0.3} (\textcolor{blue}{+38.3\%}) & 32.2 \textcolor{gray}{±0.2} (\textcolor{blue}{+28.5\%}) & 23.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+15.8\%}) & 26.1 \textcolor{gray}{±0.3} (\textcolor{blue}{+33.1\%}) & 31.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+30.0\%}) \\
\midrule
AttCAT & 42.0 \textcolor{gray}{±0.3} & 38.2 \textcolor{gray}{±0.3} & 28.8 \textcolor{gray}{±0.2} & 29.0 \textcolor{gray}{±0.3} & 34.5 \textcolor{gray}{±0.3} \\
\textbf{Libra AttCAT} & \underline{52.1} \textcolor{gray}{±0.2} (\textcolor{blue}{+24.1\%}) & \textbf{48.9} \textcolor{gray}{±0.3} (\textcolor{blue}{+28.0\%}) & \textbf{41.5} \textcolor{gray}{±0.3} (\textcolor{blue}{+44.2\%}) & \underline{44.5} \textcolor{gray}{±0.3} (\textcolor{blue}{+53.6\%}) & \underline{46.8} \textcolor{gray}{±0.3} (\textcolor{blue}{+35.6\%}) \\
\midrule
GenAtt & 49.4 \textcolor{gray}{±0.3} & 46.3 \textcolor{gray}{±0.3} & 37.9 \textcolor{gray}{±0.2} & 36.5 \textcolor{gray}{±0.3} & 42.5 \textcolor{gray}{±0.3} \\
\textbf{Libra GenAtt} & 50.5 \textcolor{gray}{±0.2} (\textcolor{blue}{+2.2\%}) & 48.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+4.2\%}) & 40.4 \textcolor{gray}{±0.3} (\textcolor{blue}{+6.6\%}) & 39.6 \textcolor{gray}{±0.3} (\textcolor{blue}{+8.7\%}) & 44.7 \textcolor{gray}{±0.3} (\textcolor{blue}{+5.1\%}) \\
\midrule
TokenTM & 48.3 \textcolor{gray}{±0.3} & 45.9 \textcolor{gray}{±0.3} & 37.4 \textcolor{gray}{±0.3} & 34.9 \textcolor{gray}{±0.3} & 41.6 \textcolor{gray}{±0.3} \\
\textbf{Libra TokenTM} & 49.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+1.9\%}) & 47.3 \textcolor{gray}{±0.3} (\textcolor{blue}{+3.0\%}) & 38.9 \textcolor{gray}{±0.3} (\textcolor{blue}{+3.8\%}) & 37.4 \textcolor{gray}{±0.3} (\textcolor{blue}{+7.1\%}) & 43.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+3.8\%}) \\
\midrule
GradCAM+ & 40.1 \textcolor{gray}{±0.2} & 35.8 \textcolor{gray}{±0.3} & 27.6 \textcolor{gray}{±0.2} & 33.0 \textcolor{gray}{±0.2} & 34.1 \textcolor{gray}{±0.2} \\
\textbf{Libra GradCAM+} & 46.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+15.7\%}) & 46.1 \textcolor{gray}{±0.3} (\textcolor{blue}{+28.7\%}) & 39.6 \textcolor{gray}{±0.2} (\textcolor{blue}{+43.5\%}) & 40.1 \textcolor{gray}{±0.3} (\textcolor{blue}{+21.8\%}) & 43.0 \textcolor{gray}{±0.3} (\textcolor{blue}{+26.2\%}) \\
\midrule
HiResCAM & 19.5 \textcolor{gray}{±0.3} & 15.3 \textcolor{gray}{±0.2} & 28.5 \textcolor{gray}{±0.2} & 12.2 \textcolor{gray}{±0.2} & 18.9 \textcolor{gray}{±0.2} \\
\textbf{Libra HiResCAM} & 44.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+125.6\%}) & 44.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+190.6\%}) & 37.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+29.6\%}) & 33.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+171.8\%}) & 39.7 \textcolor{gray}{±0.2} (\textcolor{blue}{+110.0\%}) \\
\midrule
XGradCAM+ & 41.2 \textcolor{gray}{±0.2} & 36.2 \textcolor{gray}{±0.3} & 21.5 \textcolor{gray}{±0.2} & 30.5 \textcolor{gray}{±0.3} & 32.4 \textcolor{gray}{±0.3} \\
\textbf{Libra XGradCAM+} & 49.5 \textcolor{gray}{±0.2} (\textcolor{blue}{+20.1\%}) & 47.8 \textcolor{gray}{±0.3} (\textcolor{blue}{+32.0\%}) & \textbf{41.5} \textcolor{gray}{±0.2} (\textcolor{blue}{+92.8\%}) & 42.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+38.3\%}) & 45.3 \textcolor{gray}{±0.3} (\textcolor{blue}{+39.8\%}) \\
\midrule
FullGrad+ & 39.2 \textcolor{gray}{±0.3} & 36.1 \textcolor{gray}{±0.3} & 26.3 \textcolor{gray}{±0.2} & 28.9 \textcolor{gray}{±0.3} & 32.6 \textcolor{gray}{±0.3} \\
\textbf{Libra FullGrad+} & \textbf{52.7} \textcolor{gray}{±0.2} (\textcolor{blue}{+34.7\%}) & \textbf{48.9} \textcolor{gray}{±0.3} (\textcolor{blue}{+35.3\%}) & 41.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+56.7\%}) & \textbf{45.3} \textcolor{gray}{±0.3} (\textcolor{blue}{+56.5\%}) & \textbf{47.0} \textcolor{gray}{±0.3} (\textcolor{blue}{+44.1\%}) \\
\bottomrule
\end{tabular}
\caption{How Most-Influential-First Deletion (MIF) AOPC evaluated using predicted labels varies with different model sizes.}
\label{across_models_depth_MIF_1p_AOPC_m_2}
\end{table}


==> files/tables_v1/across_models/depth/MIF_1p_accuracy/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ViT-Tiny & ViT-Small & ViT-Base & ViT-Large & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 40.5 \textcolor{gray}{±0.1} & 33.8 \textcolor{gray}{±0.1} & 26.5 \textcolor{gray}{±0.1} & 29.5 \textcolor{gray}{±0.1} & 32.6 \textcolor{gray}{±0.1} \\
RawAtt & 69.5 \textcolor{gray}{±0.1} & 58.7 \textcolor{gray}{±0.1} & 44.6 \textcolor{gray}{±0.1} & 39.1 \textcolor{gray}{±0.1} & 53.0 \textcolor{gray}{±0.1} \\
Attention Rollout & 64.1 \textcolor{gray}{±0.1} & 45.1 \textcolor{gray}{±0.1} & 35.4 \textcolor{gray}{±0.1} & 31.4 \textcolor{gray}{±0.1} & 44.0 \textcolor{gray}{±0.1} \\
AliLRP & 64.4 \textcolor{gray}{±0.1} & 42.3 \textcolor{gray}{±0.1} & 33.3 \textcolor{gray}{±0.1} & 33.2 \textcolor{gray}{±0.1} & 43.3 \textcolor{gray}{±0.1} \\
AttnLRP & 69.7 \textcolor{gray}{±0.1} & 52.4 \textcolor{gray}{±0.1} & 38.5 \textcolor{gray}{±0.1} & 41.8 \textcolor{gray}{±0.1} & 50.6 \textcolor{gray}{±0.1} \\
DecompX & 70.4 \textcolor{gray}{±0.1} & 50.4 \textcolor{gray}{±0.1} & 37.8 \textcolor{gray}{±0.1} & 38.9 \textcolor{gray}{±0.1} & 49.4 \textcolor{gray}{±0.1} \\
Integrated Gradients & 57.1 \textcolor{gray}{±0.1} & 46.0 \textcolor{gray}{±0.1} & 35.4 \textcolor{gray}{±0.1} & 35.9 \textcolor{gray}{±0.1} & 43.6 \textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 55.6 \textcolor{gray}{±0.1} & 41.8 \textcolor{gray}{±0.1} & 34.4 \textcolor{gray}{±0.1} & 33.9 \textcolor{gray}{±0.1} & 41.4 \textcolor{gray}{±0.1} \\
\textbf{Libra \IxG{} } & 70.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+27.2\%}) & 49.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+18.0\%}) & 38.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+12.0\%}) & 40.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+19.6\%}) & 49.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+20.2\%}) \\
\midrule
AttCAT & 69.3 \textcolor{gray}{±0.1} & 58.9 \textcolor{gray}{±0.1} & 46.9 \textcolor{gray}{±0.1} & 44.8 \textcolor{gray}{±0.1} & 55.0 \textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \underline{81.0} \textcolor{gray}{±0.1} (\textcolor{blue}{+16.7\%}) & \textbf{70.3} \textcolor{gray}{±0.1} (\textcolor{blue}{+19.3\%}) & \underline{63.5} \textcolor{gray}{±0.1} (\textcolor{blue}{+35.4\%}) & \underline{61.3} \textcolor{gray}{±0.1} (\textcolor{blue}{+36.9\%}) & \underline{69.0} \textcolor{gray}{±0.1} (\textcolor{blue}{+25.5\%}) \\
\midrule
GenAtt & 77.1 \textcolor{gray}{±0.1} & 66.3 \textcolor{gray}{±0.1} & 58.2 \textcolor{gray}{±0.1} & 51.8 \textcolor{gray}{±0.1} & 63.4 \textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 78.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.7\%}) & 68.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.9\%}) & 61.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.8\%}) & 55.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+6.8\%}) & 65.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+4.0\%}) \\
\midrule
TokenTM & 75.0 \textcolor{gray}{±0.1} & 65.2 \textcolor{gray}{±0.1} & 56.8 \textcolor{gray}{±0.1} & 50.0 \textcolor{gray}{±0.1} & 61.7 \textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 76.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.6\%}) & 66.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.0\%}) & 59.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+4.1\%}) & 52.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.0\%}) & 63.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.0\%}) \\
\midrule
GradCAM+ & 66.2 \textcolor{gray}{±0.1} & 55.5 \textcolor{gray}{±0.1} & 45.6 \textcolor{gray}{±0.1} & 48.6 \textcolor{gray}{±0.1} & 54.0 \textcolor{gray}{±0.1} \\
\textbf{Libra GradCAM+} & 72.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+10.1\%}) & 66.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+19.7\%}) & 61.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+34.8\%}) & 56.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+16.2\%}) & 64.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+19.2\%}) \\
\midrule
HiResCAM & 39.0 \textcolor{gray}{±0.1} & 29.5 \textcolor{gray}{±0.1} & 45.4 \textcolor{gray}{±0.1} & 25.7 \textcolor{gray}{±0.1} & 34.9 \textcolor{gray}{±0.1} \\
\textbf{Libra HiResCAM} & 69.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+79.1\%}) & 63.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+114.7\%}) & 56.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+24.8\%}) & 49.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+90.7\%}) & 59.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+71.1\%}) \\
\midrule
XGradCAM+ & 67.5 \textcolor{gray}{±0.1} & 55.9 \textcolor{gray}{±0.1} & 38.6 \textcolor{gray}{±0.1} & 45.9 \textcolor{gray}{±0.1} & 52.0 \textcolor{gray}{±0.1} \\
\textbf{Libra XGradCAM+} & 77.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+14.1\%}) & 68.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+22.4\%}) & \textbf{63.9} \textcolor{gray}{±0.1} (\textcolor{blue}{+65.6\%}) & 58.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+28.1\%}) & 67.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+29.0\%}) \\
\midrule
FullGrad+ & 65.9 \textcolor{gray}{±0.1} & 55.8 \textcolor{gray}{±0.1} & 44.2 \textcolor{gray}{±0.1} & 45.1 \textcolor{gray}{±0.1} & 52.7 \textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & \textbf{81.7} \textcolor{gray}{±0.1} (\textcolor{blue}{+24.0\%}) & \underline{70.1} \textcolor{gray}{±0.1} (\textcolor{blue}{+25.8\%}) & 63.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+42.9\%}) & \textbf{62.4} \textcolor{gray}{±0.1} (\textcolor{blue}{+38.5\%}) & \textbf{69.3} \textcolor{gray}{±0.1} (\textcolor{blue}{+31.5\%}) \\
\bottomrule
\end{tabular}
\caption{How Most-Influential-First Deletion (MIF) Accuracy evaluated using predicted labels varies with different model sizes.}
\label{across_models_depth_MIF_1p_accuracy_m_2}
\end{table}


==> files/tables_v1/across_models/depth/MIF_gt_AOPC/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ViT-Tiny & ViT-Small & ViT-Base & ViT-Large & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 17.0 \textcolor{gray}{±0.2} & 15.8 \textcolor{gray}{±0.3} & 12.3 \textcolor{gray}{±0.2} & 14.1 \textcolor{gray}{±0.2} & 14.8 \textcolor{gray}{±0.2} \\
RawAtt & 38.6 \textcolor{gray}{±0.3} & 36.5 \textcolor{gray}{±0.3} & 25.0 \textcolor{gray}{±0.3} & 22.9 \textcolor{gray}{±0.3} & 30.7 \textcolor{gray}{±0.3} \\
Attention Rollout & 33.6 \textcolor{gray}{±0.3} & 25.1 \textcolor{gray}{±0.4} & 18.8 \textcolor{gray}{±0.3} & 16.5 \textcolor{gray}{±0.3} & 23.5 \textcolor{gray}{±0.3} \\
AliLRP & 33.4 \textcolor{gray}{±0.3} & 22.8 \textcolor{gray}{±0.3} & 16.7 \textcolor{gray}{±0.2} & 17.2 \textcolor{gray}{±0.3} & 22.5 \textcolor{gray}{±0.3} \\
AttnLRP & 37.8 \textcolor{gray}{±0.3} & 30.9 \textcolor{gray}{±0.3} & 20.8 \textcolor{gray}{±0.3} & 24.8 \textcolor{gray}{±0.3} & 28.6 \textcolor{gray}{±0.3} \\
DecompX & 38.2 \textcolor{gray}{±0.3} & 29.5 \textcolor{gray}{±0.3} & 20.3 \textcolor{gray}{±0.3} & 22.6 \textcolor{gray}{±0.3} & 27.7 \textcolor{gray}{±0.3} \\
Integrated Gradients & 32.8 \textcolor{gray}{±0.3} & 29.1 \textcolor{gray}{±0.3} & 22.5 \textcolor{gray}{±0.2} & 23.1 \textcolor{gray}{±0.3} & 26.9 \textcolor{gray}{±0.3} \\
\midrule
\IxG{}  & 26.3 \textcolor{gray}{±0.3} & 21.6 \textcolor{gray}{±0.3} & 17.7 \textcolor{gray}{±0.2} & 17.5 \textcolor{gray}{±0.3} & 20.8 \textcolor{gray}{±0.2} \\
\textbf{Libra \IxG{} } & 37.5 \textcolor{gray}{±0.3} (\textcolor{blue}{+42.6\%}) & 28.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+30.4\%}) & 20.8 \textcolor{gray}{±0.3} (\textcolor{blue}{+17.4\%}) & 23.4 \textcolor{gray}{±0.3} (\textcolor{blue}{+33.5\%}) & 27.5 \textcolor{gray}{±0.3} (\textcolor{blue}{+32.2\%}) \\
\midrule
AttCAT & 35.6 \textcolor{gray}{±0.3} & 33.4 \textcolor{gray}{±0.3} & 25.3 \textcolor{gray}{±0.2} & 25.7 \textcolor{gray}{±0.3} & 30.0 \textcolor{gray}{±0.3} \\
\textbf{Libra AttCAT} & \underline{45.0} \textcolor{gray}{±0.3} (\textcolor{blue}{+26.6\%}) & \textbf{43.9} \textcolor{gray}{±0.3} (\textcolor{blue}{+31.4\%}) & \underline{37.5} \textcolor{gray}{±0.3} (\textcolor{blue}{+47.9\%}) & \underline{40.5} \textcolor{gray}{±0.3} (\textcolor{blue}{+57.3\%}) & \underline{41.7} \textcolor{gray}{±0.3} (\textcolor{blue}{+39.0\%}) \\
\midrule
GenAtt & 42.7 \textcolor{gray}{±0.3} & 41.3 \textcolor{gray}{±0.3} & 34.2 \textcolor{gray}{±0.3} & 33.2 \textcolor{gray}{±0.3} & 37.8 \textcolor{gray}{±0.3} \\
\textbf{Libra GenAtt} & 43.6 \textcolor{gray}{±0.3} (\textcolor{blue}{+2.3\%}) & 43.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+4.6\%}) & 36.6 \textcolor{gray}{±0.3} (\textcolor{blue}{+6.8\%}) & 36.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+8.9\%}) & 39.9 \textcolor{gray}{±0.3} (\textcolor{blue}{+5.4\%}) \\
\midrule
TokenTM & 41.8 \textcolor{gray}{±0.3} & 40.8 \textcolor{gray}{±0.3} & 33.8 \textcolor{gray}{±0.3} & 31.8 \textcolor{gray}{±0.3} & 37.1 \textcolor{gray}{±0.3} \\
\textbf{Libra TokenTM} & 42.6 \textcolor{gray}{±0.3} (\textcolor{blue}{+2.0\%}) & 42.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+3.4\%}) & 35.1 \textcolor{gray}{±0.3} (\textcolor{blue}{+4.0\%}) & 34.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+7.4\%}) & 38.5 \textcolor{gray}{±0.3} (\textcolor{blue}{+4.0\%}) \\
\midrule
GradCAM+ & 34.1 \textcolor{gray}{±0.3} & 31.5 \textcolor{gray}{±0.3} & 24.8 \textcolor{gray}{±0.2} & 30.0 \textcolor{gray}{±0.3} & 30.1 \textcolor{gray}{±0.3} \\
\textbf{Libra GradCAM+} & 39.9 \textcolor{gray}{±0.3} (\textcolor{blue}{+16.8\%}) & 41.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+30.7\%}) & 35.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+44.8\%}) & 36.7 \textcolor{gray}{±0.3} (\textcolor{blue}{+22.0\%}) & 38.4 \textcolor{gray}{±0.3} (\textcolor{blue}{+27.5\%}) \\
\midrule
HiResCAM & 15.8 \textcolor{gray}{±0.3} & 13.1 \textcolor{gray}{±0.2} & 25.4 \textcolor{gray}{±0.3} & 10.6 \textcolor{gray}{±0.2} & 16.2 \textcolor{gray}{±0.2} \\
\textbf{Libra HiResCAM} & 37.8 \textcolor{gray}{±0.3} (\textcolor{blue}{+138.5\%}) & 39.6 \textcolor{gray}{±0.3} (\textcolor{blue}{+202.6\%}) & 33.4 \textcolor{gray}{±0.3} (\textcolor{blue}{+31.7\%}) & 30.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+186.3\%}) & 35.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+117.4\%}) \\
\midrule
XGradCAM+ & 35.1 \textcolor{gray}{±0.3} & 31.9 \textcolor{gray}{±0.4} & 19.0 \textcolor{gray}{±0.2} & 27.7 \textcolor{gray}{±0.3} & 28.4 \textcolor{gray}{±0.3} \\
\textbf{Libra XGradCAM+} & 42.7 \textcolor{gray}{±0.3} (\textcolor{blue}{+21.7\%}) & 42.8 \textcolor{gray}{±0.3} (\textcolor{blue}{+34.1\%}) & \textbf{37.7} \textcolor{gray}{±0.2} (\textcolor{blue}{+98.6\%}) & 38.6 \textcolor{gray}{±0.3} (\textcolor{blue}{+39.2\%}) & 40.4 \textcolor{gray}{±0.3} (\textcolor{blue}{+42.3\%}) \\
\midrule
FullGrad+ & 33.1 \textcolor{gray}{±0.3} & 31.5 \textcolor{gray}{±0.3} & 23.1 \textcolor{gray}{±0.3} & 25.8 \textcolor{gray}{±0.3} & 28.4 \textcolor{gray}{±0.3} \\
\textbf{Libra FullGrad+} & \textbf{45.6} \textcolor{gray}{±0.3} (\textcolor{blue}{+37.8\%}) & \underline{43.8} \textcolor{gray}{±0.3} (\textcolor{blue}{+39.0\%}) & 37.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+60.9\%}) & \textbf{41.2} \textcolor{gray}{±0.3} (\textcolor{blue}{+59.5\%}) & \textbf{41.9} \textcolor{gray}{±0.3} (\textcolor{blue}{+47.8\%}) \\
\bottomrule
\end{tabular}
\caption{How Most-Influential-First Deletion (MIF) AOPC evaluated using ground-truth labels varies with different model sizes.}
\label{across_models_depth_MIF_gt_AOPC_m_2}
\end{table}


==> files/tables_v1/across_models/depth/MIF_gt_accuracy/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ViT-Tiny & ViT-Small & ViT-Base & ViT-Large & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 50.1 \textcolor{gray}{±0.1} & 41.8 \textcolor{gray}{±0.1} & 34.5 \textcolor{gray}{±0.1} & 36.9 \textcolor{gray}{±0.1} & 40.8 \textcolor{gray}{±0.1} \\
RawAtt & 74.0 \textcolor{gray}{±0.1} & 63.1 \textcolor{gray}{±0.1} & 50.1 \textcolor{gray}{±0.1} & 45.4 \textcolor{gray}{±0.1} & 58.2 \textcolor{gray}{±0.1} \\
Attention Rollout & 68.7 \textcolor{gray}{±0.1} & 51.2 \textcolor{gray}{±0.1} & 41.9 \textcolor{gray}{±0.1} & 39.0 \textcolor{gray}{±0.1} & 50.2 \textcolor{gray}{±0.1} \\
AliLRP & 68.9 \textcolor{gray}{±0.1} & 48.9 \textcolor{gray}{±0.1} & 39.8 \textcolor{gray}{±0.1} & 39.8 \textcolor{gray}{±0.1} & 49.4 \textcolor{gray}{±0.1} \\
AttnLRP & 73.4 \textcolor{gray}{±0.1} & 57.7 \textcolor{gray}{±0.1} & 44.5 \textcolor{gray}{±0.1} & 47.1 \textcolor{gray}{±0.1} & 55.7 \textcolor{gray}{±0.1} \\
DecompX & 74.0 \textcolor{gray}{±0.1} & 56.0 \textcolor{gray}{±0.1} & 44.0 \textcolor{gray}{±0.1} & 44.4 \textcolor{gray}{±0.1} & 54.6 \textcolor{gray}{±0.1} \\
Integrated Gradients & 69.7 \textcolor{gray}{±0.1} & 56.9 \textcolor{gray}{±0.1} & 46.9 \textcolor{gray}{±0.1} & 46.3 \textcolor{gray}{±0.1} & 54.9 \textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 61.1 \textcolor{gray}{±0.1} & 47.9 \textcolor{gray}{±0.1} & 40.4 \textcolor{gray}{±0.1} & 40.1 \textcolor{gray}{±0.1} & 47.4 \textcolor{gray}{±0.1} \\
\textbf{Libra \IxG{} } & 74.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+22.0\%}) & 54.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+14.7\%}) & 44.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+10.8\%}) & 45.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+14.4\%}) & 55.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+16.2\%}) \\
\midrule
AttCAT & 72.6 \textcolor{gray}{±0.1} & 62.1 \textcolor{gray}{±0.1} & 50.4 \textcolor{gray}{±0.1} & 48.7 \textcolor{gray}{±0.1} & 58.5 \textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \underline{83.6} \textcolor{gray}{±0.1} (\textcolor{blue}{+15.2\%}) & \textbf{73.6} \textcolor{gray}{±0.1} (\textcolor{blue}{+18.5\%}) & \underline{66.4} \textcolor{gray}{±0.1} (\textcolor{blue}{+31.7\%}) & \underline{64.7} \textcolor{gray}{±0.1} (\textcolor{blue}{+33.0\%}) & \underline{72.1} \textcolor{gray}{±0.1} (\textcolor{blue}{+23.3\%}) \\
\midrule
GenAtt & 80.4 \textcolor{gray}{±0.1} & 69.7 \textcolor{gray}{±0.1} & 61.9 \textcolor{gray}{±0.1} & 56.4 \textcolor{gray}{±0.1} & 67.1 \textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 81.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.4\%}) & 71.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.9\%}) & 65.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.1\%}) & 59.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.9\%}) & 69.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.6\%}) \\
\midrule
TokenTM & 78.8 \textcolor{gray}{±0.1} & 68.9 \textcolor{gray}{±0.1} & 60.6 \textcolor{gray}{±0.1} & 54.9 \textcolor{gray}{±0.1} & 65.8 \textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 79.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.4\%}) & 70.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.1\%}) & 62.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.6\%}) & 57.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+4.5\%}) & 67.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.7\%}) \\
\midrule
GradCAM+ & 70.5 \textcolor{gray}{±0.1} & 59.9 \textcolor{gray}{±0.1} & 50.5 \textcolor{gray}{±0.1} & 53.4 \textcolor{gray}{±0.1} & 58.6 \textcolor{gray}{±0.1} \\
\textbf{Libra GradCAM+} & 76.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+8.9\%}) & 70.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+17.0\%}) & 65.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+29.3\%}) & 60.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+14.0\%}) & 68.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+16.5\%}) \\
\midrule
HiResCAM & 48.0 \textcolor{gray}{±0.1} & 38.4 \textcolor{gray}{±0.1} & 50.4 \textcolor{gray}{±0.1} & 32.7 \textcolor{gray}{±0.1} & 42.4 \textcolor{gray}{±0.1} \\
\textbf{Libra HiResCAM} & 74.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+54.3\%}) & 67.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+75.5\%}) & 60.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+20.6\%}) & 54.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+65.2\%}) & 64.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+51.2\%}) \\
\midrule
XGradCAM+ & 71.7 \textcolor{gray}{±0.1} & 60.3 \textcolor{gray}{±0.1} & 44.0 \textcolor{gray}{±0.1} & 50.9 \textcolor{gray}{±0.1} & 56.7 \textcolor{gray}{±0.1} \\
\textbf{Libra XGradCAM+} & 80.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+12.4\%}) & 72.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+19.5\%}) & \textbf{67.4} \textcolor{gray}{±0.1} (\textcolor{blue}{+53.0\%}) & 63.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+23.6\%}) & 70.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+24.7\%}) \\
\midrule
FullGrad+ & 69.8 \textcolor{gray}{±0.1} & 59.6 \textcolor{gray}{±0.1} & 48.2 \textcolor{gray}{±0.1} & 49.1 \textcolor{gray}{±0.1} & 56.6 \textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & \textbf{84.2} \textcolor{gray}{±0.1} (\textcolor{blue}{+20.8\%}) & \underline{73.5} \textcolor{gray}{±0.1} (\textcolor{blue}{+23.3\%}) & 66.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+37.1\%}) & \textbf{65.5} \textcolor{gray}{±0.1} (\textcolor{blue}{+33.5\%}) & \textbf{72.3} \textcolor{gray}{±0.1} (\textcolor{blue}{+27.7\%}) \\
\bottomrule
\end{tabular}
\caption{How Most-Influential-First Deletion (MIF) Accuracy evaluated using ground-truth labels varies with different model sizes.}
\label{across_models_depth_MIF_gt_accuracy_m_2}
\end{table}


==> files/tables_v1/across_models/depth/SRG_1p_AOPC/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ViT-Tiny & ViT-Small & ViT-Base & ViT-Large & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 49.9 \textcolor{gray}{±0.2} & 50.2 \textcolor{gray}{±0.2} & 50.0 \textcolor{gray}{±0.2} & 49.8 \textcolor{gray}{±0.2} & 50.0 \textcolor{gray}{±0.2} \\
RawAtt & 65.2 \textcolor{gray}{±0.2} & 64.2 \textcolor{gray}{±0.3} & 57.8 \textcolor{gray}{±0.2} & 53.4 \textcolor{gray}{±0.2} & 60.1 \textcolor{gray}{±0.2} \\
Attention Rollout & 62.1 \textcolor{gray}{±0.2} & 55.6 \textcolor{gray}{±0.2} & 53.6 \textcolor{gray}{±0.2} & 50.1 \textcolor{gray}{±0.2} & 55.3 \textcolor{gray}{±0.2} \\
AliLRP & 66.0 \textcolor{gray}{±0.2} & 56.0 \textcolor{gray}{±0.3} & 54.2 \textcolor{gray}{±0.2} & 52.5 \textcolor{gray}{±0.2} & 57.2 \textcolor{gray}{±0.2} \\
AttnLRP & 68.8 \textcolor{gray}{±0.2} & 64.0 \textcolor{gray}{±0.2} & 57.1 \textcolor{gray}{±0.2} & 59.5 \textcolor{gray}{±0.2} & 62.3 \textcolor{gray}{±0.2} \\
DecompX & 69.0 \textcolor{gray}{±0.2} & 61.9 \textcolor{gray}{±0.2} & 56.7 \textcolor{gray}{±0.2} & 57.3 \textcolor{gray}{±0.2} & 61.2 \textcolor{gray}{±0.2} \\
Integrated Gradients & 61.1 \textcolor{gray}{±0.2} & 59.7 \textcolor{gray}{±0.3} & 56.3 \textcolor{gray}{±0.2} & 55.1 \textcolor{gray}{±0.2} & 58.1 \textcolor{gray}{±0.2} \\
\midrule
\IxG{}  & 60.0 \textcolor{gray}{±0.2} & 56.4 \textcolor{gray}{±0.3} & 55.2 \textcolor{gray}{±0.2} & 53.2 \textcolor{gray}{±0.2} & 56.2 \textcolor{gray}{±0.2} \\
\textbf{Libra \IxG{} } & 68.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+14.8\%}) & 60.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+8.0\%}) & 57.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+3.9\%}) & 58.2 \textcolor{gray}{±0.2} (\textcolor{blue}{+9.4\%}) & 61.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+9.1\%}) \\
\midrule
AttCAT & 68.6 \textcolor{gray}{±0.2} & 66.9 \textcolor{gray}{±0.2} & 62.7 \textcolor{gray}{±0.2} & 60.8 \textcolor{gray}{±0.2} & 64.8 \textcolor{gray}{±0.2} \\
\textbf{Libra AttCAT} & \underline{75.1} \textcolor{gray}{±0.2} (\textcolor{blue}{+9.4\%}) & \underline{73.3} \textcolor{gray}{±0.3} (\textcolor{blue}{+9.6\%}) & \textbf{70.4} \textcolor{gray}{±0.2} (\textcolor{blue}{+12.2\%}) & \underline{70.8} \textcolor{gray}{±0.2} (\textcolor{blue}{+16.4\%}) & \underline{72.4} \textcolor{gray}{±0.2} (\textcolor{blue}{+11.8\%}) \\
\midrule
GenAtt & 71.5 \textcolor{gray}{±0.2} & 69.6 \textcolor{gray}{±0.2} & 66.3 \textcolor{gray}{±0.2} & 64.0 \textcolor{gray}{±0.2} & 67.8 \textcolor{gray}{±0.2} \\
\textbf{Libra GenAtt} & 71.4 \textcolor{gray}{±0.2} (\textcolor{coral}{-0.1\%}) & 70.5 \textcolor{gray}{±0.3} (\textcolor{blue}{+1.2\%}) & 67.6 \textcolor{gray}{±0.2} (\textcolor{blue}{+2.1\%}) & 65.8 \textcolor{gray}{±0.3} (\textcolor{blue}{+2.8\%}) & 68.8 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.5\%}) \\
\midrule
TokenTM & 69.8 \textcolor{gray}{±0.2} & 68.3 \textcolor{gray}{±0.2} & 65.3 \textcolor{gray}{±0.2} & 62.6 \textcolor{gray}{±0.2} & 66.5 \textcolor{gray}{±0.2} \\
\textbf{Libra TokenTM} & 69.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.1\%}) & 69.1 \textcolor{gray}{±0.3} (\textcolor{blue}{+1.0\%}) & 66.2 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.3\%}) & 64.1 \textcolor{gray}{±0.3} (\textcolor{blue}{+2.4\%}) & 67.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.2\%}) \\
\midrule
GradCAM+ & 62.2 \textcolor{gray}{±0.2} & 62.0 \textcolor{gray}{±0.3} & 59.5 \textcolor{gray}{±0.2} & 62.0 \textcolor{gray}{±0.2} & 61.4 \textcolor{gray}{±0.2} \\
\textbf{Libra GradCAM+} & 68.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+9.3\%}) & 69.9 \textcolor{gray}{±0.3} (\textcolor{blue}{+12.8\%}) & 67.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+14.1\%}) & 66.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+7.2\%}) & 68.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+10.8\%}) \\
\midrule
HiResCAM & 45.4 \textcolor{gray}{±0.2} & 47.0 \textcolor{gray}{±0.3} & 60.1 \textcolor{gray}{±0.2} & 43.2 \textcolor{gray}{±0.2} & 48.9 \textcolor{gray}{±0.2} \\
\textbf{Libra HiResCAM} & 65.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+43.3\%}) & 67.7 \textcolor{gray}{±0.2} (\textcolor{blue}{+44.1\%}) & 65.7 \textcolor{gray}{±0.2} (\textcolor{blue}{+9.2\%}) & 60.6 \textcolor{gray}{±0.2} (\textcolor{blue}{+40.3\%}) & 64.8 \textcolor{gray}{±0.2} (\textcolor{blue}{+32.4\%}) \\
\midrule
XGradCAM+ & 63.8 \textcolor{gray}{±0.2} & 62.8 \textcolor{gray}{±0.3} & 54.1 \textcolor{gray}{±0.2} & 60.3 \textcolor{gray}{±0.2} & 60.3 \textcolor{gray}{±0.2} \\
\textbf{Libra XGradCAM+} & 70.7 \textcolor{gray}{±0.2} (\textcolor{blue}{+10.8\%}) & 71.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+12.9\%}) & 69.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+27.7\%}) & 68.0 \textcolor{gray}{±0.3} (\textcolor{blue}{+12.6\%}) & 69.7 \textcolor{gray}{±0.2} (\textcolor{blue}{+15.6\%}) \\
\midrule
FullGrad+ & 66.3 \textcolor{gray}{±0.2} & 65.2 \textcolor{gray}{±0.3} & 60.7 \textcolor{gray}{±0.2} & 60.4 \textcolor{gray}{±0.2} & 63.1 \textcolor{gray}{±0.2} \\
\textbf{Libra FullGrad+} & \textbf{76.0} \textcolor{gray}{±0.2} (\textcolor{blue}{+14.5\%}) & \textbf{73.4} \textcolor{gray}{±0.3} (\textcolor{blue}{+12.5\%}) & \textbf{70.4} \textcolor{gray}{±0.2} (\textcolor{blue}{+16.0\%}) & \textbf{71.3} \textcolor{gray}{±0.2} (\textcolor{blue}{+18.1\%}) & \textbf{72.8} \textcolor{gray}{±0.2} (\textcolor{blue}{+15.2\%}) \\
\bottomrule
\end{tabular}
\caption{How Symmetric Relevance Gain (SRG) AOPC evaluated using predicted labels varies with different model sizes.}
\label{across_models_depth_SRG_1p_AOPC_m_2}
\end{table}


==> files/tables_v1/across_models/depth/SRG_1p_accuracy/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ViT-Tiny & ViT-Small & ViT-Base & ViT-Large & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 49.6 \textcolor{gray}{±0.1} & 50.2 \textcolor{gray}{±0.1} & 49.9 \textcolor{gray}{±0.1} & 49.8 \textcolor{gray}{±0.1} & 49.9 \textcolor{gray}{±0.1} \\
RawAtt & 68.4 \textcolor{gray}{±0.1} & 65.8 \textcolor{gray}{±0.1} & 60.4 \textcolor{gray}{±0.1} & 53.3 \textcolor{gray}{±0.1} & 62.0 \textcolor{gray}{±0.1} \\
Attention Rollout & 64.8 \textcolor{gray}{±0.1} & 56.2 \textcolor{gray}{±0.1} & 54.6 \textcolor{gray}{±0.1} & 49.9 \textcolor{gray}{±0.1} & 56.3 \textcolor{gray}{±0.1} \\
AliLRP & 68.7 \textcolor{gray}{±0.1} & 56.5 \textcolor{gray}{±0.1} & 55.5 \textcolor{gray}{±0.1} & 52.8 \textcolor{gray}{±0.1} & 58.4 \textcolor{gray}{±0.1} \\
AttnLRP & 72.0 \textcolor{gray}{±0.1} & 64.9 \textcolor{gray}{±0.1} & 58.6 \textcolor{gray}{±0.1} & 59.7 \textcolor{gray}{±0.1} & 63.8 \textcolor{gray}{±0.1} \\
DecompX & 72.6 \textcolor{gray}{±0.1} & 62.9 \textcolor{gray}{±0.1} & 58.5 \textcolor{gray}{±0.1} & 57.4 \textcolor{gray}{±0.1} & 62.8 \textcolor{gray}{±0.1} \\
Integrated Gradients & 62.0 \textcolor{gray}{±0.1} & 59.9 \textcolor{gray}{±0.1} & 56.7 \textcolor{gray}{±0.1} & 54.7 \textcolor{gray}{±0.1} & 58.3 \textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 62.3 \textcolor{gray}{±0.1} & 57.0 \textcolor{gray}{±0.1} & 55.9 \textcolor{gray}{±0.1} & 53.3 \textcolor{gray}{±0.1} & 57.1 \textcolor{gray}{±0.1} \\
\textbf{Libra \IxG{} } & 72.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+16.8\%}) & 61.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+8.5\%}) & 59.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+6.3\%}) & 58.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+9.9\%}) & 63.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+10.6\%}) \\
\midrule
AttCAT & 72.0 \textcolor{gray}{±0.1} & 68.7 \textcolor{gray}{±0.1} & 64.7 \textcolor{gray}{±0.1} & 61.2 \textcolor{gray}{±0.1} & 66.7 \textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \underline{79.4} \textcolor{gray}{±0.1} (\textcolor{blue}{+10.2\%}) & \textbf{75.7} \textcolor{gray}{±0.1} (\textcolor{blue}{+10.1\%}) & \textbf{75.1} \textcolor{gray}{±0.1} (\textcolor{blue}{+16.1\%}) & \underline{71.8} \textcolor{gray}{±0.1} (\textcolor{blue}{+17.4\%}) & \underline{75.5} \textcolor{gray}{±0.1} (\textcolor{blue}{+13.2\%}) \\
\midrule
GenAtt & 76.6 \textcolor{gray}{±0.1} & 72.7 \textcolor{gray}{±0.1} & 71.1 \textcolor{gray}{±0.1} & 65.0 \textcolor{gray}{±0.1} & 71.4 \textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 76.5 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.2\%}) & 73.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.3\%}) & 73.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.6\%}) & 67.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.2\%}) & 72.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.6\%}) \\
\midrule
TokenTM & 74.6 \textcolor{gray}{±0.1} & 71.2 \textcolor{gray}{±0.1} & 70.0 \textcolor{gray}{±0.1} & 63.6 \textcolor{gray}{±0.1} & 69.8 \textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 75.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.5\%}) & 71.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.9\%}) & 71.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.7\%}) & 65.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.4\%}) & 70.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.3\%}) \\
\midrule
GradCAM+ & 65.7 \textcolor{gray}{±0.1} & 63.7 \textcolor{gray}{±0.1} & 62.0 \textcolor{gray}{±0.1} & 62.7 \textcolor{gray}{±0.1} & 63.5 \textcolor{gray}{±0.1} \\
\textbf{Libra GradCAM+} & 71.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+9.0\%}) & 72.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+13.3\%}) & 73.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+18.0\%}) & 67.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+8.1\%}) & 71.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+12.1\%}) \\
\midrule
HiResCAM & 43.7 \textcolor{gray}{±0.1} & 46.2 \textcolor{gray}{±0.1} & 62.5 \textcolor{gray}{±0.1} & 42.5 \textcolor{gray}{±0.1} & 48.7 \textcolor{gray}{±0.1} \\
\textbf{Libra HiResCAM} & 68.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+57.9\%}) & 69.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+51.1\%}) & 69.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+11.6\%}) & 61.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+44.4\%}) & 67.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+38.5\%}) \\
\midrule
XGradCAM+ & 67.1 \textcolor{gray}{±0.1} & 64.7 \textcolor{gray}{±0.1} & 55.9 \textcolor{gray}{±0.1} & 60.8 \textcolor{gray}{±0.1} & 62.1 \textcolor{gray}{±0.1} \\
\textbf{Libra XGradCAM+} & 74.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+11.6\%}) & 73.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+13.5\%}) & 74.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+33.5\%}) & 69.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+14.1\%}) & 73.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+17.6\%}) \\
\midrule
FullGrad+ & 69.7 \textcolor{gray}{±0.1} & 66.7 \textcolor{gray}{±0.1} & 62.9 \textcolor{gray}{±0.1} & 60.9 \textcolor{gray}{±0.1} & 65.0 \textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & \textbf{80.3} \textcolor{gray}{±0.1} (\textcolor{blue}{+15.2\%}) & \underline{75.6} \textcolor{gray}{±0.1} (\textcolor{blue}{+13.3\%}) & \underline{75.0} \textcolor{gray}{±0.1} (\textcolor{blue}{+19.4\%}) & \textbf{72.5} \textcolor{gray}{±0.1} (\textcolor{blue}{+19.0\%}) & \textbf{75.9} \textcolor{gray}{±0.1} (\textcolor{blue}{+16.6\%}) \\
\bottomrule
\end{tabular}
\caption{How Symmetric Relevance Gain (SRG) Accuracy evaluated using predicted labels varies with different model sizes.}
\label{across_models_depth_SRG_1p_accuracy_m_2}
\end{table}


==> files/tables_v1/across_models/depth/SRG_gt_AOPC/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ViT-Tiny & ViT-Small & ViT-Base & ViT-Large & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 49.9 \textcolor{gray}{±0.2} & 49.9 \textcolor{gray}{±0.3} & 49.9 \textcolor{gray}{±0.2} & 49.7 \textcolor{gray}{±0.2} & 49.9 \textcolor{gray}{±0.2} \\
RawAtt & 63.3 \textcolor{gray}{±0.3} & 63.0 \textcolor{gray}{±0.3} & 57.1 \textcolor{gray}{±0.2} & 53.1 \textcolor{gray}{±0.2} & 59.1 \textcolor{gray}{±0.2} \\
Attention Rollout & 60.4 \textcolor{gray}{±0.3} & 54.9 \textcolor{gray}{±0.3} & 53.3 \textcolor{gray}{±0.2} & 50.3 \textcolor{gray}{±0.3} & 54.8 \textcolor{gray}{±0.3} \\
AliLRP & 64.2 \textcolor{gray}{±0.3} & 55.5 \textcolor{gray}{±0.3} & 53.8 \textcolor{gray}{±0.2} & 52.4 \textcolor{gray}{±0.2} & 56.5 \textcolor{gray}{±0.3} \\
AttnLRP & 66.7 \textcolor{gray}{±0.3} & 62.8 \textcolor{gray}{±0.3} & 56.6 \textcolor{gray}{±0.2} & 58.8 \textcolor{gray}{±0.3} & 61.2 \textcolor{gray}{±0.3} \\
DecompX & 66.8 \textcolor{gray}{±0.3} & 60.9 \textcolor{gray}{±0.3} & 56.3 \textcolor{gray}{±0.2} & 56.8 \textcolor{gray}{±0.3} & 60.2 \textcolor{gray}{±0.3} \\
Integrated Gradients & 64.6 \textcolor{gray}{±0.3} & 62.3 \textcolor{gray}{±0.3} & 59.1 \textcolor{gray}{±0.2} & 58.2 \textcolor{gray}{±0.3} & 61.0 \textcolor{gray}{±0.3} \\
\midrule
\IxG{}  & 58.5 \textcolor{gray}{±0.2} & 55.8 \textcolor{gray}{±0.3} & 54.8 \textcolor{gray}{±0.2} & 53.0 \textcolor{gray}{±0.2} & 55.5 \textcolor{gray}{±0.2} \\
\textbf{Libra \IxG{} } & 67.0 \textcolor{gray}{±0.3} (\textcolor{blue}{+14.4\%}) & 60.1 \textcolor{gray}{±0.3} (\textcolor{blue}{+7.6\%}) & 56.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+4.0\%}) & 57.7 \textcolor{gray}{±0.3} (\textcolor{blue}{+8.9\%}) & 60.4 \textcolor{gray}{±0.3} (\textcolor{blue}{+8.8\%}) \\
\midrule
AttCAT & 66.8 \textcolor{gray}{±0.3} & 65.5 \textcolor{gray}{±0.3} & 61.9 \textcolor{gray}{±0.2} & 60.0 \textcolor{gray}{±0.2} & 63.5 \textcolor{gray}{±0.2} \\
\textbf{Libra AttCAT} & \underline{72.9} \textcolor{gray}{±0.2} (\textcolor{blue}{+9.2\%}) & \underline{71.9} \textcolor{gray}{±0.3} (\textcolor{blue}{+9.8\%}) & \underline{69.1} \textcolor{gray}{±0.2} (\textcolor{blue}{+11.7\%}) & \underline{69.5} \textcolor{gray}{±0.3} (\textcolor{blue}{+15.8\%}) & \underline{70.9} \textcolor{gray}{±0.3} (\textcolor{blue}{+11.5\%}) \\
\midrule
GenAtt & 69.1 \textcolor{gray}{±0.2} & 68.0 \textcolor{gray}{±0.3} & 65.0 \textcolor{gray}{±0.2} & 63.0 \textcolor{gray}{±0.2} & 66.2 \textcolor{gray}{±0.2} \\
\textbf{Libra GenAtt} & 69.0 \textcolor{gray}{±0.2} (\textcolor{coral}{-0.1\%}) & 68.8 \textcolor{gray}{±0.3} (\textcolor{blue}{+1.3\%}) & 66.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+2.0\%}) & 64.7 \textcolor{gray}{±0.3} (\textcolor{blue}{+2.7\%}) & 67.2 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.4\%}) \\
\midrule
TokenTM & 67.6 \textcolor{gray}{±0.2} & 66.8 \textcolor{gray}{±0.3} & 64.1 \textcolor{gray}{±0.2} & 61.7 \textcolor{gray}{±0.3} & 65.0 \textcolor{gray}{±0.3} \\
\textbf{Libra TokenTM} & 67.7 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.1\%}) & 67.5 \textcolor{gray}{±0.3} (\textcolor{blue}{+1.1\%}) & 64.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.2\%}) & 63.1 \textcolor{gray}{±0.3} (\textcolor{blue}{+2.3\%}) & 65.8 \textcolor{gray}{±0.3} (\textcolor{blue}{+1.2\%}) \\
\midrule
GradCAM+ & 61.4 \textcolor{gray}{±0.3} & 61.0 \textcolor{gray}{±0.3} & 59.2 \textcolor{gray}{±0.2} & 61.5 \textcolor{gray}{±0.3} & 60.8 \textcolor{gray}{±0.3} \\
\textbf{Libra GradCAM+} & 66.6 \textcolor{gray}{±0.3} (\textcolor{blue}{+8.4\%}) & 68.6 \textcolor{gray}{±0.3} (\textcolor{blue}{+12.4\%}) & 67.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+13.3\%}) & 65.5 \textcolor{gray}{±0.3} (\textcolor{blue}{+6.6\%}) & 66.9 \textcolor{gray}{±0.3} (\textcolor{blue}{+10.2\%}) \\
\midrule
HiResCAM & 46.2 \textcolor{gray}{±0.3} & 47.4 \textcolor{gray}{±0.3} & 59.3 \textcolor{gray}{±0.2} & 43.6 \textcolor{gray}{±0.2} & 49.2 \textcolor{gray}{±0.3} \\
\textbf{Libra HiResCAM} & 64.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+38.4\%}) & 66.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+40.0\%}) & 64.7 \textcolor{gray}{±0.2} (\textcolor{blue}{+9.1\%}) & 60.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+37.7\%}) & 63.8 \textcolor{gray}{±0.2} (\textcolor{blue}{+29.8\%}) \\
\midrule
XGradCAM+ & 62.8 \textcolor{gray}{±0.3} & 61.9 \textcolor{gray}{±0.3} & 53.9 \textcolor{gray}{±0.2} & 59.9 \textcolor{gray}{±0.3} & 59.6 \textcolor{gray}{±0.3} \\
\textbf{Libra XGradCAM+} & 69.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+10.1\%}) & 69.7 \textcolor{gray}{±0.3} (\textcolor{blue}{+12.6\%}) & 68.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+26.2\%}) & 66.9 \textcolor{gray}{±0.3} (\textcolor{blue}{+11.8\%}) & 68.4 \textcolor{gray}{±0.3} (\textcolor{blue}{+14.8\%}) \\
\midrule
FullGrad+ & 64.7 \textcolor{gray}{±0.3} & 63.9 \textcolor{gray}{±0.3} & 59.8 \textcolor{gray}{±0.2} & 59.8 \textcolor{gray}{±0.2} & 62.1 \textcolor{gray}{±0.3} \\
\textbf{Libra FullGrad+} & \textbf{73.7} \textcolor{gray}{±0.2} (\textcolor{blue}{+13.9\%}) & \textbf{72.0} \textcolor{gray}{±0.3} (\textcolor{blue}{+12.6\%}) & \textbf{69.2} \textcolor{gray}{±0.2} (\textcolor{blue}{+15.6\%}) & \textbf{70.0} \textcolor{gray}{±0.3} (\textcolor{blue}{+17.1\%}) & \textbf{71.2} \textcolor{gray}{±0.3} (\textcolor{blue}{+14.7\%}) \\
\bottomrule
\end{tabular}
\caption{How Symmetric Relevance Gain (SRG) AOPC evaluated using ground-truth labels varies with different model sizes.}
\label{across_models_depth_SRG_gt_AOPC_m_2}
\end{table}


==> files/tables_v1/across_models/depth/SRG_gt_accuracy/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ViT-Tiny & ViT-Small & ViT-Base & ViT-Large & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 49.6 \textcolor{gray}{±0.1} & 49.7 \textcolor{gray}{±0.1} & 49.9 \textcolor{gray}{±0.1} & 49.9 \textcolor{gray}{±0.1} & 49.8 \textcolor{gray}{±0.1} \\
RawAtt & 64.6 \textcolor{gray}{±0.1} & 63.5 \textcolor{gray}{±0.1} & 58.8 \textcolor{gray}{±0.1} & 52.9 \textcolor{gray}{±0.1} & 60.0 \textcolor{gray}{±0.1} \\
Attention Rollout & 61.6 \textcolor{gray}{±0.1} & 54.9 \textcolor{gray}{±0.1} & 53.9 \textcolor{gray}{±0.1} & 50.4 \textcolor{gray}{±0.1} & 55.2 \textcolor{gray}{±0.1} \\
AliLRP & 66.0 \textcolor{gray}{±0.1} & 55.7 \textcolor{gray}{±0.1} & 54.8 \textcolor{gray}{±0.1} & 52.6 \textcolor{gray}{±0.1} & 57.3 \textcolor{gray}{±0.1} \\
AttnLRP & 68.3 \textcolor{gray}{±0.1} & 63.0 \textcolor{gray}{±0.1} & 57.8 \textcolor{gray}{±0.1} & 58.7 \textcolor{gray}{±0.1} & 62.0 \textcolor{gray}{±0.1} \\
DecompX & 68.6 \textcolor{gray}{±0.1} & 61.3 \textcolor{gray}{±0.1} & 57.6 \textcolor{gray}{±0.1} & 56.6 \textcolor{gray}{±0.1} & 61.0 \textcolor{gray}{±0.1} \\
Integrated Gradients & 66.8 \textcolor{gray}{±0.1} & 63.3 \textcolor{gray}{±0.1} & 60.6 \textcolor{gray}{±0.1} & 58.7 \textcolor{gray}{±0.1} & 62.4 \textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 59.8 \textcolor{gray}{±0.1} & 56.1 \textcolor{gray}{±0.1} & 55.1 \textcolor{gray}{±0.1} & 53.0 \textcolor{gray}{±0.1} & 56.0 \textcolor{gray}{±0.1} \\
\textbf{Libra \IxG{} } & 69.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+16.8\%}) & 60.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+8.2\%}) & 58.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+6.3\%}) & 58.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+9.5\%}) & 61.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+10.3\%}) \\
\midrule
AttCAT & 69.5 \textcolor{gray}{±0.1} & 67.0 \textcolor{gray}{±0.1} & 63.6 \textcolor{gray}{±0.1} & 60.2 \textcolor{gray}{±0.1} & 65.1 \textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \underline{76.5} \textcolor{gray}{±0.1} (\textcolor{blue}{+10.1\%}) & \underline{73.9} \textcolor{gray}{±0.1} (\textcolor{blue}{+10.3\%}) & \textbf{73.3} \textcolor{gray}{±0.1} (\textcolor{blue}{+15.3\%}) & \underline{70.5} \textcolor{gray}{±0.1} (\textcolor{blue}{+17.0\%}) & \underline{73.6} \textcolor{gray}{±0.1} (\textcolor{blue}{+13.0\%}) \\
\midrule
GenAtt & 72.0 \textcolor{gray}{±0.1} & 69.6 \textcolor{gray}{±0.1} & 68.4 \textcolor{gray}{±0.1} & 63.2 \textcolor{gray}{±0.1} & 68.3 \textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 71.9 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.1\%}) & 70.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.4\%}) & 70.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.5\%}) & 65.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.3\%}) & 69.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.7\%}) \\
\midrule
TokenTM & 70.0 \textcolor{gray}{±0.1} & 68.2 \textcolor{gray}{±0.1} & 67.1 \textcolor{gray}{±0.1} & 61.9 \textcolor{gray}{±0.1} & 66.8 \textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 70.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.5\%}) & 68.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.0\%}) & 68.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.7\%}) & 63.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.4\%}) & 67.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.4\%}) \\
\midrule
GradCAM+ & 64.2 \textcolor{gray}{±0.1} & 62.5 \textcolor{gray}{±0.1} & 61.3 \textcolor{gray}{±0.1} & 62.0 \textcolor{gray}{±0.1} & 62.5 \textcolor{gray}{±0.1} \\
\textbf{Libra GradCAM+} & 69.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+8.0\%}) & 70.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+12.8\%}) & 71.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+17.0\%}) & 66.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+7.7\%}) & 69.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+11.3\%}) \\
\midrule
HiResCAM & 45.2 \textcolor{gray}{±0.1} & 47.1 \textcolor{gray}{±0.1} & 61.2 \textcolor{gray}{±0.1} & 43.2 \textcolor{gray}{±0.1} & 49.2 \textcolor{gray}{±0.1} \\
\textbf{Libra HiResCAM} & 67.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+48.3\%}) & 68.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+44.2\%}) & 68.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+11.5\%}) & 60.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+40.7\%}) & 66.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+34.2\%}) \\
\midrule
XGradCAM+ & 65.6 \textcolor{gray}{±0.1} & 63.3 \textcolor{gray}{±0.1} & 55.5 \textcolor{gray}{±0.1} & 60.2 \textcolor{gray}{±0.1} & 61.2 \textcolor{gray}{±0.1} \\
\textbf{Libra XGradCAM+} & 72.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+10.5\%}) & 71.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+13.3\%}) & 72.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+31.0\%}) & 68.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+13.3\%}) & 71.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+16.6\%}) \\
\midrule
FullGrad+ & 67.1 \textcolor{gray}{±0.1} & 65.0 \textcolor{gray}{±0.1} & 61.7 \textcolor{gray}{±0.1} & 60.3 \textcolor{gray}{±0.1} & 63.5 \textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & \textbf{77.2} \textcolor{gray}{±0.1} (\textcolor{blue}{+15.0\%}) & \textbf{74.0} \textcolor{gray}{±0.1} (\textcolor{blue}{+13.9\%}) & \textbf{73.3} \textcolor{gray}{±0.1} (\textcolor{blue}{+18.8\%}) & \textbf{71.2} \textcolor{gray}{±0.1} (\textcolor{blue}{+18.1\%}) & \textbf{73.9} \textcolor{gray}{±0.1} (\textcolor{blue}{+16.4\%}) \\
\bottomrule
\end{tabular}
\caption{How Symmetric Relevance Gain (SRG) Accuracy evaluated using ground-truth labels varies with different model sizes.}
\label{across_models_depth_SRG_gt_accuracy_m_2}
\end{table}


==> files/tables_v1/across_models/ds/LIF_1p_AOPC/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ImageNet & ImageNet-Hard & MURA & Oxford-IIIT Pet & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 85.8 \textcolor{gray}{±0.2} & 83.1 \textcolor{gray}{±0.2} & 96.2 \textcolor{gray}{±0.1} & 95.4 \textcolor{gray}{±0.1} & 90.1 \textcolor{gray}{±0.2} \\
RawAtt & 87.6 \textcolor{gray}{±0.1} & 85.5 \textcolor{gray}{±0.2} & 96.6 \textcolor{gray}{±0.1} & 96.1 \textcolor{gray}{±0.1} & 91.5 \textcolor{gray}{±0.1} \\
Attention Rollout & 86.0 \textcolor{gray}{±0.2} & 84.1 \textcolor{gray}{±0.2} & 94.9 \textcolor{gray}{±0.1} & 91.7 \textcolor{gray}{±0.2} & 89.2 \textcolor{gray}{±0.2} \\
AliLRP & 89.3 \textcolor{gray}{±0.2} & 87.3 \textcolor{gray}{±0.2} & 98.5 \textcolor{gray}{±0.1} & 98.0 \textcolor{gray}{±0.1} & 93.3 \textcolor{gray}{±0.2} \\
AttnLRP & 90.8 \textcolor{gray}{±0.1} & 93.4 \textcolor{gray}{±0.2} & 98.7 \textcolor{gray}{±0.1} & 99.4 \textcolor{gray}{±0.1} & 95.6 \textcolor{gray}{±0.1} \\
DecompX & 90.6 \textcolor{gray}{±0.1} & 89.4 \textcolor{gray}{±0.2} & 99.4 \textcolor{gray}{±0.1} & 98.3 \textcolor{gray}{±0.1} & 94.4 \textcolor{gray}{±0.2} \\
Integrated Gradients & 91.3 \textcolor{gray}{±0.1} & 89.7 \textcolor{gray}{±0.2} & 99.2 \textcolor{gray}{±0.1} & 97.5 \textcolor{gray}{±0.1} & 94.4 \textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 90.2 \textcolor{gray}{±0.1} & 89.9 \textcolor{gray}{±0.2} & 100.5 \textcolor{gray}{±0.1} & 99.4 \textcolor{gray}{±0.1} & 95.0 \textcolor{gray}{±0.2} \\
\textbf{Libra \IxG{} } & 91.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.2\%}) & 90.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.2\%}) & 99.4 \textcolor{gray}{±0.1} (\textcolor{coral}{-1.1\%}) & 98.7 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.7\%}) & 94.9 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.1\%}) \\
\midrule
AttCAT & 96.6 \textcolor{gray}{±0.2} & 102.1 \textcolor{gray}{±0.2} & 102.1 \textcolor{gray}{±0.1} & \underline{100.9} \textcolor{gray}{±0.1} & 100.4 \textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \underline{99.2} \textcolor{gray}{±0.1} (\textcolor{blue}{+2.7\%}) & \underline{105.6} \textcolor{gray}{±0.2} (\textcolor{blue}{+3.5\%}) & 102.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.2\%}) & 100.8 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.1\%}) & \underline{102.0} \textcolor{gray}{±0.1} (\textcolor{blue}{+1.6\%}) \\
\midrule
GenAtt & 94.6 \textcolor{gray}{±0.1} & 93.4 \textcolor{gray}{±0.2} & 99.3 \textcolor{gray}{±0.1} & 99.2 \textcolor{gray}{±0.1} & 96.6 \textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 94.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.2\%}) & 93.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.1\%}) & 99.2 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.1\%}) & 98.6 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.6\%}) & 96.5 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.1\%}) \\
\midrule
TokenTM & 93.3 \textcolor{gray}{±0.1} & 91.1 \textcolor{gray}{±0.2} & 98.2 \textcolor{gray}{±0.1} & 98.7 \textcolor{gray}{±0.1} & 95.3 \textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 93.5 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.2\%}) & 91.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.2\%}) & 98.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.1\%}) & 98.3 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.5\%}) & 95.3 \textcolor{gray}{±0.1} (+0.0\%) \\
\midrule
GradCAM+ & 91.5 \textcolor{gray}{±0.2} & 93.9 \textcolor{gray}{±0.2} & 96.9 \textcolor{gray}{±0.2} & 94.1 \textcolor{gray}{±0.2} & 94.1 \textcolor{gray}{±0.2} \\
\textbf{Libra GradCAM+} & 96.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.2\%}) & 98.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+4.6\%}) & 100.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.8\%}) & 99.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.3\%}) & 98.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+4.7\%}) \\
\midrule
HiResCAM & 91.7 \textcolor{gray}{±0.2} & 90.6 \textcolor{gray}{±0.2} & 97.6 \textcolor{gray}{±0.1} & 90.9 \textcolor{gray}{±0.2} & 92.7 \textcolor{gray}{±0.2} \\
\textbf{Libra HiResCAM} & 94.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.8\%}) & 93.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+3.0\%}) & 99.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.3\%}) & 96.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+5.9\%}) & 95.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.5\%}) \\
\midrule
XGradCAM+ & 86.6 \textcolor{gray}{±0.2} & 92.5 \textcolor{gray}{±0.2} & 97.0 \textcolor{gray}{±0.1} & 95.5 \textcolor{gray}{±0.2} & 92.9 \textcolor{gray}{±0.2} \\
\textbf{Libra XGradCAM+} & 96.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+11.6\%}) & 99.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+7.1\%}) & 100.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.5\%}) & 99.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+4.2\%}) & 98.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+6.5\%}) \\
\midrule
FullGrad+ & 95.0 \textcolor{gray}{±0.2} & 99.8 \textcolor{gray}{±0.2} & \textbf{102.7} \textcolor{gray}{±0.1} & 100.8 \textcolor{gray}{±0.1} & 99.6 \textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & \textbf{99.6} \textcolor{gray}{±0.1} (\textcolor{blue}{+4.8\%}) & \textbf{106.3} \textcolor{gray}{±0.2} (\textcolor{blue}{+6.5\%}) & \textbf{102.7} \textcolor{gray}{±0.1} (+0.0\%) & \textbf{101.1} \textcolor{gray}{±0.1} (\textcolor{blue}{+0.3\%}) & \textbf{102.4} \textcolor{gray}{±0.1} (\textcolor{blue}{+2.8\%}) \\
\bottomrule
\end{tabular}
\caption{Cross-dataset analysis of Least-Influential-First Deletion (LIF) AOPC evaluated using predicted labels on ViT-B.}
\label{across_models_ds_LIF_1p_AOPC_m_2}
\end{table}


==> files/tables_v1/across_models/ds/LIF_1p_accuracy/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ImageNet & ImageNet-Hard & MURA & Oxford-IIIT Pet & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 73.3 \textcolor{gray}{±0.1} & 47.0 \textcolor{gray}{±0.1} & 85.8 \textcolor{gray}{±0.1} & 85.8 \textcolor{gray}{±0.1} & 72.9 \textcolor{gray}{±0.1} \\
RawAtt & 76.2 \textcolor{gray}{±0.1} & 52.0 \textcolor{gray}{±0.1} & 85.7 \textcolor{gray}{±0.1} & 86.0 \textcolor{gray}{±0.1} & 75.0 \textcolor{gray}{±0.1} \\
Attention Rollout & 73.8 \textcolor{gray}{±0.1} & 49.8 \textcolor{gray}{±0.1} & 84.1 \textcolor{gray}{±0.1} & 82.4 \textcolor{gray}{±0.1} & 72.5 \textcolor{gray}{±0.1} \\
AliLRP & 77.8 \textcolor{gray}{±0.1} & 53.5 \textcolor{gray}{±0.1} & 87.0 \textcolor{gray}{±0.1} & 87.7 \textcolor{gray}{±0.0} & 76.5 \textcolor{gray}{±0.1} \\
AttnLRP & 78.7 \textcolor{gray}{±0.1} & 61.6 \textcolor{gray}{±0.1} & 87.0 \textcolor{gray}{±0.1} & 88.7 \textcolor{gray}{±0.0} & 79.0 \textcolor{gray}{±0.1} \\
DecompX & 79.1 \textcolor{gray}{±0.1} & 56.8 \textcolor{gray}{±0.1} & 87.7 \textcolor{gray}{±0.0} & 88.1 \textcolor{gray}{±0.0} & 77.9 \textcolor{gray}{±0.1} \\
Integrated Gradients & 78.0 \textcolor{gray}{±0.1} & 54.2 \textcolor{gray}{±0.1} & 86.3 \textcolor{gray}{±0.1} & 87.0 \textcolor{gray}{±0.1} & 76.4 \textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 77.3 \textcolor{gray}{±0.1} & 55.9 \textcolor{gray}{±0.1} & 88.2 \textcolor{gray}{±0.0} & 88.7 \textcolor{gray}{±0.0} & 77.5 \textcolor{gray}{±0.1} \\
\textbf{Libra \IxG{} } & 80.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.8\%}) & 57.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.5\%}) & 87.7 \textcolor{gray}{±0.0} (\textcolor{coral}{-0.5\%}) & 88.3 \textcolor{gray}{±0.0} (\textcolor{coral}{-0.5\%}) & 78.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.3\%}) \\
\midrule
AttCAT & 82.5 \textcolor{gray}{±0.1} & 69.2 \textcolor{gray}{±0.1} & 89.1 \textcolor{gray}{±0.0} & \underline{89.3} \textcolor{gray}{±0.0} & 82.5 \textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \underline{86.7} \textcolor{gray}{±0.1} (\textcolor{blue}{+5.1\%}) & \underline{75.9} \textcolor{gray}{±0.1} (\textcolor{blue}{+9.5\%}) & 89.4 \textcolor{gray}{±0.0} (\textcolor{blue}{+0.3\%}) & \underline{89.3} \textcolor{gray}{±0.0} (+0.0\%) & \underline{85.3} \textcolor{gray}{±0.1} (\textcolor{blue}{+3.4\%}) \\
\midrule
GenAtt & 84.0 \textcolor{gray}{±0.1} & 65.7 \textcolor{gray}{±0.1} & 88.3 \textcolor{gray}{±0.0} & 88.7 \textcolor{gray}{±0.0} & 81.7 \textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 84.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.4\%}) & 66.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.1\%}) & 88.3 \textcolor{gray}{±0.0} (\textcolor{blue}{+0.1\%}) & 88.4 \textcolor{gray}{±0.0} (\textcolor{coral}{-0.3\%}) & 81.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.2\%}) \\
\midrule
TokenTM & 83.1 \textcolor{gray}{±0.1} & 62.9 \textcolor{gray}{±0.1} & 87.4 \textcolor{gray}{±0.1} & 88.4 \textcolor{gray}{±0.0} & 80.4 \textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 83.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.1\%}) & 63.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.3\%}) & 87.5 \textcolor{gray}{±0.0} (\textcolor{blue}{+0.2\%}) & 88.2 \textcolor{gray}{±0.0} (\textcolor{coral}{-0.3\%}) & 80.5 \textcolor{gray}{±0.1} (+0.0\%) \\
\midrule
GradCAM+ & 78.5 \textcolor{gray}{±0.1} & 61.2 \textcolor{gray}{±0.1} & 85.9 \textcolor{gray}{±0.1} & 84.2 \textcolor{gray}{±0.1} & 77.4 \textcolor{gray}{±0.1} \\
\textbf{Libra GradCAM+} & 84.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+8.3\%}) & 68.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+12.2\%}) & 88.6 \textcolor{gray}{±0.0} (\textcolor{blue}{+3.1\%}) & 88.4 \textcolor{gray}{±0.0} (\textcolor{blue}{+5.0\%}) & 82.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+6.7\%}) \\
\midrule
HiResCAM & 79.5 \textcolor{gray}{±0.1} & 57.7 \textcolor{gray}{±0.1} & 86.1 \textcolor{gray}{±0.1} & 81.6 \textcolor{gray}{±0.1} & 76.2 \textcolor{gray}{±0.1} \\
\textbf{Libra HiResCAM} & 82.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+4.0\%}) & 62.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+7.6\%}) & 87.8 \textcolor{gray}{±0.0} (\textcolor{blue}{+1.9\%}) & 86.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.7\%}) & 79.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+4.5\%}) \\
\midrule
XGradCAM+ & 73.3 \textcolor{gray}{±0.1} & 58.9 \textcolor{gray}{±0.1} & 85.8 \textcolor{gray}{±0.1} & 85.2 \textcolor{gray}{±0.1} & 75.8 \textcolor{gray}{±0.1} \\
\textbf{Libra XGradCAM+} & 85.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+16.6\%}) & 69.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+18.5\%}) & 88.2 \textcolor{gray}{±0.0} (\textcolor{blue}{+2.8\%}) & 88.6 \textcolor{gray}{±0.0} (\textcolor{blue}{+4.0\%}) & 83.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+9.5\%}) \\
\midrule
FullGrad+ & 81.6 \textcolor{gray}{±0.1} & 67.3 \textcolor{gray}{±0.1} & \textbf{89.5} \textcolor{gray}{±0.0} & \underline{89.3} \textcolor{gray}{±0.0} & 81.9 \textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & \textbf{87.0} \textcolor{gray}{±0.0} (\textcolor{blue}{+6.6\%}) & \textbf{76.2} \textcolor{gray}{±0.1} (\textcolor{blue}{+13.4\%}) & \textbf{89.5} \textcolor{gray}{±0.0} (+0.0\%) & \textbf{89.6} \textcolor{gray}{±0.0} (\textcolor{blue}{+0.3\%}) & \textbf{85.6} \textcolor{gray}{±0.1} (\textcolor{blue}{+4.5\%}) \\
\bottomrule
\end{tabular}
\caption{Cross-dataset analysis of Least-Influential-First Deletion (LIF) Accuracy evaluated using predicted labels on ViT-B.}
\label{across_models_ds_LIF_1p_accuracy_m_2}
\end{table}


==> files/tables_v1/across_models/ds/LIF_gt_AOPC/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ImageNet & ImageNet-Hard & MURA & Oxford-IIIT Pet & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 87.5 \textcolor{gray}{±0.2} & 93.5 \textcolor{gray}{±0.1} & 97.0 \textcolor{gray}{±0.1} & 95.6 \textcolor{gray}{±0.1} & 93.4 \textcolor{gray}{±0.2} \\
RawAtt & 89.2 \textcolor{gray}{±0.1} & 94.2 \textcolor{gray}{±0.1} & 97.7 \textcolor{gray}{±0.1} & 96.3 \textcolor{gray}{±0.2} & 94.4 \textcolor{gray}{±0.1} \\
Attention Rollout & 87.9 \textcolor{gray}{±0.2} & 94.0 \textcolor{gray}{±0.1} & 96.4 \textcolor{gray}{±0.1} & 92.0 \textcolor{gray}{±0.2} & 92.6 \textcolor{gray}{±0.2} \\
AliLRP & 90.9 \textcolor{gray}{±0.2} & 95.2 \textcolor{gray}{±0.1} & 99.9 \textcolor{gray}{±0.1} & 98.3 \textcolor{gray}{±0.1} & 96.1 \textcolor{gray}{±0.2} \\
AttnLRP & 92.4 \textcolor{gray}{±0.2} & 98.2 \textcolor{gray}{±0.1} & 100.4 \textcolor{gray}{±0.1} & 99.7 \textcolor{gray}{±0.1} & 97.7 \textcolor{gray}{±0.1} \\
DecompX & 92.2 \textcolor{gray}{±0.2} & 96.2 \textcolor{gray}{±0.1} & 100.9 \textcolor{gray}{±0.1} & 98.4 \textcolor{gray}{±0.1} & 96.9 \textcolor{gray}{±0.1} \\
Integrated Gradients & 95.7 \textcolor{gray}{±0.2} & 99.7 \textcolor{gray}{±0.1} & 103.7 \textcolor{gray}{±0.1} & 100.0 \textcolor{gray}{±0.1} & 99.8 \textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 91.8 \textcolor{gray}{±0.2} & 96.6 \textcolor{gray}{±0.1} & 102.6 \textcolor{gray}{±0.1} & 99.9 \textcolor{gray}{±0.1} & 97.7 \textcolor{gray}{±0.1} \\
\textbf{Libra \IxG{} } & 93.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.4\%}) & 96.5 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.1\%}) & 100.9 \textcolor{gray}{±0.1} (\textcolor{coral}{-1.7\%}) & 99.0 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.8\%}) & 97.4 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.4\%}) \\
\midrule
AttCAT & 98.4 \textcolor{gray}{±0.2} & 104.1 \textcolor{gray}{±0.1} & 105.0 \textcolor{gray}{±0.1} & \underline{101.4} \textcolor{gray}{±0.1} & 102.2 \textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \underline{100.8} \textcolor{gray}{±0.2} (\textcolor{blue}{+2.4\%}) & \underline{104.4} \textcolor{gray}{±0.2} (\textcolor{blue}{+0.4\%}) & \underline{105.7} \textcolor{gray}{±0.2} (\textcolor{blue}{+0.7\%}) & 101.3 \textcolor{gray}{±0.1} (+0.0\%) & \underline{103.1} \textcolor{gray}{±0.1} (\textcolor{blue}{+0.8\%}) \\
\midrule
GenAtt & 95.7 \textcolor{gray}{±0.2} & 97.8 \textcolor{gray}{±0.1} & 100.4 \textcolor{gray}{±0.1} & 99.4 \textcolor{gray}{±0.1} & 98.4 \textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 96.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.3\%}) & 97.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.1\%}) & 100.3 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.1\%}) & 98.9 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.6\%}) & 98.3 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.1\%}) \\
\midrule
TokenTM & 94.4 \textcolor{gray}{±0.1} & 96.9 \textcolor{gray}{±0.1} & 99.1 \textcolor{gray}{±0.1} & 99.0 \textcolor{gray}{±0.1} & 97.4 \textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 94.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.2\%}) & 97.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.1\%}) & 99.1 \textcolor{gray}{±0.1} (+0.0\%) & 98.5 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.4\%}) & 97.3 \textcolor{gray}{±0.1} (+0.0\%) \\
\midrule
GradCAM+ & 93.5 \textcolor{gray}{±0.2} & 98.8 \textcolor{gray}{±0.1} & 98.7 \textcolor{gray}{±0.2} & 94.6 \textcolor{gray}{±0.2} & 96.4 \textcolor{gray}{±0.2} \\
\textbf{Libra GradCAM+} & 98.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+4.9\%}) & 100.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.6\%}) & 103.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+4.3\%}) & 99.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.3\%}) & 100.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+4.0\%}) \\
\midrule
HiResCAM & 93.3 \textcolor{gray}{±0.2} & 97.1 \textcolor{gray}{±0.1} & 99.0 \textcolor{gray}{±0.2} & 91.4 \textcolor{gray}{±0.2} & 95.2 \textcolor{gray}{±0.2} \\
\textbf{Libra HiResCAM} & 96.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+3.0\%}) & 98.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.2\%}) & 102.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.1\%}) & 96.6 \textcolor{gray}{±0.2} (\textcolor{blue}{+5.7\%}) & 98.2 \textcolor{gray}{±0.2} (\textcolor{blue}{+3.2\%}) \\
\midrule
XGradCAM+ & 88.9 \textcolor{gray}{±0.3} & 98.3 \textcolor{gray}{±0.1} & 98.7 \textcolor{gray}{±0.2} & 96.0 \textcolor{gray}{±0.2} & 95.4 \textcolor{gray}{±0.2} \\
\textbf{Libra XGradCAM+} & 98.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+10.8\%}) & 100.7 \textcolor{gray}{±0.2} (\textcolor{blue}{+2.5\%}) & 103.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+4.8\%}) & 100.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+4.2\%}) & 100.6 \textcolor{gray}{±0.2} (\textcolor{blue}{+5.4\%}) \\
\midrule
FullGrad+ & 96.6 \textcolor{gray}{±0.2} & 102.0 \textcolor{gray}{±0.1} & \underline{105.7} \textcolor{gray}{±0.1} & 101.2 \textcolor{gray}{±0.1} & 101.4 \textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & \textbf{101.2} \textcolor{gray}{±0.2} (\textcolor{blue}{+4.8\%}) & \textbf{104.7} \textcolor{gray}{±0.1} (\textcolor{blue}{+2.7\%}) & \textbf{106.3} \textcolor{gray}{±0.2} (\textcolor{blue}{+0.5\%}) & \textbf{101.5} \textcolor{gray}{±0.1} (\textcolor{blue}{+0.3\%}) & \textbf{103.4} \textcolor{gray}{±0.1} (\textcolor{blue}{+2.0\%}) \\
\bottomrule
\end{tabular}
\caption{Cross-dataset analysis of Least-Influential-First Deletion (LIF) AOPC evaluated using ground-truth labels on ViT-B.}
\label{across_models_ds_LIF_gt_AOPC_m_2}
\end{table}


==> files/tables_v1/across_models/ds/LIF_gt_accuracy/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ImageNet & ImageNet-Hard & MURA & Oxford-IIIT Pet & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 65.2 \textcolor{gray}{±0.1} & 18.6 \textcolor{gray}{±0.1} & 75.2 \textcolor{gray}{±0.1} & 84.9 \textcolor{gray}{±0.1} & 61.0 \textcolor{gray}{±0.1} \\
RawAtt & 67.5 \textcolor{gray}{±0.1} & 19.5 \textcolor{gray}{±0.1} & 75.9 \textcolor{gray}{±0.1} & 85.0 \textcolor{gray}{±0.1} & 62.0 \textcolor{gray}{±0.1} \\
Attention Rollout & 65.9 \textcolor{gray}{±0.1} & 19.8 \textcolor{gray}{±0.1} & 75.0 \textcolor{gray}{±0.1} & 81.6 \textcolor{gray}{±0.1} & 60.6 \textcolor{gray}{±0.1} \\
AliLRP & 69.9 \textcolor{gray}{±0.1} & 21.5 \textcolor{gray}{±0.1} & 77.8 \textcolor{gray}{±0.1} & 86.9 \textcolor{gray}{±0.1} & 64.0 \textcolor{gray}{±0.1} \\
AttnLRP & 71.0 \textcolor{gray}{±0.1} & 26.4 \textcolor{gray}{±0.1} & 78.2 \textcolor{gray}{±0.1} & 88.0 \textcolor{gray}{±0.0} & 65.9 \textcolor{gray}{±0.1} \\
DecompX & 71.1 \textcolor{gray}{±0.1} & 22.6 \textcolor{gray}{±0.1} & 78.7 \textcolor{gray}{±0.1} & 87.1 \textcolor{gray}{±0.1} & 64.9 \textcolor{gray}{±0.1} \\
Integrated Gradients & 74.4 \textcolor{gray}{±0.1} & 28.6 \textcolor{gray}{±0.1} & 81.2 \textcolor{gray}{±0.1} & 88.1 \textcolor{gray}{±0.0} & 68.1 \textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 69.9 \textcolor{gray}{±0.1} & 23.4 \textcolor{gray}{±0.1} & 80.4 \textcolor{gray}{±0.1} & 88.2 \textcolor{gray}{±0.0} & 65.5 \textcolor{gray}{±0.1} \\
\textbf{Libra \IxG{} } & 72.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.7\%}) & 23.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.6\%}) & 78.7 \textcolor{gray}{±0.1} (\textcolor{coral}{-2.0\%}) & 87.4 \textcolor{gray}{±0.0} (\textcolor{coral}{-0.9\%}) & 65.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.2\%}) \\
\midrule
AttCAT & 76.8 \textcolor{gray}{±0.1} & 35.1 \textcolor{gray}{±0.1} & 82.4 \textcolor{gray}{±0.1} & \underline{89.0} \textcolor{gray}{±0.0} & 70.8 \textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \underline{80.2} \textcolor{gray}{±0.1} (\textcolor{blue}{+4.5\%}) & \underline{35.8} \textcolor{gray}{±0.1} (\textcolor{blue}{+1.8\%}) & \underline{83.2} \textcolor{gray}{±0.1} (\textcolor{blue}{+0.9\%}) & 88.9 \textcolor{gray}{±0.0} (+0.0\%) & \underline{72.0} \textcolor{gray}{±0.1} (\textcolor{blue}{+1.7\%}) \\
\midrule
GenAtt & 74.8 \textcolor{gray}{±0.1} & 25.4 \textcolor{gray}{±0.1} & 78.3 \textcolor{gray}{±0.1} & 87.8 \textcolor{gray}{±0.0} & 66.6 \textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 75.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.4\%}) & 25.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.1\%}) & 78.3 \textcolor{gray}{±0.1} (+0.0\%) & 87.6 \textcolor{gray}{±0.0} (\textcolor{coral}{-0.3\%}) & 66.6 \textcolor{gray}{±0.1} (+0.0\%) \\
\midrule
TokenTM & 73.5 \textcolor{gray}{±0.1} & 23.9 \textcolor{gray}{±0.1} & 77.1 \textcolor{gray}{±0.1} & 87.4 \textcolor{gray}{±0.0} & 65.5 \textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 73.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.1\%}) & 24.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.8\%}) & 77.1 \textcolor{gray}{±0.1} (+0.0\%) & 87.2 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.2\%}) & 65.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.1\%}) \\
\midrule
GradCAM+ & 72.0 \textcolor{gray}{±0.1} & 27.9 \textcolor{gray}{±0.1} & 77.3 \textcolor{gray}{±0.1} & 83.7 \textcolor{gray}{±0.1} & 65.2 \textcolor{gray}{±0.1} \\
\textbf{Libra GradCAM+} & 78.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+8.3\%}) & 30.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+8.3\%}) & 80.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+4.7\%}) & 87.9 \textcolor{gray}{±0.0} (\textcolor{blue}{+5.0\%}) & 69.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+6.2\%}) \\
\midrule
HiResCAM & 71.9 \textcolor{gray}{±0.1} & 24.7 \textcolor{gray}{±0.1} & 76.8 \textcolor{gray}{±0.1} & 81.1 \textcolor{gray}{±0.1} & 63.6 \textcolor{gray}{±0.1} \\
\textbf{Libra HiResCAM} & 75.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.1\%}) & 26.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+7.7\%}) & 80.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+4.3\%}) & 85.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.5\%}) & 67.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.2\%}) \\
\midrule
XGradCAM+ & 67.0 \textcolor{gray}{±0.1} & 26.9 \textcolor{gray}{±0.1} & 77.1 \textcolor{gray}{±0.1} & 84.8 \textcolor{gray}{±0.1} & 64.0 \textcolor{gray}{±0.1} \\
\textbf{Libra XGradCAM+} & 78.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+16.6\%}) & 30.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+12.3\%}) & 81.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.5\%}) & 88.2 \textcolor{gray}{±0.0} (\textcolor{blue}{+4.0\%}) & 69.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+8.6\%}) \\
\midrule
FullGrad+ & 75.2 \textcolor{gray}{±0.1} & 32.3 \textcolor{gray}{±0.1} & \underline{83.2} \textcolor{gray}{±0.1} & 88.9 \textcolor{gray}{±0.0} & 69.9 \textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & \textbf{80.6} \textcolor{gray}{±0.1} (\textcolor{blue}{+7.1\%}) & \textbf{36.1} \textcolor{gray}{±0.1} (\textcolor{blue}{+12.0\%}) & \textbf{84.0} \textcolor{gray}{±0.1} (\textcolor{blue}{+0.9\%}) & \textbf{89.1} \textcolor{gray}{±0.0} (\textcolor{blue}{+0.2\%}) & \textbf{72.4} \textcolor{gray}{±0.1} (\textcolor{blue}{+3.6\%}) \\
\bottomrule
\end{tabular}
\caption{Cross-dataset analysis of Least-Influential-First Deletion (LIF) Accuracy evaluated using ground-truth labels on ViT-B.}
\label{across_models_ds_LIF_gt_accuracy_m_2}
\end{table}


==> files/tables_v1/across_models/ds/MIF_1p_AOPC/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ImageNet & ImageNet-Hard & MURA & Oxford-IIIT Pet & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 14.2 \textcolor{gray}{±0.2} & 16.4 \textcolor{gray}{±0.2} & 4.2 \textcolor{gray}{±0.1} & 4.3 \textcolor{gray}{±0.1} & 9.8 \textcolor{gray}{±0.1} \\
RawAtt & 27.9 \textcolor{gray}{±0.3} & 23.8 \textcolor{gray}{±0.2} & 14.9 \textcolor{gray}{±0.2} & 29.6 \textcolor{gray}{±0.3} & 24.0 \textcolor{gray}{±0.2} \\
Attention Rollout & 21.2 \textcolor{gray}{±0.2} & 21.7 \textcolor{gray}{±0.2} & 10.8 \textcolor{gray}{±0.2} & 12.4 \textcolor{gray}{±0.2} & 16.5 \textcolor{gray}{±0.2} \\
AliLRP & 19.1 \textcolor{gray}{±0.2} & 22.6 \textcolor{gray}{±0.2} & 8.5 \textcolor{gray}{±0.2} & 10.0 \textcolor{gray}{±0.2} & 15.1 \textcolor{gray}{±0.2} \\
AttnLRP & 23.4 \textcolor{gray}{±0.2} & 26.3 \textcolor{gray}{±0.2} & 12.1 \textcolor{gray}{±0.2} & 22.5 \textcolor{gray}{±0.2} & 21.1 \textcolor{gray}{±0.2} \\
DecompX & 22.8 \textcolor{gray}{±0.2} & 25.0 \textcolor{gray}{±0.2} & 10.9 \textcolor{gray}{±0.2} & 14.1 \textcolor{gray}{±0.2} & 18.2 \textcolor{gray}{±0.2} \\
Integrated Gradients & 21.4 \textcolor{gray}{±0.2} & 24.6 \textcolor{gray}{±0.3} & 13.8 \textcolor{gray}{±0.2} & 11.5 \textcolor{gray}{±0.2} & 17.8 \textcolor{gray}{±0.2} \\
\midrule
\IxG{}  & 20.2 \textcolor{gray}{±0.2} & 24.3 \textcolor{gray}{±0.2} & 14.1 \textcolor{gray}{±0.2} & 11.6 \textcolor{gray}{±0.2} & 17.6 \textcolor{gray}{±0.2} \\
\textbf{Libra \IxG{} } & 23.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+15.8\%}) & 25.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+3.7\%}) & 10.9 \textcolor{gray}{±0.2} (\textcolor{coral}{-23.0\%}) & 15.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+30.0\%}) & 18.6 \textcolor{gray}{±0.2} (\textcolor{blue}{+6.2\%}) \\
\midrule
AttCAT & 28.8 \textcolor{gray}{±0.2} & 31.9 \textcolor{gray}{±0.2} & 19.6 \textcolor{gray}{±0.1} & 27.3 \textcolor{gray}{±0.4} & 26.9 \textcolor{gray}{±0.2} \\
\textbf{Libra AttCAT} & \textbf{41.5} \textcolor{gray}{±0.3} (\textcolor{blue}{+44.2\%}) & \underline{35.5} \textcolor{gray}{±0.2} (\textcolor{blue}{+11.2\%}) & \underline{28.9} \textcolor{gray}{±0.2} (\textcolor{blue}{+47.7\%}) & \underline{44.9} \textcolor{gray}{±0.3} (\textcolor{blue}{+64.7\%}) & \underline{37.7} \textcolor{gray}{±0.3} (\textcolor{blue}{+40.2\%}) \\
\midrule
GenAtt & 37.9 \textcolor{gray}{±0.2} & 32.2 \textcolor{gray}{±0.2} & 21.2 \textcolor{gray}{±0.2} & 35.7 \textcolor{gray}{±0.3} & 31.8 \textcolor{gray}{±0.3} \\
\textbf{Libra GenAtt} & 40.4 \textcolor{gray}{±0.3} (\textcolor{blue}{+6.6\%}) & 33.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+2.6\%}) & 21.1 \textcolor{gray}{±0.2} (\textcolor{coral}{-0.6\%}) & 38.1 \textcolor{gray}{±0.3} (\textcolor{blue}{+6.6\%}) & 33.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+4.4\%}) \\
\midrule
TokenTM & 37.4 \textcolor{gray}{±0.3} & 31.3 \textcolor{gray}{±0.2} & 19.5 \textcolor{gray}{±0.2} & 36.1 \textcolor{gray}{±0.3} & 31.1 \textcolor{gray}{±0.3} \\
\textbf{Libra TokenTM} & 38.9 \textcolor{gray}{±0.3} (\textcolor{blue}{+3.8\%}) & 31.7 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.4\%}) & 19.2 \textcolor{gray}{±0.2} (\textcolor{coral}{-1.7\%}) & 37.5 \textcolor{gray}{±0.3} (\textcolor{blue}{+3.9\%}) & 31.8 \textcolor{gray}{±0.3} (\textcolor{blue}{+2.4\%}) \\
\midrule
GradCAM+ & 27.6 \textcolor{gray}{±0.2} & 28.4 \textcolor{gray}{±0.2} & 12.8 \textcolor{gray}{±0.2} & 22.8 \textcolor{gray}{±0.3} & 22.9 \textcolor{gray}{±0.2} \\
\textbf{Libra GradCAM+} & 39.6 \textcolor{gray}{±0.2} (\textcolor{blue}{+43.5\%}) & 33.2 \textcolor{gray}{±0.2} (\textcolor{blue}{+17.0\%}) & 22.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+75.5\%}) & 38.6 \textcolor{gray}{±0.3} (\textcolor{blue}{+69.7\%}) & 33.5 \textcolor{gray}{±0.2} (\textcolor{blue}{+46.3\%}) \\
\midrule
HiResCAM & 28.5 \textcolor{gray}{±0.2} & 28.2 \textcolor{gray}{±0.2} & 11.8 \textcolor{gray}{±0.2} & 8.7 \textcolor{gray}{±0.2} & 19.3 \textcolor{gray}{±0.2} \\
\textbf{Libra HiResCAM} & 37.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+29.6\%}) & 31.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+11.3\%}) & 19.2 \textcolor{gray}{±0.2} (\textcolor{blue}{+63.0\%}) & 30.9 \textcolor{gray}{±0.4} (\textcolor{blue}{+254.4\%}) & 29.6 \textcolor{gray}{±0.3} (\textcolor{blue}{+53.4\%}) \\
\midrule
XGradCAM+ & 21.5 \textcolor{gray}{±0.2} & 26.4 \textcolor{gray}{±0.2} & 12.3 \textcolor{gray}{±0.1} & 23.5 \textcolor{gray}{±0.3} & 20.9 \textcolor{gray}{±0.2} \\
\textbf{Libra XGradCAM+} & \textbf{41.5} \textcolor{gray}{±0.2} (\textcolor{blue}{+92.8\%}) & 33.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+28.3\%}) & 25.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+104.9\%}) & 42.8 \textcolor{gray}{±0.3} (\textcolor{blue}{+81.7\%}) & 35.8 \textcolor{gray}{±0.3} (\textcolor{blue}{+71.1\%}) \\
\midrule
FullGrad+ & 26.3 \textcolor{gray}{±0.2} & 30.5 \textcolor{gray}{±0.2} & 20.7 \textcolor{gray}{±0.2} & 25.0 \textcolor{gray}{±0.3} & 25.6 \textcolor{gray}{±0.2} \\
\textbf{Libra FullGrad+} & 41.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+56.7\%}) & \textbf{35.6} \textcolor{gray}{±0.2} (\textcolor{blue}{+16.6\%}) & \textbf{30.5} \textcolor{gray}{±0.2} (\textcolor{blue}{+47.1\%}) & \textbf{46.7} \textcolor{gray}{±0.3} (\textcolor{blue}{+86.8\%}) & \textbf{38.5} \textcolor{gray}{±0.2} (\textcolor{blue}{+50.2\%}) \\
\bottomrule
\end{tabular}
\caption{Cross-dataset analysis of Most-Influential-First Deletion (MIF) AOPC evaluated using predicted labels on ViT-B.}
\label{across_models_ds_MIF_1p_AOPC_m_2}
\end{table}


==> files/tables_v1/across_models/ds/MIF_1p_accuracy/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ImageNet & ImageNet-Hard & MURA & Oxford-IIIT Pet & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 26.5 \textcolor{gray}{±0.1} & 52.4 \textcolor{gray}{±0.1} & 15.1 \textcolor{gray}{±0.1} & 13.7 \textcolor{gray}{±0.1} & 26.9 \textcolor{gray}{±0.1} \\
RawAtt & 44.6 \textcolor{gray}{±0.1} & 65.9 \textcolor{gray}{±0.1} & 24.8 \textcolor{gray}{±0.1} & 37.2 \textcolor{gray}{±0.1} & 43.1 \textcolor{gray}{±0.1} \\
Attention Rollout & 35.4 \textcolor{gray}{±0.1} & 62.2 \textcolor{gray}{±0.1} & 21.5 \textcolor{gray}{±0.1} & 21.2 \textcolor{gray}{±0.1} & 35.1 \textcolor{gray}{±0.1} \\
AliLRP & 33.3 \textcolor{gray}{±0.1} & 64.1 \textcolor{gray}{±0.1} & 19.2 \textcolor{gray}{±0.1} & 19.0 \textcolor{gray}{±0.1} & 33.9 \textcolor{gray}{±0.1} \\
AttnLRP & 38.5 \textcolor{gray}{±0.1} & 70.8 \textcolor{gray}{±0.1} & 22.8 \textcolor{gray}{±0.1} & 30.3 \textcolor{gray}{±0.1} & 40.6 \textcolor{gray}{±0.1} \\
DecompX & 37.8 \textcolor{gray}{±0.1} & 67.7 \textcolor{gray}{±0.1} & 21.6 \textcolor{gray}{±0.1} & 22.5 \textcolor{gray}{±0.1} & 37.4 \textcolor{gray}{±0.1} \\
Integrated Gradients & 35.4 \textcolor{gray}{±0.1} & 66.6 \textcolor{gray}{±0.1} & 23.8 \textcolor{gray}{±0.1} & 20.7 \textcolor{gray}{±0.1} & 36.6 \textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 34.4 \textcolor{gray}{±0.1} & 67.6 \textcolor{gray}{±0.1} & 25.5 \textcolor{gray}{±0.1} & 20.4 \textcolor{gray}{±0.1} & 37.0 \textcolor{gray}{±0.1} \\
\textbf{Libra \IxG{} } & 38.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+12.0\%}) & 68.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.8\%}) & 21.6 \textcolor{gray}{±0.1} (\textcolor{coral}{-15.1\%}) & 23.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+15.4\%}) & 38.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.1\%}) \\
\midrule
AttCAT & 46.9 \textcolor{gray}{±0.1} & 82.3 \textcolor{gray}{±0.1} & 31.1 \textcolor{gray}{±0.1} & 37.3 \textcolor{gray}{±0.1} & 49.4 \textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \underline{63.5} \textcolor{gray}{±0.1} (\textcolor{blue}{+35.4\%}) & \underline{87.3} \textcolor{gray}{±0.1} (\textcolor{blue}{+6.1\%}) & \underline{40.9} \textcolor{gray}{±0.1} (\textcolor{blue}{+31.6\%}) & \underline{55.3} \textcolor{gray}{±0.1} (\textcolor{blue}{+48.1\%}) & \underline{61.8} \textcolor{gray}{±0.1} (\textcolor{blue}{+25.0\%}) \\
\midrule
GenAtt & 58.2 \textcolor{gray}{±0.1} & 81.3 \textcolor{gray}{±0.1} & 30.0 \textcolor{gray}{±0.1} & 44.1 \textcolor{gray}{±0.1} & 53.4 \textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 61.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.8\%}) & 82.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.8\%}) & 30.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.4\%}) & 46.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.4\%}) & 55.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.4\%}) \\
\midrule
TokenTM & 56.8 \textcolor{gray}{±0.1} & 79.3 \textcolor{gray}{±0.1} & 28.0 \textcolor{gray}{±0.1} & 44.0 \textcolor{gray}{±0.1} & 52.0 \textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 59.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+4.1\%}) & 80.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.8\%}) & 28.0 \textcolor{gray}{±0.1} (+0.0\%) & 45.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.3\%}) & 53.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.1\%}) \\
\midrule
GradCAM+ & 45.6 \textcolor{gray}{±0.1} & 75.8 \textcolor{gray}{±0.1} & 24.0 \textcolor{gray}{±0.1} & 32.6 \textcolor{gray}{±0.1} & 44.5 \textcolor{gray}{±0.1} \\
\textbf{Libra GradCAM+} & 61.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+34.8\%}) & 83.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+10.0\%}) & 34.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+44.8\%}) & 47.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+46.6\%}) & 56.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+27.8\%}) \\
\midrule
HiResCAM & 45.4 \textcolor{gray}{±0.1} & 74.2 \textcolor{gray}{±0.1} & 22.2 \textcolor{gray}{±0.1} & 18.0 \textcolor{gray}{±0.1} & 39.9 \textcolor{gray}{±0.1} \\
\textbf{Libra HiResCAM} & 56.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+24.8\%}) & 79.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+7.4\%}) & 30.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+35.7\%}) & 39.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+119.0\%}) & 51.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+28.9\%}) \\
\midrule
XGradCAM+ & 38.6 \textcolor{gray}{±0.1} & 72.1 \textcolor{gray}{±0.1} & 23.7 \textcolor{gray}{±0.1} & 33.2 \textcolor{gray}{±0.1} & 41.9 \textcolor{gray}{±0.1} \\
\textbf{Libra XGradCAM+} & \textbf{63.9} \textcolor{gray}{±0.1} (\textcolor{blue}{+65.6\%}) & 84.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+17.3\%}) & 36.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+54.6\%}) & 52.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+58.4\%}) & 59.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+41.8\%}) \\
\midrule
FullGrad+ & 44.2 \textcolor{gray}{±0.1} & 80.1 \textcolor{gray}{±0.1} & 32.8 \textcolor{gray}{±0.1} & 35.3 \textcolor{gray}{±0.1} & 48.1 \textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & 63.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+42.9\%}) & \textbf{87.6} \textcolor{gray}{±0.1} (\textcolor{blue}{+9.4\%}) & \textbf{43.2} \textcolor{gray}{±0.1} (\textcolor{blue}{+31.7\%}) & \textbf{57.3} \textcolor{gray}{±0.1} (\textcolor{blue}{+62.3\%}) & \textbf{62.8} \textcolor{gray}{±0.1} (\textcolor{blue}{+30.6\%}) \\
\bottomrule
\end{tabular}
\caption{Cross-dataset analysis of Most-Influential-First Deletion (MIF) Accuracy evaluated using predicted labels on ViT-B.}
\label{across_models_ds_MIF_1p_accuracy_m_2}
\end{table}


==> files/tables_v1/across_models/ds/MIF_gt_AOPC/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ImageNet & ImageNet-Hard & MURA & Oxford-IIIT Pet & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 12.3 \textcolor{gray}{±0.2} & 6.6 \textcolor{gray}{±0.1} & 3.3 \textcolor{gray}{±0.1} & 4.1 \textcolor{gray}{±0.1} & 6.6 \textcolor{gray}{±0.1} \\
RawAtt & 25.0 \textcolor{gray}{±0.3} & 9.5 \textcolor{gray}{±0.1} & 12.6 \textcolor{gray}{±0.3} & 29.1 \textcolor{gray}{±0.3} & 19.0 \textcolor{gray}{±0.3} \\
Attention Rollout & 18.8 \textcolor{gray}{±0.3} & 8.7 \textcolor{gray}{±0.1} & 8.6 \textcolor{gray}{±0.2} & 12.2 \textcolor{gray}{±0.2} & 12.1 \textcolor{gray}{±0.2} \\
AliLRP & 16.7 \textcolor{gray}{±0.2} & 9.1 \textcolor{gray}{±0.1} & 7.1 \textcolor{gray}{±0.2} & 9.7 \textcolor{gray}{±0.2} & 10.7 \textcolor{gray}{±0.2} \\
AttnLRP & 20.8 \textcolor{gray}{±0.3} & 10.8 \textcolor{gray}{±0.2} & 10.4 \textcolor{gray}{±0.2} & 22.1 \textcolor{gray}{±0.2} & 16.0 \textcolor{gray}{±0.2} \\
DecompX & 20.3 \textcolor{gray}{±0.3} & 10.2 \textcolor{gray}{±0.1} & 9.5 \textcolor{gray}{±0.2} & 13.8 \textcolor{gray}{±0.2} & 13.4 \textcolor{gray}{±0.2} \\
Integrated Gradients & 22.5 \textcolor{gray}{±0.2} & 11.7 \textcolor{gray}{±0.1} & 14.5 \textcolor{gray}{±0.2} & 17.6 \textcolor{gray}{±0.3} & 16.6 \textcolor{gray}{±0.2} \\
\midrule
\IxG{}  & 17.7 \textcolor{gray}{±0.2} & 9.8 \textcolor{gray}{±0.1} & 12.0 \textcolor{gray}{±0.2} & 11.2 \textcolor{gray}{±0.2} & 12.7 \textcolor{gray}{±0.2} \\
\textbf{Libra \IxG{} } & 20.8 \textcolor{gray}{±0.3} (\textcolor{blue}{+17.4\%}) & 10.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.3\%}) & 9.5 \textcolor{gray}{±0.2} (\textcolor{coral}{-20.9\%}) & 14.8 \textcolor{gray}{±0.2} (\textcolor{blue}{+32.2\%}) & 13.8 \textcolor{gray}{±0.2} (\textcolor{blue}{+9.3\%}) \\
\midrule
AttCAT & 25.3 \textcolor{gray}{±0.2} & 13.1 \textcolor{gray}{±0.1} & 16.7 \textcolor{gray}{±0.2} & 26.7 \textcolor{gray}{±0.3} & 20.5 \textcolor{gray}{±0.2} \\
\textbf{Libra AttCAT} & \underline{37.5} \textcolor{gray}{±0.3} (\textcolor{blue}{+47.9\%}) & \underline{14.9} \textcolor{gray}{±0.1} (\textcolor{blue}{+14.0\%}) & \underline{25.6} \textcolor{gray}{±0.3} (\textcolor{blue}{+53.0\%}) & \underline{44.3} \textcolor{gray}{±0.3} (\textcolor{blue}{+65.8\%}) & \underline{30.6} \textcolor{gray}{±0.3} (\textcolor{blue}{+49.3\%}) \\
\midrule
GenAtt & 34.2 \textcolor{gray}{±0.3} & 13.5 \textcolor{gray}{±0.1} & 18.1 \textcolor{gray}{±0.3} & 35.2 \textcolor{gray}{±0.3} & 25.2 \textcolor{gray}{±0.3} \\
\textbf{Libra GenAtt} & 36.6 \textcolor{gray}{±0.3} (\textcolor{blue}{+6.8\%}) & 13.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.8\%}) & 18.0 \textcolor{gray}{±0.3} (\textcolor{coral}{-0.2\%}) & 37.6 \textcolor{gray}{±0.3} (\textcolor{blue}{+6.7\%}) & 26.5 \textcolor{gray}{±0.3} (\textcolor{blue}{+5.0\%}) \\
\midrule
TokenTM & 33.8 \textcolor{gray}{±0.3} & 12.9 \textcolor{gray}{±0.1} & 16.4 \textcolor{gray}{±0.3} & 35.6 \textcolor{gray}{±0.3} & 24.7 \textcolor{gray}{±0.3} \\
\textbf{Libra TokenTM} & 35.1 \textcolor{gray}{±0.3} (\textcolor{blue}{+4.0\%}) & 13.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.0\%}) & 16.2 \textcolor{gray}{±0.3} (\textcolor{coral}{-1.5\%}) & 37.0 \textcolor{gray}{±0.3} (\textcolor{blue}{+4.0\%}) & 25.4 \textcolor{gray}{±0.3} (\textcolor{blue}{+2.8\%}) \\
\midrule
GradCAM+ & 24.8 \textcolor{gray}{±0.2} & 11.4 \textcolor{gray}{±0.1} & 11.0 \textcolor{gray}{±0.2} & 22.2 \textcolor{gray}{±0.3} & 17.4 \textcolor{gray}{±0.2} \\
\textbf{Libra GradCAM+} & 35.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+44.8\%}) & 13.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+21.2\%}) & 20.1 \textcolor{gray}{±0.3} (\textcolor{blue}{+82.2\%}) & 38.0 \textcolor{gray}{±0.3} (\textcolor{blue}{+71.0\%}) & 27.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+55.3\%}) \\
\midrule
HiResCAM & 25.4 \textcolor{gray}{±0.3} & 11.5 \textcolor{gray}{±0.1} & 10.4 \textcolor{gray}{±0.2} & 8.5 \textcolor{gray}{±0.2} & 13.9 \textcolor{gray}{±0.2} \\
\textbf{Libra HiResCAM} & 33.4 \textcolor{gray}{±0.3} (\textcolor{blue}{+31.7\%}) & 12.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+12.7\%}) & 17.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+63.5\%}) & 30.7 \textcolor{gray}{±0.4} (\textcolor{blue}{+260.3\%}) & 23.5 \textcolor{gray}{±0.3} (\textcolor{blue}{+68.7\%}) \\
\midrule
XGradCAM+ & 19.0 \textcolor{gray}{±0.2} & 10.6 \textcolor{gray}{±0.1} & 10.6 \textcolor{gray}{±0.2} & 23.0 \textcolor{gray}{±0.3} & 15.8 \textcolor{gray}{±0.2} \\
\textbf{Libra XGradCAM+} & \textbf{37.7} \textcolor{gray}{±0.2} (\textcolor{blue}{+98.6\%}) & 14.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+33.7\%}) & 22.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+108.5\%}) & 42.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+83.3\%}) & 29.0 \textcolor{gray}{±0.3} (\textcolor{blue}{+83.8\%}) \\
\midrule
FullGrad+ & 23.1 \textcolor{gray}{±0.3} & 12.3 \textcolor{gray}{±0.1} & 17.7 \textcolor{gray}{±0.2} & 24.5 \textcolor{gray}{±0.3} & 19.4 \textcolor{gray}{±0.2} \\
\textbf{Libra FullGrad+} & 37.2 \textcolor{gray}{±0.3} (\textcolor{blue}{+60.9\%}) & \textbf{15.0} \textcolor{gray}{±0.1} (\textcolor{blue}{+22.4\%}) & \textbf{26.9} \textcolor{gray}{±0.3} (\textcolor{blue}{+51.7\%}) & \textbf{46.1} \textcolor{gray}{±0.3} (\textcolor{blue}{+88.1\%}) & \textbf{31.3} \textcolor{gray}{±0.3} (\textcolor{blue}{+61.3\%}) \\
\bottomrule
\end{tabular}
\caption{Cross-dataset analysis of Most-Influential-First Deletion (MIF) AOPC evaluated using ground-truth labels on ViT-B.}
\label{across_models_ds_MIF_gt_AOPC_m_2}
\end{table}


==> files/tables_v1/across_models/ds/MIF_gt_accuracy/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ImageNet & ImageNet-Hard & MURA & Oxford-IIIT Pet & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 34.5 \textcolor{gray}{±0.1} & 81.7 \textcolor{gray}{±0.1} & 25.4 \textcolor{gray}{±0.1} & 14.6 \textcolor{gray}{±0.1} & 39.1 \textcolor{gray}{±0.1} \\
RawAtt & 50.1 \textcolor{gray}{±0.1} & 85.9 \textcolor{gray}{±0.1} & 33.4 \textcolor{gray}{±0.1} & 37.7 \textcolor{gray}{±0.1} & 51.8 \textcolor{gray}{±0.1} \\
Attention Rollout & 41.9 \textcolor{gray}{±0.1} & 84.7 \textcolor{gray}{±0.1} & 29.9 \textcolor{gray}{±0.1} & 22.2 \textcolor{gray}{±0.1} & 44.7 \textcolor{gray}{±0.1} \\
AliLRP & 39.8 \textcolor{gray}{±0.1} & 85.7 \textcolor{gray}{±0.1} & 28.4 \textcolor{gray}{±0.1} & 19.7 \textcolor{gray}{±0.1} & 43.4 \textcolor{gray}{±0.1} \\
AttnLRP & 44.5 \textcolor{gray}{±0.1} & 88.2 \textcolor{gray}{±0.1} & 31.6 \textcolor{gray}{±0.1} & 30.9 \textcolor{gray}{±0.1} & 48.8 \textcolor{gray}{±0.1} \\
DecompX & 44.0 \textcolor{gray}{±0.1} & 87.1 \textcolor{gray}{±0.1} & 30.7 \textcolor{gray}{±0.1} & 23.2 \textcolor{gray}{±0.1} & 46.3 \textcolor{gray}{±0.1} \\
Integrated Gradients & 46.9 \textcolor{gray}{±0.1} & 89.5 \textcolor{gray}{±0.1} & 35.6 \textcolor{gray}{±0.1} & 27.5 \textcolor{gray}{±0.1} & 49.9 \textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 40.4 \textcolor{gray}{±0.1} & 87.0 \textcolor{gray}{±0.1} & 33.2 \textcolor{gray}{±0.1} & 20.9 \textcolor{gray}{±0.1} & 45.4 \textcolor{gray}{±0.1} \\
\textbf{Libra \IxG{} } & 44.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+10.8\%}) & 87.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.6\%}) & 30.7 \textcolor{gray}{±0.1} (\textcolor{coral}{-7.5\%}) & 24.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+16.2\%}) & 46.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.2\%}) \\
\midrule
AttCAT & 50.4 \textcolor{gray}{±0.1} & 91.8 \textcolor{gray}{±0.1} & 37.8 \textcolor{gray}{±0.1} & 37.6 \textcolor{gray}{±0.1} & 54.4 \textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \underline{66.4} \textcolor{gray}{±0.1} (\textcolor{blue}{+31.7\%}) & \underline{94.4} \textcolor{gray}{±0.1} (\textcolor{blue}{+2.9\%}) & \underline{47.1} \textcolor{gray}{±0.1} (\textcolor{blue}{+24.5\%}) & \underline{55.5} \textcolor{gray}{±0.1} (\textcolor{blue}{+47.6\%}) & \underline{65.9} \textcolor{gray}{±0.1} (\textcolor{blue}{+21.0\%}) \\
\midrule
GenAtt & 61.9 \textcolor{gray}{±0.1} & 92.0 \textcolor{gray}{±0.1} & 37.8 \textcolor{gray}{±0.1} & 44.5 \textcolor{gray}{±0.1} & 59.1 \textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 65.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.1\%}) & 92.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.6\%}) & 38.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.7\%}) & 46.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.3\%}) & 60.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.7\%}) \\
\midrule
TokenTM & 60.6 \textcolor{gray}{±0.1} & 90.9 \textcolor{gray}{±0.1} & 36.1 \textcolor{gray}{±0.1} & 44.4 \textcolor{gray}{±0.1} & 58.0 \textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 62.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.6\%}) & 91.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.5\%}) & 36.0 \textcolor{gray}{±0.1} (\textcolor{coral}{-0.1\%}) & 45.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.3\%}) & 59.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.7\%}) \\
\midrule
GradCAM+ & 50.5 \textcolor{gray}{±0.1} & 89.2 \textcolor{gray}{±0.1} & 32.6 \textcolor{gray}{±0.1} & 33.1 \textcolor{gray}{±0.1} & 51.4 \textcolor{gray}{±0.1} \\
\textbf{Libra GradCAM+} & 65.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+29.3\%}) & 92.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.9\%}) & 42.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+29.9\%}) & 48.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+45.8\%}) & 62.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+21.0\%}) \\
\midrule
HiResCAM & 50.4 \textcolor{gray}{±0.1} & 89.3 \textcolor{gray}{±0.1} & 31.4 \textcolor{gray}{±0.1} & 18.7 \textcolor{gray}{±0.1} & 47.5 \textcolor{gray}{±0.1} \\
\textbf{Libra HiResCAM} & 60.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+20.6\%}) & 91.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.4\%}) & 37.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+20.4\%}) & 40.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+114.4\%}) & 57.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+21.3\%}) \\
\midrule
XGradCAM+ & 44.0 \textcolor{gray}{±0.1} & 87.8 \textcolor{gray}{±0.1} & 32.4 \textcolor{gray}{±0.1} & 33.5 \textcolor{gray}{±0.1} & 49.4 \textcolor{gray}{±0.1} \\
\textbf{Libra XGradCAM+} & \textbf{67.4} \textcolor{gray}{±0.1} (\textcolor{blue}{+53.0\%}) & 93.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+6.2\%}) & 43.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+34.1\%}) & 52.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+57.6\%}) & 64.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+29.9\%}) \\
\midrule
FullGrad+ & 48.2 \textcolor{gray}{±0.1} & 90.5 \textcolor{gray}{±0.1} & 39.1 \textcolor{gray}{±0.1} & 35.6 \textcolor{gray}{±0.1} & 53.4 \textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & 66.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+37.1\%}) & \textbf{94.7} \textcolor{gray}{±0.1} (\textcolor{blue}{+4.6\%}) & \textbf{48.7} \textcolor{gray}{±0.1} (\textcolor{blue}{+24.5\%}) & \textbf{57.5} \textcolor{gray}{±0.1} (\textcolor{blue}{+61.6\%}) & \textbf{66.7} \textcolor{gray}{±0.1} (\textcolor{blue}{+25.1\%}) \\
\bottomrule
\end{tabular}
\caption{Cross-dataset analysis of Most-Influential-First Deletion (MIF) Accuracy evaluated using ground-truth labels on ViT-B.}
\label{across_models_ds_MIF_gt_accuracy_m_2}
\end{table}


==> files/tables_v1/across_models/ds/SRG_1p_AOPC/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ImageNet & ImageNet-Hard & MURA & Oxford-IIIT Pet & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 50.0 \textcolor{gray}{±0.2} & 49.8 \textcolor{gray}{±0.2} & 50.2 \textcolor{gray}{±0.1} & 49.8 \textcolor{gray}{±0.1} & 50.0 \textcolor{gray}{±0.2} \\
RawAtt & 57.8 \textcolor{gray}{±0.2} & 54.6 \textcolor{gray}{±0.2} & 55.8 \textcolor{gray}{±0.2} & 62.8 \textcolor{gray}{±0.2} & 57.7 \textcolor{gray}{±0.2} \\
Attention Rollout & 53.6 \textcolor{gray}{±0.2} & 52.9 \textcolor{gray}{±0.2} & 52.9 \textcolor{gray}{±0.2} & 52.0 \textcolor{gray}{±0.2} & 52.9 \textcolor{gray}{±0.2} \\
AliLRP & 54.2 \textcolor{gray}{±0.2} & 55.0 \textcolor{gray}{±0.2} & 53.5 \textcolor{gray}{±0.1} & 54.0 \textcolor{gray}{±0.2} & 54.2 \textcolor{gray}{±0.2} \\
AttnLRP & 57.1 \textcolor{gray}{±0.2} & 59.9 \textcolor{gray}{±0.2} & 55.4 \textcolor{gray}{±0.2} & 60.9 \textcolor{gray}{±0.2} & 58.3 \textcolor{gray}{±0.2} \\
DecompX & 56.7 \textcolor{gray}{±0.2} & 57.2 \textcolor{gray}{±0.2} & 55.1 \textcolor{gray}{±0.1} & 56.2 \textcolor{gray}{±0.2} & 56.3 \textcolor{gray}{±0.2} \\
Integrated Gradients & 56.3 \textcolor{gray}{±0.2} & 57.2 \textcolor{gray}{±0.2} & 56.5 \textcolor{gray}{±0.1} & 54.5 \textcolor{gray}{±0.1} & 56.1 \textcolor{gray}{±0.2} \\
\midrule
\IxG{}  & 55.2 \textcolor{gray}{±0.2} & 57.1 \textcolor{gray}{±0.2} & 57.3 \textcolor{gray}{±0.2} & 55.5 \textcolor{gray}{±0.2} & 56.3 \textcolor{gray}{±0.2} \\
\textbf{Libra \IxG{} } & 57.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+3.9\%}) & 57.7 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.0\%}) & 55.1 \textcolor{gray}{±0.1} (\textcolor{coral}{-3.8\%}) & 56.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+2.5\%}) & 56.8 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.9\%}) \\
\midrule
AttCAT & 62.7 \textcolor{gray}{±0.2} & 67.0 \textcolor{gray}{±0.2} & 60.8 \textcolor{gray}{±0.1} & 64.1 \textcolor{gray}{±0.3} & 63.7 \textcolor{gray}{±0.2} \\
\textbf{Libra AttCAT} & \textbf{70.4} \textcolor{gray}{±0.2} (\textcolor{blue}{+12.2\%}) & \underline{70.5} \textcolor{gray}{±0.2} (\textcolor{blue}{+5.3\%}) & \underline{65.6} \textcolor{gray}{±0.2} (\textcolor{blue}{+7.9\%}) & \underline{72.9} \textcolor{gray}{±0.2} (\textcolor{blue}{+13.7\%}) & \underline{69.9} \textcolor{gray}{±0.2} (\textcolor{blue}{+9.7\%}) \\
\midrule
GenAtt & 66.3 \textcolor{gray}{±0.2} & 62.8 \textcolor{gray}{±0.2} & 60.3 \textcolor{gray}{±0.2} & 67.5 \textcolor{gray}{±0.2} & 64.2 \textcolor{gray}{±0.2} \\
\textbf{Libra GenAtt} & 67.6 \textcolor{gray}{±0.2} (\textcolor{blue}{+2.1\%}) & 63.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.7\%}) & 60.1 \textcolor{gray}{±0.2} (\textcolor{coral}{-0.2\%}) & 68.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.3\%}) & 64.8 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.0\%}) \\
\midrule
TokenTM & 65.3 \textcolor{gray}{±0.2} & 61.2 \textcolor{gray}{±0.2} & 58.8 \textcolor{gray}{±0.2} & 67.4 \textcolor{gray}{±0.2} & 63.2 \textcolor{gray}{±0.2} \\
\textbf{Libra TokenTM} & 66.2 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.3\%}) & 61.5 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.5\%}) & 58.7 \textcolor{gray}{±0.2} (\textcolor{coral}{-0.2\%}) & 67.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.7\%}) & 63.6 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.6\%}) \\
\midrule
GradCAM+ & 59.5 \textcolor{gray}{±0.2} & 61.2 \textcolor{gray}{±0.2} & 54.8 \textcolor{gray}{±0.2} & 58.5 \textcolor{gray}{±0.2} & 58.5 \textcolor{gray}{±0.2} \\
\textbf{Libra GradCAM+} & 67.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+14.1\%}) & 65.7 \textcolor{gray}{±0.2} (\textcolor{blue}{+7.5\%}) & 61.5 \textcolor{gray}{±0.2} (\textcolor{blue}{+12.2\%}) & 68.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+17.8\%}) & 66.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+12.8\%}) \\
\midrule
HiResCAM & 60.1 \textcolor{gray}{±0.2} & 59.4 \textcolor{gray}{±0.2} & 54.7 \textcolor{gray}{±0.1} & 49.8 \textcolor{gray}{±0.2} & 56.0 \textcolor{gray}{±0.2} \\
\textbf{Libra HiResCAM} & 65.7 \textcolor{gray}{±0.2} (\textcolor{blue}{+9.2\%}) & 62.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+5.0\%}) & 59.5 \textcolor{gray}{±0.2} (\textcolor{blue}{+8.8\%}) & 63.6 \textcolor{gray}{±0.3} (\textcolor{blue}{+27.7\%}) & 62.8 \textcolor{gray}{±0.2} (\textcolor{blue}{+12.1\%}) \\
\midrule
XGradCAM+ & 54.1 \textcolor{gray}{±0.2} & 59.4 \textcolor{gray}{±0.2} & 54.6 \textcolor{gray}{±0.1} & 59.5 \textcolor{gray}{±0.2} & 56.9 \textcolor{gray}{±0.2} \\
\textbf{Libra XGradCAM+} & 69.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+27.7\%}) & 66.5 \textcolor{gray}{±0.2} (\textcolor{blue}{+11.8\%}) & 62.8 \textcolor{gray}{±0.2} (\textcolor{blue}{+14.9\%}) & 71.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+19.6\%}) & 67.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+18.4\%}) \\
\midrule
FullGrad+ & 60.7 \textcolor{gray}{±0.2} & 65.2 \textcolor{gray}{±0.2} & 61.7 \textcolor{gray}{±0.1} & 62.9 \textcolor{gray}{±0.2} & 62.6 \textcolor{gray}{±0.2} \\
\textbf{Libra FullGrad+} & \textbf{70.4} \textcolor{gray}{±0.2} (\textcolor{blue}{+16.0\%}) & \textbf{71.0} \textcolor{gray}{±0.2} (\textcolor{blue}{+8.9\%}) & \textbf{66.6} \textcolor{gray}{±0.2} (\textcolor{blue}{+7.9\%}) & \textbf{73.9} \textcolor{gray}{±0.2} (\textcolor{blue}{+17.5\%}) & \textbf{70.5} \textcolor{gray}{±0.2} (\textcolor{blue}{+12.5\%}) \\
\bottomrule
\end{tabular}
\caption{Cross-dataset analysis of Symmetric Relevance Gain (SRG) AOPC evaluated using predicted labels on ViT-B.}
\label{across_models_ds_SRG_1p_AOPC_m_2}
\end{table}


==> files/tables_v1/across_models/ds/SRG_1p_accuracy/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ImageNet & ImageNet-Hard & MURA & Oxford-IIIT Pet & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 49.9 \textcolor{gray}{±0.1} & 49.7 \textcolor{gray}{±0.1} & 50.4 \textcolor{gray}{±0.1} & 49.7 \textcolor{gray}{±0.1} & 49.9 \textcolor{gray}{±0.1} \\
RawAtt & 60.4 \textcolor{gray}{±0.1} & 58.9 \textcolor{gray}{±0.1} & 55.3 \textcolor{gray}{±0.1} & 61.6 \textcolor{gray}{±0.1} & 59.1 \textcolor{gray}{±0.1} \\
Attention Rollout & 54.6 \textcolor{gray}{±0.1} & 56.0 \textcolor{gray}{±0.1} & 52.8 \textcolor{gray}{±0.1} & 51.8 \textcolor{gray}{±0.1} & 53.8 \textcolor{gray}{±0.1} \\
AliLRP & 55.5 \textcolor{gray}{±0.1} & 58.8 \textcolor{gray}{±0.1} & 53.1 \textcolor{gray}{±0.1} & 53.3 \textcolor{gray}{±0.1} & 55.2 \textcolor{gray}{±0.1} \\
AttnLRP & 58.6 \textcolor{gray}{±0.1} & 66.2 \textcolor{gray}{±0.1} & 54.9 \textcolor{gray}{±0.1} & 59.5 \textcolor{gray}{±0.1} & 59.8 \textcolor{gray}{±0.1} \\
DecompX & 58.5 \textcolor{gray}{±0.1} & 62.2 \textcolor{gray}{±0.1} & 54.7 \textcolor{gray}{±0.1} & 55.3 \textcolor{gray}{±0.1} & 57.7 \textcolor{gray}{±0.1} \\
Integrated Gradients & 56.7 \textcolor{gray}{±0.1} & 60.4 \textcolor{gray}{±0.1} & 55.1 \textcolor{gray}{±0.1} & 53.8 \textcolor{gray}{±0.1} & 56.5 \textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 55.9 \textcolor{gray}{±0.1} & 61.8 \textcolor{gray}{±0.1} & 56.8 \textcolor{gray}{±0.1} & 54.5 \textcolor{gray}{±0.1} & 57.2 \textcolor{gray}{±0.1} \\
\textbf{Libra \IxG{} } & 59.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+6.3\%}) & 63.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.6\%}) & 54.7 \textcolor{gray}{±0.1} (\textcolor{coral}{-3.8\%}) & 55.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.5\%}) & 58.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.9\%}) \\
\midrule
AttCAT & 64.7 \textcolor{gray}{±0.1} & 75.8 \textcolor{gray}{±0.1} & 60.1 \textcolor{gray}{±0.1} & 63.3 \textcolor{gray}{±0.1} & 66.0 \textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \textbf{75.1} \textcolor{gray}{±0.1} (\textcolor{blue}{+16.1\%}) & \underline{81.6} \textcolor{gray}{±0.1} (\textcolor{blue}{+7.7\%}) & \underline{65.2} \textcolor{gray}{±0.1} (\textcolor{blue}{+8.4\%}) & \underline{72.3} \textcolor{gray}{±0.1} (\textcolor{blue}{+14.2\%}) & \underline{73.5} \textcolor{gray}{±0.1} (\textcolor{blue}{+11.5\%}) \\
\midrule
GenAtt & 71.1 \textcolor{gray}{±0.1} & 73.5 \textcolor{gray}{±0.1} & 59.1 \textcolor{gray}{±0.1} & 66.4 \textcolor{gray}{±0.1} & 67.5 \textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 73.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.6\%}) & 74.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.5\%}) & 59.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.1\%}) & 67.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.6\%}) & 68.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.5\%}) \\
\midrule
TokenTM & 70.0 \textcolor{gray}{±0.1} & 71.1 \textcolor{gray}{±0.1} & 57.7 \textcolor{gray}{±0.1} & 66.2 \textcolor{gray}{±0.1} & 66.2 \textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 71.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.7\%}) & 71.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.6\%}) & 57.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.2\%}) & 66.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.9\%}) & 66.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.9\%}) \\
\midrule
GradCAM+ & 62.0 \textcolor{gray}{±0.1} & 68.5 \textcolor{gray}{±0.1} & 54.9 \textcolor{gray}{±0.1} & 58.4 \textcolor{gray}{±0.1} & 61.0 \textcolor{gray}{±0.1} \\
\textbf{Libra GradCAM+} & 73.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+18.0\%}) & 76.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+11.0\%}) & 61.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+12.2\%}) & 68.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+16.6\%}) & 69.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+14.4\%}) \\
\midrule
HiResCAM & 62.5 \textcolor{gray}{±0.1} & 65.9 \textcolor{gray}{±0.1} & 54.1 \textcolor{gray}{±0.1} & 49.8 \textcolor{gray}{±0.1} & 58.1 \textcolor{gray}{±0.1} \\
\textbf{Libra HiResCAM} & 69.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+11.6\%}) & 70.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+7.5\%}) & 58.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+8.9\%}) & 62.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+26.2\%}) & 65.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+12.9\%}) \\
\midrule
XGradCAM+ & 55.9 \textcolor{gray}{±0.1} & 65.5 \textcolor{gray}{±0.1} & 54.7 \textcolor{gray}{±0.1} & 59.2 \textcolor{gray}{±0.1} & 58.8 \textcolor{gray}{±0.1} \\
\textbf{Libra XGradCAM+} & 74.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+33.5\%}) & 77.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+17.9\%}) & 62.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+14.0\%}) & 70.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+19.3\%}) & 71.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+21.0\%}) \\
\midrule
FullGrad+ & 62.9 \textcolor{gray}{±0.1} & 73.7 \textcolor{gray}{±0.1} & 61.2 \textcolor{gray}{±0.1} & 62.3 \textcolor{gray}{±0.1} & 65.0 \textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & \underline{75.0} \textcolor{gray}{±0.1} (\textcolor{blue}{+19.4\%}) & \textbf{81.9} \textcolor{gray}{±0.1} (\textcolor{blue}{+11.2\%}) & \textbf{66.4} \textcolor{gray}{±0.1} (\textcolor{blue}{+8.5\%}) & \textbf{73.4} \textcolor{gray}{±0.1} (\textcolor{blue}{+17.9\%}) & \textbf{74.2} \textcolor{gray}{±0.1} (\textcolor{blue}{+14.2\%}) \\
\bottomrule
\end{tabular}
\caption{Cross-dataset analysis of Symmetric Relevance Gain (SRG) Accuracy evaluated using predicted labels on ViT-B.}
\label{across_models_ds_SRG_1p_accuracy_m_2}
\end{table}


==> files/tables_v1/across_models/ds/SRG_gt_AOPC/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ImageNet & ImageNet-Hard & MURA & Oxford-IIIT Pet & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 49.9 \textcolor{gray}{±0.2} & 50.0 \textcolor{gray}{±0.1} & 50.2 \textcolor{gray}{±0.1} & 49.9 \textcolor{gray}{±0.1} & 50.0 \textcolor{gray}{±0.1} \\
RawAtt & 57.1 \textcolor{gray}{±0.2} & 51.8 \textcolor{gray}{±0.1} & 55.2 \textcolor{gray}{±0.2} & 62.7 \textcolor{gray}{±0.2} & 56.7 \textcolor{gray}{±0.2} \\
Attention Rollout & 53.3 \textcolor{gray}{±0.2} & 51.3 \textcolor{gray}{±0.1} & 52.5 \textcolor{gray}{±0.2} & 52.1 \textcolor{gray}{±0.2} & 52.3 \textcolor{gray}{±0.2} \\
AliLRP & 53.8 \textcolor{gray}{±0.2} & 52.1 \textcolor{gray}{±0.1} & 53.5 \textcolor{gray}{±0.2} & 54.0 \textcolor{gray}{±0.2} & 53.4 \textcolor{gray}{±0.2} \\
AttnLRP & 56.6 \textcolor{gray}{±0.2} & 54.5 \textcolor{gray}{±0.1} & 55.4 \textcolor{gray}{±0.2} & 60.9 \textcolor{gray}{±0.2} & 56.8 \textcolor{gray}{±0.2} \\
DecompX & 56.3 \textcolor{gray}{±0.2} & 53.2 \textcolor{gray}{±0.1} & 55.2 \textcolor{gray}{±0.2} & 56.1 \textcolor{gray}{±0.2} & 55.2 \textcolor{gray}{±0.2} \\
Integrated Gradients & 59.1 \textcolor{gray}{±0.2} & 55.7 \textcolor{gray}{±0.1} & 59.1 \textcolor{gray}{±0.2} & 58.8 \textcolor{gray}{±0.2} & 58.2 \textcolor{gray}{±0.2} \\
\midrule
\IxG{}  & 54.8 \textcolor{gray}{±0.2} & 53.2 \textcolor{gray}{±0.1} & 57.3 \textcolor{gray}{±0.2} & 55.5 \textcolor{gray}{±0.2} & 55.2 \textcolor{gray}{±0.2} \\
\textbf{Libra \IxG{} } & 56.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+4.0\%}) & 53.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.4\%}) & 55.2 \textcolor{gray}{±0.2} (\textcolor{coral}{-3.7\%}) & 56.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+2.5\%}) & 55.6 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.7\%}) \\
\midrule
AttCAT & 61.9 \textcolor{gray}{±0.2} & 58.6 \textcolor{gray}{±0.1} & 60.8 \textcolor{gray}{±0.2} & 64.0 \textcolor{gray}{±0.2} & 61.3 \textcolor{gray}{±0.2} \\
\textbf{Libra AttCAT} & \underline{69.1} \textcolor{gray}{±0.2} (\textcolor{blue}{+11.7\%}) & \underline{59.7} \textcolor{gray}{±0.2} (\textcolor{blue}{+1.9\%}) & \underline{65.6} \textcolor{gray}{±0.2} (\textcolor{blue}{+7.9\%}) & \underline{72.8} \textcolor{gray}{±0.2} (\textcolor{blue}{+13.7\%}) & \underline{66.8} \textcolor{gray}{±0.2} (\textcolor{blue}{+8.9\%}) \\
\midrule
GenAtt & 65.0 \textcolor{gray}{±0.2} & 55.6 \textcolor{gray}{±0.1} & 59.2 \textcolor{gray}{±0.2} & 67.3 \textcolor{gray}{±0.2} & 61.8 \textcolor{gray}{±0.2} \\
\textbf{Libra GenAtt} & 66.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+2.0\%}) & 55.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.4\%}) & 59.2 \textcolor{gray}{±0.2} (\textcolor{coral}{-0.1\%}) & 68.2 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.3\%}) & 62.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.9\%}) \\
\midrule
TokenTM & 64.1 \textcolor{gray}{±0.2} & 54.9 \textcolor{gray}{±0.1} & 57.8 \textcolor{gray}{±0.2} & 67.3 \textcolor{gray}{±0.2} & 61.0 \textcolor{gray}{±0.2} \\
\textbf{Libra TokenTM} & 64.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+1.2\%}) & 55.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.3\%}) & 57.7 \textcolor{gray}{±0.2} (\textcolor{coral}{-0.2\%}) & 67.8 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.8\%}) & 61.3 \textcolor{gray}{±0.2} (\textcolor{blue}{+0.5\%}) \\
\midrule
GradCAM+ & 59.2 \textcolor{gray}{±0.2} & 55.1 \textcolor{gray}{±0.1} & 54.9 \textcolor{gray}{±0.2} & 58.4 \textcolor{gray}{±0.2} & 56.9 \textcolor{gray}{±0.2} \\
\textbf{Libra GradCAM+} & 67.0 \textcolor{gray}{±0.2} (\textcolor{blue}{+13.3\%}) & 57.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.7\%}) & 61.5 \textcolor{gray}{±0.2} (\textcolor{blue}{+12.2\%}) & 68.8 \textcolor{gray}{±0.2} (\textcolor{blue}{+17.8\%}) & 63.6 \textcolor{gray}{±0.2} (\textcolor{blue}{+11.9\%}) \\
\midrule
HiResCAM & 59.3 \textcolor{gray}{±0.2} & 54.3 \textcolor{gray}{±0.1} & 54.7 \textcolor{gray}{±0.2} & 50.0 \textcolor{gray}{±0.2} & 54.6 \textcolor{gray}{±0.2} \\
\textbf{Libra HiResCAM} & 64.7 \textcolor{gray}{±0.2} (\textcolor{blue}{+9.1\%}) & 55.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.4\%}) & 59.5 \textcolor{gray}{±0.2} (\textcolor{blue}{+8.8\%}) & 63.6 \textcolor{gray}{±0.3} (\textcolor{blue}{+27.4\%}) & 60.9 \textcolor{gray}{±0.2} (\textcolor{blue}{+11.6\%}) \\
\midrule
XGradCAM+ & 53.9 \textcolor{gray}{±0.2} & 54.4 \textcolor{gray}{±0.1} & 54.6 \textcolor{gray}{±0.2} & 59.5 \textcolor{gray}{±0.2} & 55.6 \textcolor{gray}{±0.2} \\
\textbf{Libra XGradCAM+} & 68.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+26.2\%}) & 57.4 \textcolor{gray}{±0.2} (\textcolor{blue}{+5.5\%}) & 62.8 \textcolor{gray}{±0.3} (\textcolor{blue}{+14.9\%}) & 71.1 \textcolor{gray}{±0.2} (\textcolor{blue}{+19.5\%}) & 64.8 \textcolor{gray}{±0.2} (\textcolor{blue}{+16.6\%}) \\
\midrule
FullGrad+ & 59.8 \textcolor{gray}{±0.2} & 57.1 \textcolor{gray}{±0.1} & 61.7 \textcolor{gray}{±0.2} & 62.9 \textcolor{gray}{±0.2} & 60.4 \textcolor{gray}{±0.2} \\
\textbf{Libra FullGrad+} & \textbf{69.2} \textcolor{gray}{±0.2} (\textcolor{blue}{+15.6\%}) & \textbf{59.9} \textcolor{gray}{±0.1} (\textcolor{blue}{+4.8\%}) & \textbf{66.6} \textcolor{gray}{±0.2} (\textcolor{blue}{+7.9\%}) & \textbf{73.8} \textcolor{gray}{±0.2} (\textcolor{blue}{+17.4\%}) & \textbf{67.4} \textcolor{gray}{±0.2} (\textcolor{blue}{+11.5\%}) \\
\bottomrule
\end{tabular}
\caption{Cross-dataset analysis of Symmetric Relevance Gain (SRG) AOPC evaluated using ground-truth labels on ViT-B.}
\label{across_models_ds_SRG_gt_AOPC_m_2}
\end{table}


==> files/tables_v1/across_models/ds/SRG_gt_accuracy/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
Method & ImageNet & ImageNet-Hard & MURA & Oxford-IIIT Pet & \textit{Avg.} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-5}
\cmidrule(l){6-6}
Random & 49.9 \textcolor{gray}{±0.1} & 50.1 \textcolor{gray}{±0.1} & 50.3 \textcolor{gray}{±0.1} & 49.7 \textcolor{gray}{±0.1} & 50.0 \textcolor{gray}{±0.1} \\
RawAtt & 58.8 \textcolor{gray}{±0.1} & 52.7 \textcolor{gray}{±0.1} & 54.7 \textcolor{gray}{±0.1} & 61.3 \textcolor{gray}{±0.1} & 56.9 \textcolor{gray}{±0.1} \\
Attention Rollout & 53.9 \textcolor{gray}{±0.1} & 52.3 \textcolor{gray}{±0.1} & 52.5 \textcolor{gray}{±0.1} & 51.9 \textcolor{gray}{±0.1} & 52.6 \textcolor{gray}{±0.1} \\
AliLRP & 54.8 \textcolor{gray}{±0.1} & 53.6 \textcolor{gray}{±0.1} & 53.1 \textcolor{gray}{±0.1} & 53.3 \textcolor{gray}{±0.1} & 53.7 \textcolor{gray}{±0.1} \\
AttnLRP & 57.8 \textcolor{gray}{±0.1} & 57.3 \textcolor{gray}{±0.1} & 54.9 \textcolor{gray}{±0.1} & 59.4 \textcolor{gray}{±0.1} & 57.4 \textcolor{gray}{±0.1} \\
DecompX & 57.6 \textcolor{gray}{±0.1} & 54.8 \textcolor{gray}{±0.1} & 54.7 \textcolor{gray}{±0.1} & 55.1 \textcolor{gray}{±0.1} & 55.6 \textcolor{gray}{±0.1} \\
Integrated Gradients & 60.6 \textcolor{gray}{±0.1} & 59.0 \textcolor{gray}{±0.1} & 58.4 \textcolor{gray}{±0.1} & 57.8 \textcolor{gray}{±0.1} & 59.0 \textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 55.1 \textcolor{gray}{±0.1} & 55.2 \textcolor{gray}{±0.1} & 56.8 \textcolor{gray}{±0.1} & 54.6 \textcolor{gray}{±0.1} & 55.4 \textcolor{gray}{±0.1} \\
\textbf{Libra \IxG{} } & 58.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+6.3\%}) & 55.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.8\%}) & 54.7 \textcolor{gray}{±0.1} (\textcolor{coral}{-3.6\%}) & 55.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.4\%}) & 56.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.4\%}) \\
\midrule
AttCAT & 63.6 \textcolor{gray}{±0.1} & 63.5 \textcolor{gray}{±0.1} & 60.1 \textcolor{gray}{±0.1} & 63.3 \textcolor{gray}{±0.1} & 62.6 \textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \textbf{73.3} \textcolor{gray}{±0.1} (\textcolor{blue}{+15.3\%}) & \underline{65.1} \textcolor{gray}{±0.1} (\textcolor{blue}{+2.6\%}) & \underline{65.1} \textcolor{gray}{±0.1} (\textcolor{blue}{+8.3\%}) & \underline{72.2} \textcolor{gray}{±0.1} (\textcolor{blue}{+14.1\%}) & \underline{68.9} \textcolor{gray}{±0.1} (\textcolor{blue}{+10.1\%}) \\
\midrule
GenAtt & 68.4 \textcolor{gray}{±0.1} & 58.7 \textcolor{gray}{±0.1} & 58.0 \textcolor{gray}{±0.1} & 66.1 \textcolor{gray}{±0.1} & 62.8 \textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 70.1 \textcolor{gray}{±0.1} (\textcolor{blue}{+2.5\%}) & 59.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.5\%}) & 58.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.2\%}) & 67.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.6\%}) & 63.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.3\%}) \\
\midrule
TokenTM & 67.1 \textcolor{gray}{±0.1} & 57.4 \textcolor{gray}{±0.1} & 56.6 \textcolor{gray}{±0.1} & 65.9 \textcolor{gray}{±0.1} & 61.8 \textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 68.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.7\%}) & 57.9 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.8\%}) & 56.6 \textcolor{gray}{±0.1} (+0.0\%) & 66.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+1.0\%}) & 62.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+0.9\%}) \\
\midrule
GradCAM+ & 61.3 \textcolor{gray}{±0.1} & 58.6 \textcolor{gray}{±0.1} & 54.9 \textcolor{gray}{±0.1} & 58.4 \textcolor{gray}{±0.1} & 58.3 \textcolor{gray}{±0.1} \\
\textbf{Libra GradCAM+} & 71.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+17.0\%}) & 61.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+5.0\%}) & 61.6 \textcolor{gray}{±0.1} (\textcolor{blue}{+12.1\%}) & 68.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+16.6\%}) & 65.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+12.7\%}) \\
\midrule
HiResCAM & 61.2 \textcolor{gray}{±0.1} & 57.0 \textcolor{gray}{±0.1} & 54.1 \textcolor{gray}{±0.1} & 49.9 \textcolor{gray}{±0.1} & 55.5 \textcolor{gray}{±0.1} \\
\textbf{Libra HiResCAM} & 68.2 \textcolor{gray}{±0.1} (\textcolor{blue}{+11.5\%}) & 59.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+3.5\%}) & 59.0 \textcolor{gray}{±0.1} (\textcolor{blue}{+9.0\%}) & 62.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+26.0\%}) & 62.3 \textcolor{gray}{±0.1} (\textcolor{blue}{+12.1\%}) \\
\midrule
XGradCAM+ & 55.5 \textcolor{gray}{±0.1} & 57.4 \textcolor{gray}{±0.1} & 54.7 \textcolor{gray}{±0.1} & 59.1 \textcolor{gray}{±0.1} & 56.7 \textcolor{gray}{±0.1} \\
\textbf{Libra XGradCAM+} & 72.7 \textcolor{gray}{±0.1} (\textcolor{blue}{+31.0\%}) & 61.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+7.6\%}) & 62.4 \textcolor{gray}{±0.1} (\textcolor{blue}{+14.0\%}) & 70.5 \textcolor{gray}{±0.1} (\textcolor{blue}{+19.2\%}) & 66.8 \textcolor{gray}{±0.1} (\textcolor{blue}{+17.9\%}) \\
\midrule
FullGrad+ & 61.7 \textcolor{gray}{±0.1} & 61.4 \textcolor{gray}{±0.1} & 61.2 \textcolor{gray}{±0.1} & 62.2 \textcolor{gray}{±0.1} & 61.6 \textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & \textbf{73.3} \textcolor{gray}{±0.1} (\textcolor{blue}{+18.8\%}) & \textbf{65.4} \textcolor{gray}{±0.1} (\textcolor{blue}{+6.5\%}) & \textbf{66.4} \textcolor{gray}{±0.1} (\textcolor{blue}{+8.5\%}) & \textbf{73.3} \textcolor{gray}{±0.1} (\textcolor{blue}{+17.8\%}) & \textbf{69.6} \textcolor{gray}{±0.1} (\textcolor{blue}{+12.9\%}) \\
\bottomrule
\end{tabular}
\caption{Cross-dataset analysis of Symmetric Relevance Gain (SRG) Accuracy evaluated using ground-truth labels on ViT-B.}
\label{across_models_ds_SRG_gt_accuracy_m_2}
\end{table}


==> files/tables_v1/across_models/sel1/LIF_1p_AOPC/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}l}
\toprule
Method & \multicolumn{2}{c}{ViT-L} & \multicolumn{2}{c}{EVA2-S} & \multicolumn{2}{c}{BEiT2-L} & \multicolumn{2}{c}{FlexiViT-L} & \multicolumn{2}{c}{SigLIP-L} & \multicolumn{2}{c}{CLIP-H} & \multicolumn{2}{c}{DeiT3-H} & \multicolumn{2}{c}{\textit{Avg.}} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-15}
\cmidrule(l){16-17}
Random & 83.7& \,\textcolor{gray}{±0.2} & 92.3& \,\textcolor{gray}{±0.2} & 93.2& \,\textcolor{gray}{±0.1} & 93.7& \,\textcolor{gray}{±0.1} & 81.0& \,\textcolor{gray}{±0.1} & 87.5& \,\textcolor{gray}{±0.2} & 81.1& \,\textcolor{gray}{±0.1} & 87.5& \,\textcolor{gray}{±0.2} \\
RawAtt & 81.5& \,\textcolor{gray}{±0.1} & 95.7& \,\textcolor{gray}{±0.1} & 94.9& \,\textcolor{gray}{±0.1} & 95.4& \,\textcolor{gray}{±0.1} & -& & 90.0& \,\textcolor{gray}{±0.2} & 84.3& \,\textcolor{gray}{±0.2} & 90.3& \,\textcolor{gray}{±0.1} \\
Attention Rollout & 81.9& \,\textcolor{gray}{±0.2} & 91.9& \,\textcolor{gray}{±0.2} & 87.4& \,\textcolor{gray}{±0.2} & 86.2& \,\textcolor{gray}{±0.2} & -& & 89.4& \,\textcolor{gray}{±0.2} & 74.8& \,\textcolor{gray}{±0.2} & 85.3& \,\textcolor{gray}{±0.2} \\
AliLRP & 85.9& \,\textcolor{gray}{±0.2} & 100.9& \,\textcolor{gray}{±0.1} & 95.5& \,\textcolor{gray}{±0.1} & 97.8& \,\textcolor{gray}{±0.1} & 89.8& \,\textcolor{gray}{±0.2} & 89.9& \,\textcolor{gray}{±0.1} & 96.0& \,\textcolor{gray}{±0.1} & 93.7& \,\textcolor{gray}{±0.1} \\
AttnLRP & 91.3& \,\textcolor{gray}{±0.2} & 101.9& \,\textcolor{gray}{±0.1} & 96.8& \,\textcolor{gray}{±0.1} & 90.9& \,\textcolor{gray}{±0.2} & 95.0& \,\textcolor{gray}{±0.1} & 96.1& \,\textcolor{gray}{±0.1} & 92.2& \,\textcolor{gray}{±0.2} & 94.9& \,\textcolor{gray}{±0.2} \\
DecompX & 89.3& \,\textcolor{gray}{±0.2} & 99.5& \,\textcolor{gray}{±0.1} & 96.3& \,\textcolor{gray}{±0.1} & 99.6& \,\textcolor{gray}{±0.1} & 90.5& \,\textcolor{gray}{±0.2} & 94.2& \,\textcolor{gray}{±0.2} & 93.4& \,\textcolor{gray}{±0.1} & 94.7& \,\textcolor{gray}{±0.1} \\
Integrated Gradients & 88.4& \,\textcolor{gray}{±0.2} & 99.8& \,\textcolor{gray}{±0.2} & 96.5& \,\textcolor{gray}{±0.2} & 91.9& \,\textcolor{gray}{±0.2} & 91.2& \,\textcolor{gray}{±0.2} & 85.7& \,\textcolor{gray}{±0.1} & 84.9& \,\textcolor{gray}{±0.2} & 91.2& \,\textcolor{gray}{±0.2} \\
\midrule
\IxG{}  & 86.7& \,\textcolor{gray}{±0.1} & 98.9& \,\textcolor{gray}{±0.2} & 93.5& \,\textcolor{gray}{±0.1} & 91.4& \,\textcolor{gray}{±0.2} & 87.6& \,\textcolor{gray}{±0.2} & 84.9& \,\textcolor{gray}{±0.1} & 87.8& \,\textcolor{gray}{±0.2} & 90.1& \,\textcolor{gray}{±0.2} \\
\textbf{Libra \IxG{} } & 90.2& \,\textcolor{gray}{±0.2} & 102.5& \,\textcolor{gray}{±0.1} & 96.9& \,\textcolor{gray}{±0.1} & 100.4& \,\textcolor{gray}{±0.1} & 90.6& \,\textcolor{gray}{±0.2} & 94.7& \,\textcolor{gray}{±0.2} & 94.0& \,\textcolor{gray}{±0.2} & 95.6& \,\textcolor{gray}{±0.1} \\
\midrule
AttCAT & 92.6& \,\textcolor{gray}{±0.2} & \textbf{105.3}& \,\textcolor{gray}{±0.1} & \textbf{100.0}& \,\textcolor{gray}{±0.1} & \textbf{104.5}& \,\textcolor{gray}{±0.2} & 92.4& \,\textcolor{gray}{±0.2} & 94.8& \,\textcolor{gray}{±0.2} & 90.6& \,\textcolor{gray}{±0.2} & 97.2& \,\textcolor{gray}{±0.2} \\
\textbf{Libra AttCAT} & \underline{97.1}& \,\textcolor{gray}{±0.2} & 102.8& \,\textcolor{gray}{±0.1} & 97.9& \,\textcolor{gray}{±0.1} & 103.0& \,\textcolor{gray}{±0.1} & \textbf{98.4}& \,\textcolor{gray}{±0.1} & \underline{96.4}& \,\textcolor{gray}{±0.1} & \underline{98.6}& \,\textcolor{gray}{±0.1} & \underline{99.2}& \,\textcolor{gray}{±0.1} \\
\midrule
GenAtt & 91.5& \,\textcolor{gray}{±0.2} & 94.0& \,\textcolor{gray}{±0.2} & 94.4& \,\textcolor{gray}{±0.1} & 99.7& \,\textcolor{gray}{±0.1} & -& & 94.3& \,\textcolor{gray}{±0.2} & 93.6& \,\textcolor{gray}{±0.1} & 94.6& \,\textcolor{gray}{±0.2} \\
\textbf{Libra GenAtt} & 92.0& \,\textcolor{gray}{±0.2} & 94.5& \,\textcolor{gray}{±0.2} & 94.3& \,\textcolor{gray}{±0.2} & 99.4& \,\textcolor{gray}{±0.1} & -& & 94.5& \,\textcolor{gray}{±0.1} & 94.0& \,\textcolor{gray}{±0.1} & 94.8& \,\textcolor{gray}{±0.2} \\
\midrule
TokenTM & 90.3& \,\textcolor{gray}{±0.2} & 95.2& \,\textcolor{gray}{±0.1} & 95.5& \,\textcolor{gray}{±0.1} & 98.5& \,\textcolor{gray}{±0.1} & -& & 93.4& \,\textcolor{gray}{±0.1} & 93.0& \,\textcolor{gray}{±0.1} & 94.3& \,\textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 90.8& \,\textcolor{gray}{±0.2} & 94.8& \,\textcolor{gray}{±0.2} & 94.6& \,\textcolor{gray}{±0.1} & 98.6& \,\textcolor{gray}{±0.1} & -& & 93.6& \,\textcolor{gray}{±0.1} & 93.3& \,\textcolor{gray}{±0.2} & 94.3& \,\textcolor{gray}{±0.1} \\
\midrule
GradCAM+ & 91.0& \,\textcolor{gray}{±0.2} & 98.6& \,\textcolor{gray}{±0.2} & 97.1& \,\textcolor{gray}{±0.1} & 85.7& \,\textcolor{gray}{±0.2} & 60.7& \,\textcolor{gray}{±0.3} & 85.6& \,\textcolor{gray}{±0.2} & 84.4& \,\textcolor{gray}{±0.2} & 86.2& \,\textcolor{gray}{±0.2} \\
\textbf{Libra GradCAM+} & 92.7& \,\textcolor{gray}{±0.2} & 100.3& \,\textcolor{gray}{±0.1} & 95.6& \,\textcolor{gray}{±0.1} & 93.8& \,\textcolor{gray}{±0.1} & 80.8& \,\textcolor{gray}{±0.2} & 86.4& \,\textcolor{gray}{±0.2} & 89.8& \,\textcolor{gray}{±0.2} & 91.3& \,\textcolor{gray}{±0.2} \\
\midrule
HiResCAM & 74.2& \,\textcolor{gray}{±0.3} & 101.0& \,\textcolor{gray}{±0.1} & 97.0& \,\textcolor{gray}{±0.1} & 91.2& \,\textcolor{gray}{±0.2} & 66.3& \,\textcolor{gray}{±0.3} & 92.7& \,\textcolor{gray}{±0.2} & 84.2& \,\textcolor{gray}{±0.1} & 86.6& \,\textcolor{gray}{±0.2} \\
\textbf{Libra HiResCAM} & 88.0& \,\textcolor{gray}{±0.2} & 100.5& \,\textcolor{gray}{±0.1} & 97.1& \,\textcolor{gray}{±0.1} & 101.6& \,\textcolor{gray}{±0.1} & 82.6& \,\textcolor{gray}{±0.2} & 94.1& \,\textcolor{gray}{±0.1} & 86.9& \,\textcolor{gray}{±0.2} & 93.0& \,\textcolor{gray}{±0.2} \\
\midrule
XGradCAM+ & 90.1& \,\textcolor{gray}{±0.2} & 99.7& \,\textcolor{gray}{±0.2} & 96.4& \,\textcolor{gray}{±0.1} & 84.7& \,\textcolor{gray}{±0.3} & 75.2& \,\textcolor{gray}{±0.3} & 90.6& \,\textcolor{gray}{±0.2} & 87.3& \,\textcolor{gray}{±0.2} & 89.2& \,\textcolor{gray}{±0.2} \\
\textbf{Libra XGradCAM+} & 93.7& \,\textcolor{gray}{±0.2} & 100.3& \,\textcolor{gray}{±0.1} & 96.6& \,\textcolor{gray}{±0.1} & 99.0& \,\textcolor{gray}{±0.1} & 88.4& \,\textcolor{gray}{±0.2} & 93.9& \,\textcolor{gray}{±0.2} & 95.3& \,\textcolor{gray}{±0.1} & 95.3& \,\textcolor{gray}{±0.1} \\
\midrule
FullGrad+ & 91.8& \,\textcolor{gray}{±0.2} & \underline{104.5}& \,\textcolor{gray}{±0.2} & \underline{98.0}& \,\textcolor{gray}{±0.1} & \underline{103.2}& \,\textcolor{gray}{±0.2} & 89.3& \,\textcolor{gray}{±0.2} & 93.4& \,\textcolor{gray}{±0.2} & 90.1& \,\textcolor{gray}{±0.2} & 95.8& \,\textcolor{gray}{±0.2} \\
\textbf{Libra FullGrad+} & \textbf{97.4}& \,\textcolor{gray}{±0.2} & 103.0& \,\textcolor{gray}{±0.1} & \underline{98.0}& \,\textcolor{gray}{±0.1} & 103.0& \,\textcolor{gray}{±0.1} & \underline{98.2}& \,\textcolor{gray}{±0.1} & \textbf{96.8}& \,\textcolor{gray}{±0.2} & \textbf{98.8}& \,\textcolor{gray}{±0.1} & \textbf{99.3}& \,\textcolor{gray}{±0.1} \\
\bottomrule
\end{tabular}
\caption{Least-Influential-First Deletion (LIF) AOPC evaluated using predicted labels across multiple models.}
\label{across_models_sel1_LIF_1p_AOPC_m_2}
\end{table}


==> files/tables_v1/across_models/sel1/LIF_1p_accuracy/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}l}
\toprule
Method & \multicolumn{2}{c}{ViT-L} & \multicolumn{2}{c}{EVA2-S} & \multicolumn{2}{c}{BEiT2-L} & \multicolumn{2}{c}{FlexiViT-L} & \multicolumn{2}{c}{SigLIP-L} & \multicolumn{2}{c}{CLIP-H} & \multicolumn{2}{c}{DeiT3-H} & \multicolumn{2}{c}{\textit{Avg.}} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-15}
\cmidrule(l){16-17}
Random & 70.2& \,\textcolor{gray}{±0.1} & 79.0& \,\textcolor{gray}{±0.1} & 81.7& \,\textcolor{gray}{±0.1} & 80.7& \,\textcolor{gray}{±0.1} & 67.1& \,\textcolor{gray}{±0.1} & 72.4& \,\textcolor{gray}{±0.1} & 70.7& \,\textcolor{gray}{±0.1} & 74.5& \,\textcolor{gray}{±0.1} \\
RawAtt & 67.6& \,\textcolor{gray}{±0.1} & 82.7& \,\textcolor{gray}{±0.1} & 83.7& \,\textcolor{gray}{±0.1} & 82.6& \,\textcolor{gray}{±0.1} & -& & 76.0& \,\textcolor{gray}{±0.1} & 78.4& \,\textcolor{gray}{±0.1} & 78.5& \,\textcolor{gray}{±0.1} \\
Attention Rollout & 68.3& \,\textcolor{gray}{±0.1} & 78.8& \,\textcolor{gray}{±0.1} & 75.6& \,\textcolor{gray}{±0.1} & 72.7& \,\textcolor{gray}{±0.1} & -& & 74.6& \,\textcolor{gray}{±0.1} & 64.5& \,\textcolor{gray}{±0.1} & 72.4& \,\textcolor{gray}{±0.1} \\
AliLRP & 72.5& \,\textcolor{gray}{±0.1} & 87.2& \,\textcolor{gray}{±0.1} & 84.5& \,\textcolor{gray}{±0.1} & 84.7& \,\textcolor{gray}{±0.1} & 77.0& \,\textcolor{gray}{±0.1} & 75.3& \,\textcolor{gray}{±0.1} & 86.1& \,\textcolor{gray}{±0.1} & 81.0& \,\textcolor{gray}{±0.1} \\
AttnLRP & 77.6& \,\textcolor{gray}{±0.1} & 87.5& \,\textcolor{gray}{±0.0} & 85.7& \,\textcolor{gray}{±0.1} & 77.9& \,\textcolor{gray}{±0.1} & 82.2& \,\textcolor{gray}{±0.1} & 83.3& \,\textcolor{gray}{±0.1} & 80.8& \,\textcolor{gray}{±0.1} & 82.2& \,\textcolor{gray}{±0.1} \\
DecompX & 75.8& \,\textcolor{gray}{±0.1} & 85.8& \,\textcolor{gray}{±0.1} & 84.9& \,\textcolor{gray}{±0.1} & 86.2& \,\textcolor{gray}{±0.1} & 78.1& \,\textcolor{gray}{±0.1} & 81.7& \,\textcolor{gray}{±0.1} & 83.1& \,\textcolor{gray}{±0.1} & 82.2& \,\textcolor{gray}{±0.1} \\
Integrated Gradients & 73.5& \,\textcolor{gray}{±0.1} & 83.5& \,\textcolor{gray}{±0.1} & 84.2& \,\textcolor{gray}{±0.1} & 77.7& \,\textcolor{gray}{±0.1} & 75.6& \,\textcolor{gray}{±0.1} & 69.4& \,\textcolor{gray}{±0.1} & 74.6& \,\textcolor{gray}{±0.1} & 76.9& \,\textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 72.8& \,\textcolor{gray}{±0.1} & 84.0& \,\textcolor{gray}{±0.1} & 82.0& \,\textcolor{gray}{±0.1} & 78.3& \,\textcolor{gray}{±0.1} & 71.6& \,\textcolor{gray}{±0.1} & 68.8& \,\textcolor{gray}{±0.1} & 77.7& \,\textcolor{gray}{±0.1} & 76.5& \,\textcolor{gray}{±0.1} \\
\textbf{Libra \IxG{} } & 76.7& \,\textcolor{gray}{±0.1} & \underline{88.3}& \,\textcolor{gray}{±0.0} & 85.7& \,\textcolor{gray}{±0.1} & 86.9& \,\textcolor{gray}{±0.1} & 78.3& \,\textcolor{gray}{±0.1} & 82.2& \,\textcolor{gray}{±0.1} & 83.7& \,\textcolor{gray}{±0.1} & 83.1& \,\textcolor{gray}{±0.1} \\
\midrule
AttCAT & 77.5& \,\textcolor{gray}{±0.1} & 87.8& \,\textcolor{gray}{±0.0} & \textbf{87.5}& \,\textcolor{gray}{±0.0} & \underline{88.3}& \,\textcolor{gray}{±0.0} & 76.6& \,\textcolor{gray}{±0.1} & 76.9& \,\textcolor{gray}{±0.1} & 80.5& \,\textcolor{gray}{±0.1} & 82.2& \,\textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \underline{82.2}& \,\textcolor{gray}{±0.1} & \underline{88.3}& \,\textcolor{gray}{±0.0} & \underline{87.0}& \,\textcolor{gray}{±0.1} & \textbf{88.5}& \,\textcolor{gray}{±0.0} & \textbf{85.9}& \,\textcolor{gray}{±0.1} & \underline{83.8}& \,\textcolor{gray}{±0.1} & \textbf{87.7}& \,\textcolor{gray}{±0.0} & \underline{86.2}& \,\textcolor{gray}{±0.1} \\
\midrule
GenAtt & 78.2& \,\textcolor{gray}{±0.1} & 80.7& \,\textcolor{gray}{±0.1} & 83.2& \,\textcolor{gray}{±0.1} & 87.0& \,\textcolor{gray}{±0.1} & -& & 80.8& \,\textcolor{gray}{±0.1} & 85.7& \,\textcolor{gray}{±0.1} & 82.6& \,\textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 78.8& \,\textcolor{gray}{±0.1} & 81.6& \,\textcolor{gray}{±0.1} & 83.2& \,\textcolor{gray}{±0.1} & 86.6& \,\textcolor{gray}{±0.1} & -& & 82.5& \,\textcolor{gray}{±0.1} & 86.0& \,\textcolor{gray}{±0.1} & 83.1& \,\textcolor{gray}{±0.1} \\
\midrule
TokenTM & 77.3& \,\textcolor{gray}{±0.1} & 82.1& \,\textcolor{gray}{±0.1} & 84.6& \,\textcolor{gray}{±0.1} & 86.0& \,\textcolor{gray}{±0.1} & -& & 80.6& \,\textcolor{gray}{±0.1} & 85.0& \,\textcolor{gray}{±0.1} & 82.6& \,\textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 77.8& \,\textcolor{gray}{±0.1} & 81.9& \,\textcolor{gray}{±0.1} & 83.8& \,\textcolor{gray}{±0.1} & 85.8& \,\textcolor{gray}{±0.1} & -& & 81.7& \,\textcolor{gray}{±0.1} & 85.4& \,\textcolor{gray}{±0.1} & 82.7& \,\textcolor{gray}{±0.1} \\
\midrule
GradCAM+ & 76.8& \,\textcolor{gray}{±0.1} & 82.8& \,\textcolor{gray}{±0.1} & 85.1& \,\textcolor{gray}{±0.1} & 72.3& \,\textcolor{gray}{±0.1} & 49.0& \,\textcolor{gray}{±0.1} & 69.4& \,\textcolor{gray}{±0.1} & 75.8& \,\textcolor{gray}{±0.1} & 73.0& \,\textcolor{gray}{±0.1} \\
\textbf{Libra GradCAM+} & 79.1& \,\textcolor{gray}{±0.1} & 86.4& \,\textcolor{gray}{±0.1} & 84.2& \,\textcolor{gray}{±0.1} & 80.6& \,\textcolor{gray}{±0.1} & 67.5& \,\textcolor{gray}{±0.1} & 70.7& \,\textcolor{gray}{±0.1} & 80.7& \,\textcolor{gray}{±0.1} & 78.5& \,\textcolor{gray}{±0.1} \\
\midrule
HiResCAM & 59.3& \,\textcolor{gray}{±0.1} & 86.1& \,\textcolor{gray}{±0.1} & 85.5& \,\textcolor{gray}{±0.1} & 78.7& \,\textcolor{gray}{±0.1} & 51.9& \,\textcolor{gray}{±0.1} & 77.9& \,\textcolor{gray}{±0.1} & 75.5& \,\textcolor{gray}{±0.1} & 73.5& \,\textcolor{gray}{±0.1} \\
\textbf{Libra HiResCAM} & 73.8& \,\textcolor{gray}{±0.1} & 86.3& \,\textcolor{gray}{±0.1} & 86.0& \,\textcolor{gray}{±0.1} & 87.3& \,\textcolor{gray}{±0.0} & 68.2& \,\textcolor{gray}{±0.1} & 80.9& \,\textcolor{gray}{±0.1} & 80.6& \,\textcolor{gray}{±0.1} & 80.5& \,\textcolor{gray}{±0.1} \\
\midrule
XGradCAM+ & 75.7& \,\textcolor{gray}{±0.1} & 83.8& \,\textcolor{gray}{±0.1} & 84.3& \,\textcolor{gray}{±0.1} & 72.3& \,\textcolor{gray}{±0.1} & 60.6& \,\textcolor{gray}{±0.1} & 75.4& \,\textcolor{gray}{±0.1} & 77.1& \,\textcolor{gray}{±0.1} & 75.6& \,\textcolor{gray}{±0.1} \\
\textbf{Libra XGradCAM+} & 80.0& \,\textcolor{gray}{±0.1} & 86.6& \,\textcolor{gray}{±0.1} & 85.6& \,\textcolor{gray}{±0.1} & 85.3& \,\textcolor{gray}{±0.1} & 76.4& \,\textcolor{gray}{±0.1} & 81.0& \,\textcolor{gray}{±0.1} & 86.4& \,\textcolor{gray}{±0.1} & 83.0& \,\textcolor{gray}{±0.1} \\
\midrule
FullGrad+ & 76.8& \,\textcolor{gray}{±0.1} & 86.8& \,\textcolor{gray}{±0.1} & 86.0& \,\textcolor{gray}{±0.1} & 87.8& \,\textcolor{gray}{±0.0} & 73.3& \,\textcolor{gray}{±0.1} & 76.2& \,\textcolor{gray}{±0.1} & 79.9& \,\textcolor{gray}{±0.1} & 81.0& \,\textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & \textbf{82.6}& \,\textcolor{gray}{±0.1} & \textbf{88.5}& \,\textcolor{gray}{±0.0} & 86.9& \,\textcolor{gray}{±0.1} & \underline{88.3}& \,\textcolor{gray}{±0.0} & \underline{85.8}& \,\textcolor{gray}{±0.1} & \textbf{84.9}& \,\textcolor{gray}{±0.1} & \underline{87.6}& \,\textcolor{gray}{±0.0} & \textbf{86.4}& \,\textcolor{gray}{±0.1} \\
\bottomrule
\end{tabular}
\caption{Least-Influential-First Deletion (LIF) Accuracy evaluated using predicted labels across multiple models.}
\label{across_models_sel1_LIF_1p_accuracy_m_2}
\end{table}


==> files/tables_v1/across_models/sel1/LIF_gt_AOPC/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}l}
\toprule
Method & \multicolumn{2}{c}{ViT-L} & \multicolumn{2}{c}{EVA2-S} & \multicolumn{2}{c}{BEiT2-L} & \multicolumn{2}{c}{FlexiViT-L} & \multicolumn{2}{c}{SigLIP-L} & \multicolumn{2}{c}{CLIP-H} & \multicolumn{2}{c}{DeiT3-H} & \multicolumn{2}{c}{\textit{Avg.}} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-15}
\cmidrule(l){16-17}
Random & 85.4& \,\textcolor{gray}{±0.2} & 93.5& \,\textcolor{gray}{±0.2} & 94.1& \,\textcolor{gray}{±0.1} & 94.7& \,\textcolor{gray}{±0.2} & 82.7& \,\textcolor{gray}{±0.2} & 88.8& \,\textcolor{gray}{±0.2} & 83.5& \,\textcolor{gray}{±0.2} & 89.0& \,\textcolor{gray}{±0.2} \\
RawAtt & 83.3& \,\textcolor{gray}{±0.2} & 96.9& \,\textcolor{gray}{±0.1} & 95.8& \,\textcolor{gray}{±0.1} & 96.6& \,\textcolor{gray}{±0.1} & -& & 91.1& \,\textcolor{gray}{±0.1} & 86.3& \,\textcolor{gray}{±0.2} & 91.7& \,\textcolor{gray}{±0.1} \\
Attention Rollout & 84.1& \,\textcolor{gray}{±0.2} & 93.6& \,\textcolor{gray}{±0.2} & 89.1& \,\textcolor{gray}{±0.2} & 88.2& \,\textcolor{gray}{±0.2} & -& & 90.7& \,\textcolor{gray}{±0.2} & 77.9& \,\textcolor{gray}{±0.3} & 87.3& \,\textcolor{gray}{±0.2} \\
AliLRP & 87.7& \,\textcolor{gray}{±0.2} & 102.6& \,\textcolor{gray}{±0.2} & 96.7& \,\textcolor{gray}{±0.1} & 98.9& \,\textcolor{gray}{±0.1} & 91.2& \,\textcolor{gray}{±0.2} & 91.3& \,\textcolor{gray}{±0.1} & 97.5& \,\textcolor{gray}{±0.2} & 95.1& \,\textcolor{gray}{±0.2} \\
AttnLRP & 92.9& \,\textcolor{gray}{±0.2} & 103.0& \,\textcolor{gray}{±0.1} & 97.8& \,\textcolor{gray}{±0.1} & 92.2& \,\textcolor{gray}{±0.2} & 96.0& \,\textcolor{gray}{±0.2} & 97.3& \,\textcolor{gray}{±0.2} & 94.2& \,\textcolor{gray}{±0.2} & 96.2& \,\textcolor{gray}{±0.2} \\
DecompX & 91.0& \,\textcolor{gray}{±0.2} & 100.4& \,\textcolor{gray}{±0.1} & 97.2& \,\textcolor{gray}{±0.1} & 100.6& \,\textcolor{gray}{±0.1} & 91.8& \,\textcolor{gray}{±0.2} & 95.4& \,\textcolor{gray}{±0.2} & 95.2& \,\textcolor{gray}{±0.2} & 95.9& \,\textcolor{gray}{±0.2} \\
Integrated Gradients & 93.3& \,\textcolor{gray}{±0.2} & 105.3& \,\textcolor{gray}{±0.2} & 98.8& \,\textcolor{gray}{±0.1} & 93.8& \,\textcolor{gray}{±0.2} & 97.0& \,\textcolor{gray}{±0.3} & 87.2& \,\textcolor{gray}{±0.1} & 91.2& \,\textcolor{gray}{±0.3} & 95.2& \,\textcolor{gray}{±0.2} \\
\midrule
\IxG{}  & 88.4& \,\textcolor{gray}{±0.2} & 100.0& \,\textcolor{gray}{±0.2} & 94.5& \,\textcolor{gray}{±0.1} & 92.8& \,\textcolor{gray}{±0.2} & 89.7& \,\textcolor{gray}{±0.3} & 86.5& \,\textcolor{gray}{±0.2} & 90.5& \,\textcolor{gray}{±0.2} & 91.8& \,\textcolor{gray}{±0.2} \\
\textbf{Libra \IxG{} } & 92.0& \,\textcolor{gray}{±0.2} & 104.7& \,\textcolor{gray}{±0.1} & 98.1& \,\textcolor{gray}{±0.1} & 101.6& \,\textcolor{gray}{±0.1} & 91.9& \,\textcolor{gray}{±0.3} & 96.3& \,\textcolor{gray}{±0.2} & 95.8& \,\textcolor{gray}{±0.2} & 97.2& \,\textcolor{gray}{±0.2} \\
\midrule
AttCAT & 94.3& \,\textcolor{gray}{±0.2} & \textbf{107.2}& \,\textcolor{gray}{±0.2} & \textbf{101.1}& \,\textcolor{gray}{±0.1} & \textbf{106.1}& \,\textcolor{gray}{±0.2} & 95.3& \,\textcolor{gray}{±0.3} & 96.3& \,\textcolor{gray}{±0.2} & 93.6& \,\textcolor{gray}{±0.2} & 99.1& \,\textcolor{gray}{±0.2} \\
\textbf{Libra AttCAT} & \underline{98.5}& \,\textcolor{gray}{±0.2} & 105.0& \,\textcolor{gray}{±0.1} & 99.2& \,\textcolor{gray}{±0.1} & 104.4& \,\textcolor{gray}{±0.1} & \textbf{99.6}& \,\textcolor{gray}{±0.2} & \underline{98.1}& \,\textcolor{gray}{±0.1} & \underline{100.0}& \,\textcolor{gray}{±0.2} & \underline{100.7}& \,\textcolor{gray}{±0.2} \\
\midrule
GenAtt & 92.8& \,\textcolor{gray}{±0.2} & 95.3& \,\textcolor{gray}{±0.2} & 95.2& \,\textcolor{gray}{±0.1} & 100.8& \,\textcolor{gray}{±0.1} & -& & 95.3& \,\textcolor{gray}{±0.2} & 94.9& \,\textcolor{gray}{±0.2} & 95.7& \,\textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 93.2& \,\textcolor{gray}{±0.2} & 95.9& \,\textcolor{gray}{±0.2} & 95.2& \,\textcolor{gray}{±0.2} & 100.5& \,\textcolor{gray}{±0.1} & -& & 95.5& \,\textcolor{gray}{±0.1} & 95.3& \,\textcolor{gray}{±0.2} & 95.9& \,\textcolor{gray}{±0.1} \\
\midrule
TokenTM & 91.6& \,\textcolor{gray}{±0.2} & 96.6& \,\textcolor{gray}{±0.2} & 96.2& \,\textcolor{gray}{±0.1} & 99.6& \,\textcolor{gray}{±0.1} & -& & 94.5& \,\textcolor{gray}{±0.1} & 94.2& \,\textcolor{gray}{±0.2} & 95.4& \,\textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 92.1& \,\textcolor{gray}{±0.2} & 96.3& \,\textcolor{gray}{±0.2} & 95.5& \,\textcolor{gray}{±0.1} & 99.6& \,\textcolor{gray}{±0.1} & -& & 94.6& \,\textcolor{gray}{±0.1} & 94.6& \,\textcolor{gray}{±0.2} & 95.4& \,\textcolor{gray}{±0.1} \\
\midrule
GradCAM+ & 92.9& \,\textcolor{gray}{±0.2} & 100.8& \,\textcolor{gray}{±0.3} & 98.5& \,\textcolor{gray}{±0.2} & 87.5& \,\textcolor{gray}{±0.2} & 64.3& \,\textcolor{gray}{±0.4} & 87.4& \,\textcolor{gray}{±0.2} & 86.7& \,\textcolor{gray}{±0.2} & 88.3& \,\textcolor{gray}{±0.2} \\
\textbf{Libra GradCAM+} & 94.4& \,\textcolor{gray}{±0.2} & 102.6& \,\textcolor{gray}{±0.1} & 97.1& \,\textcolor{gray}{±0.1} & 95.5& \,\textcolor{gray}{±0.1} & 83.0& \,\textcolor{gray}{±0.3} & 88.4& \,\textcolor{gray}{±0.3} & 91.9& \,\textcolor{gray}{±0.2} & 93.3& \,\textcolor{gray}{±0.2} \\
\midrule
HiResCAM & 76.7& \,\textcolor{gray}{±0.2} & 103.1& \,\textcolor{gray}{±0.2} & 98.3& \,\textcolor{gray}{±0.1} & 92.6& \,\textcolor{gray}{±0.2} & 69.4& \,\textcolor{gray}{±0.4} & 94.3& \,\textcolor{gray}{±0.2} & 86.2& \,\textcolor{gray}{±0.2} & 88.7& \,\textcolor{gray}{±0.2} \\
\textbf{Libra HiResCAM} & 90.0& \,\textcolor{gray}{±0.2} & 102.4& \,\textcolor{gray}{±0.2} & 98.4& \,\textcolor{gray}{±0.1} & 103.4& \,\textcolor{gray}{±0.1} & 84.8& \,\textcolor{gray}{±0.3} & 95.6& \,\textcolor{gray}{±0.1} & 89.8& \,\textcolor{gray}{±0.3} & 94.9& \,\textcolor{gray}{±0.2} \\
\midrule
XGradCAM+ & 92.1& \,\textcolor{gray}{±0.2} & 101.9& \,\textcolor{gray}{±0.3} & 97.9& \,\textcolor{gray}{±0.2} & 86.6& \,\textcolor{gray}{±0.3} & 78.4& \,\textcolor{gray}{±0.4} & 92.1& \,\textcolor{gray}{±0.2} & 89.9& \,\textcolor{gray}{±0.3} & 91.3& \,\textcolor{gray}{±0.3} \\
\textbf{Libra XGradCAM+} & 95.3& \,\textcolor{gray}{±0.2} & 102.6& \,\textcolor{gray}{±0.1} & 98.0& \,\textcolor{gray}{±0.1} & 100.4& \,\textcolor{gray}{±0.1} & 89.8& \,\textcolor{gray}{±0.3} & 95.8& \,\textcolor{gray}{±0.1} & 97.0& \,\textcolor{gray}{±0.2} & 97.0& \,\textcolor{gray}{±0.2} \\
\midrule
FullGrad+ & 93.8& \,\textcolor{gray}{±0.2} & \underline{106.6}& \,\textcolor{gray}{±0.3} & 98.9& \,\textcolor{gray}{±0.1} & 104.3& \,\textcolor{gray}{±0.2} & 92.2& \,\textcolor{gray}{±0.3} & 95.0& \,\textcolor{gray}{±0.2} & 92.8& \,\textcolor{gray}{±0.2} & 97.7& \,\textcolor{gray}{±0.2} \\
\textbf{Libra FullGrad+} & \textbf{98.9}& \,\textcolor{gray}{±0.2} & 105.3& \,\textcolor{gray}{±0.2} & \underline{99.3}& \,\textcolor{gray}{±0.1} & \underline{104.5}& \,\textcolor{gray}{±0.1} & \underline{99.4}& \,\textcolor{gray}{±0.2} & \textbf{98.4}& \,\textcolor{gray}{±0.1} & \textbf{100.4}& \,\textcolor{gray}{±0.2} & \textbf{100.9}& \,\textcolor{gray}{±0.2} \\
\bottomrule
\end{tabular}
\caption{Least-Influential-First Deletion (LIF) AOPC evaluated using ground-truth labels across multiple models.}
\label{across_models_sel1_LIF_gt_AOPC_m_2}
\end{table}


==> files/tables_v1/across_models/sel1/LIF_gt_accuracy/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}l}
\toprule
Method & \multicolumn{2}{c}{ViT-L} & \multicolumn{2}{c}{EVA2-S} & \multicolumn{2}{c}{BEiT2-L} & \multicolumn{2}{c}{FlexiViT-L} & \multicolumn{2}{c}{SigLIP-L} & \multicolumn{2}{c}{CLIP-H} & \multicolumn{2}{c}{DeiT3-H} & \multicolumn{2}{c}{\textit{Avg.}} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-15}
\cmidrule(l){16-17}
Random & 62.9& \,\textcolor{gray}{±0.1} & 70.0& \,\textcolor{gray}{±0.1} & 74.6& \,\textcolor{gray}{±0.1} & 70.7& \,\textcolor{gray}{±0.1} & 61.1& \,\textcolor{gray}{±0.1} & 65.8& \,\textcolor{gray}{±0.1} & 64.2& \,\textcolor{gray}{±0.1} & 67.0& \,\textcolor{gray}{±0.1} \\
RawAtt & 60.3& \,\textcolor{gray}{±0.1} & 73.3& \,\textcolor{gray}{±0.1} & 76.6& \,\textcolor{gray}{±0.1} & 72.8& \,\textcolor{gray}{±0.1} & -& & 68.7& \,\textcolor{gray}{±0.1} & 70.9& \,\textcolor{gray}{±0.1} & 70.4& \,\textcolor{gray}{±0.1} \\
Attention Rollout & 61.9& \,\textcolor{gray}{±0.1} & 70.1& \,\textcolor{gray}{±0.1} & 69.9& \,\textcolor{gray}{±0.1} & 65.0& \,\textcolor{gray}{±0.1} & -& & 68.1& \,\textcolor{gray}{±0.1} & 59.0& \,\textcolor{gray}{±0.1} & 65.7& \,\textcolor{gray}{±0.1} \\
AliLRP & 65.4& \,\textcolor{gray}{±0.1} & 79.7& \,\textcolor{gray}{±0.1} & 78.0& \,\textcolor{gray}{±0.1} & 75.8& \,\textcolor{gray}{±0.1} & 70.8& \,\textcolor{gray}{±0.1} & 69.1& \,\textcolor{gray}{±0.1} & 79.5& \,\textcolor{gray}{±0.1} & 74.0& \,\textcolor{gray}{±0.1} \\
AttnLRP & 70.3& \,\textcolor{gray}{±0.1} & 78.8& \,\textcolor{gray}{±0.1} & 78.4& \,\textcolor{gray}{±0.1} & 68.9& \,\textcolor{gray}{±0.1} & 75.0& \,\textcolor{gray}{±0.1} & 76.8& \,\textcolor{gray}{±0.1} & 74.1& \,\textcolor{gray}{±0.1} & 74.6& \,\textcolor{gray}{±0.1} \\
DecompX & 68.8& \,\textcolor{gray}{±0.1} & 76.3& \,\textcolor{gray}{±0.1} & 77.6& \,\textcolor{gray}{±0.1} & 76.7& \,\textcolor{gray}{±0.1} & 71.3& \,\textcolor{gray}{±0.1} & 74.8& \,\textcolor{gray}{±0.1} & 75.8& \,\textcolor{gray}{±0.1} & 74.5& \,\textcolor{gray}{±0.1} \\
Integrated Gradients & 71.1& \,\textcolor{gray}{±0.1} & 82.0& \,\textcolor{gray}{±0.1} & 79.4& \,\textcolor{gray}{±0.1} & 70.2& \,\textcolor{gray}{±0.1} & 75.9& \,\textcolor{gray}{±0.1} & 63.3& \,\textcolor{gray}{±0.1} & 71.5& \,\textcolor{gray}{±0.1} & 73.3& \,\textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 65.8& \,\textcolor{gray}{±0.1} & 76.5& \,\textcolor{gray}{±0.1} & 75.5& \,\textcolor{gray}{±0.1} & 69.6& \,\textcolor{gray}{±0.1} & 67.4& \,\textcolor{gray}{±0.1} & 62.7& \,\textcolor{gray}{±0.1} & 71.9& \,\textcolor{gray}{±0.1} & 69.9& \,\textcolor{gray}{±0.1} \\
\textbf{Libra \IxG{} } & 70.1& \,\textcolor{gray}{±0.1} & 82.0& \,\textcolor{gray}{±0.1} & 79.2& \,\textcolor{gray}{±0.1} & 78.2& \,\textcolor{gray}{±0.1} & 71.8& \,\textcolor{gray}{±0.1} & 76.0& \,\textcolor{gray}{±0.1} & 77.1& \,\textcolor{gray}{±0.1} & 76.3& \,\textcolor{gray}{±0.1} \\
\midrule
AttCAT & 71.8& \,\textcolor{gray}{±0.1} & \textbf{82.7}& \,\textcolor{gray}{±0.1} & \textbf{81.8}& \,\textcolor{gray}{±0.1} & \textbf{83.1}& \,\textcolor{gray}{±0.1} & 73.8& \,\textcolor{gray}{±0.1} & 72.3& \,\textcolor{gray}{±0.1} & 75.3& \,\textcolor{gray}{±0.1} & 77.3& \,\textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \underline{76.3}& \,\textcolor{gray}{±0.1} & 82.2& \,\textcolor{gray}{±0.1} & \underline{80.8}& \,\textcolor{gray}{±0.1} & 81.4& \,\textcolor{gray}{±0.1} & \textbf{80.0}& \,\textcolor{gray}{±0.1} & \underline{78.1}& \,\textcolor{gray}{±0.1} & \underline{81.7}& \,\textcolor{gray}{±0.1} & \underline{80.1}& \,\textcolor{gray}{±0.1} \\
\midrule
GenAtt & 70.0& \,\textcolor{gray}{±0.1} & 71.9& \,\textcolor{gray}{±0.1} & 75.6& \,\textcolor{gray}{±0.1} & 77.3& \,\textcolor{gray}{±0.1} & -& & 73.4& \,\textcolor{gray}{±0.1} & 76.9& \,\textcolor{gray}{±0.1} & 74.2& \,\textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 70.9& \,\textcolor{gray}{±0.1} & 72.7& \,\textcolor{gray}{±0.1} & 75.5& \,\textcolor{gray}{±0.1} & 77.0& \,\textcolor{gray}{±0.1} & -& & 75.0& \,\textcolor{gray}{±0.1} & 77.3& \,\textcolor{gray}{±0.1} & 74.7& \,\textcolor{gray}{±0.1} \\
\midrule
TokenTM & 68.9& \,\textcolor{gray}{±0.1} & 73.3& \,\textcolor{gray}{±0.1} & 76.8& \,\textcolor{gray}{±0.1} & 76.0& \,\textcolor{gray}{±0.1} & -& & 73.1& \,\textcolor{gray}{±0.1} & 76.2& \,\textcolor{gray}{±0.1} & 74.0& \,\textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 69.4& \,\textcolor{gray}{±0.1} & 72.9& \,\textcolor{gray}{±0.1} & 76.2& \,\textcolor{gray}{±0.1} & 75.7& \,\textcolor{gray}{±0.1} & -& & 74.1& \,\textcolor{gray}{±0.1} & 76.4& \,\textcolor{gray}{±0.1} & 74.1& \,\textcolor{gray}{±0.1} \\
\midrule
GradCAM+ & 70.5& \,\textcolor{gray}{±0.1} & 77.3& \,\textcolor{gray}{±0.1} & 79.2& \,\textcolor{gray}{±0.1} & 64.7& \,\textcolor{gray}{±0.1} & 45.8& \,\textcolor{gray}{±0.1} & 63.8& \,\textcolor{gray}{±0.1} & 69.3& \,\textcolor{gray}{±0.1} & 67.2& \,\textcolor{gray}{±0.1} \\
\textbf{Libra GradCAM+} & 72.6& \,\textcolor{gray}{±0.1} & 80.1& \,\textcolor{gray}{±0.1} & 78.4& \,\textcolor{gray}{±0.1} & 72.9& \,\textcolor{gray}{±0.1} & 62.8& \,\textcolor{gray}{±0.1} & 65.6& \,\textcolor{gray}{±0.1} & 74.1& \,\textcolor{gray}{±0.1} & 72.3& \,\textcolor{gray}{±0.1} \\
\midrule
HiResCAM & 53.6& \,\textcolor{gray}{±0.1} & 79.3& \,\textcolor{gray}{±0.1} & 79.4& \,\textcolor{gray}{±0.1} & 70.0& \,\textcolor{gray}{±0.1} & 48.1& \,\textcolor{gray}{±0.1} & 72.4& \,\textcolor{gray}{±0.1} & 68.1& \,\textcolor{gray}{±0.1} & 67.3& \,\textcolor{gray}{±0.1} \\
\textbf{Libra HiResCAM} & 67.4& \,\textcolor{gray}{±0.1} & 79.4& \,\textcolor{gray}{±0.1} & 80.0& \,\textcolor{gray}{±0.1} & 80.7& \,\textcolor{gray}{±0.1} & 63.7& \,\textcolor{gray}{±0.1} & 74.7& \,\textcolor{gray}{±0.1} & 75.2& \,\textcolor{gray}{±0.1} & 74.4& \,\textcolor{gray}{±0.1} \\
\midrule
XGradCAM+ & 69.5& \,\textcolor{gray}{±0.1} & 78.3& \,\textcolor{gray}{±0.1} & 78.9& \,\textcolor{gray}{±0.1} & 65.0& \,\textcolor{gray}{±0.1} & 57.3& \,\textcolor{gray}{±0.1} & 69.7& \,\textcolor{gray}{±0.1} & 71.4& \,\textcolor{gray}{±0.1} & 70.0& \,\textcolor{gray}{±0.1} \\
\textbf{Libra XGradCAM+} & 73.5& \,\textcolor{gray}{±0.1} & 80.1& \,\textcolor{gray}{±0.1} & 79.5& \,\textcolor{gray}{±0.1} & 77.5& \,\textcolor{gray}{±0.1} & 70.5& \,\textcolor{gray}{±0.1} & 75.5& \,\textcolor{gray}{±0.1} & 79.6& \,\textcolor{gray}{±0.1} & 76.6& \,\textcolor{gray}{±0.1} \\
\midrule
FullGrad+ & 71.5& \,\textcolor{gray}{±0.1} & 82.1& \,\textcolor{gray}{±0.1} & 79.9& \,\textcolor{gray}{±0.1} & 81.4& \,\textcolor{gray}{±0.1} & 70.4& \,\textcolor{gray}{±0.1} & 71.4& \,\textcolor{gray}{±0.1} & 74.6& \,\textcolor{gray}{±0.1} & 75.9& \,\textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & \textbf{76.8}& \,\textcolor{gray}{±0.1} & \underline{82.6}& \,\textcolor{gray}{±0.1} & \underline{80.8}& \,\textcolor{gray}{±0.1} & \underline{81.5}& \,\textcolor{gray}{±0.1} & \underline{79.8}& \,\textcolor{gray}{±0.1} & \textbf{79.1}& \,\textcolor{gray}{±0.1} & \textbf{81.8}& \,\textcolor{gray}{±0.1} & \textbf{80.4}& \,\textcolor{gray}{±0.1} \\
\bottomrule
\end{tabular}
\caption{Least-Influential-First Deletion (LIF) Accuracy evaluated using ground-truth labels across multiple models.}
\label{across_models_sel1_LIF_gt_accuracy_m_2}
\end{table}


==> files/tables_v1/across_models/sel1/MIF_1p_AOPC/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}l}
\toprule
Method & \multicolumn{2}{c}{ViT-L} & \multicolumn{2}{c}{EVA2-S} & \multicolumn{2}{c}{BEiT2-L} & \multicolumn{2}{c}{FlexiViT-L} & \multicolumn{2}{c}{SigLIP-L} & \multicolumn{2}{c}{CLIP-H} & \multicolumn{2}{c}{DeiT3-H} & \multicolumn{2}{c}{\textit{Avg.}} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-15}
\cmidrule(l){16-17}
Random & 15.8& \,\textcolor{gray}{±0.2} & 8.2& \,\textcolor{gray}{±0.2} & 6.8& \,\textcolor{gray}{±0.1} & 6.4& \,\textcolor{gray}{±0.2} & 19.1& \,\textcolor{gray}{±0.2} & 12.7& \,\textcolor{gray}{±0.2} & 19.2& \,\textcolor{gray}{±0.2} & 12.6& \,\textcolor{gray}{±0.2} \\
RawAtt & 25.3& \,\textcolor{gray}{±0.2} & 33.9& \,\textcolor{gray}{±0.3} & 17.5& \,\textcolor{gray}{±0.2} & 26.5& \,\textcolor{gray}{±0.3} & -& & 23.3& \,\textcolor{gray}{±0.2} & 37.2& \,\textcolor{gray}{±0.2} & 27.3& \,\textcolor{gray}{±0.2} \\
Attention Rollout & 18.3& \,\textcolor{gray}{±0.3} & 24.9& \,\textcolor{gray}{±0.3} & 8.6& \,\textcolor{gray}{±0.1} & 9.7& \,\textcolor{gray}{±0.2} & -& & 22.5& \,\textcolor{gray}{±0.3} & 21.9& \,\textcolor{gray}{±0.2} & 17.7& \,\textcolor{gray}{±0.2} \\
AliLRP & 19.2& \,\textcolor{gray}{±0.2} & 31.3& \,\textcolor{gray}{±0.3} & 13.9& \,\textcolor{gray}{±0.2} & 10.5& \,\textcolor{gray}{±0.2} & 40.0& \,\textcolor{gray}{±0.3} & 17.3& \,\textcolor{gray}{±0.2} & 41.7& \,\textcolor{gray}{±0.2} & 24.8& \,\textcolor{gray}{±0.2} \\
AttnLRP & 27.6& \,\textcolor{gray}{±0.3} & 44.2& \,\textcolor{gray}{±0.2} & 25.0& \,\textcolor{gray}{±0.2} & 8.3& \,\textcolor{gray}{±0.2} & 46.2& \,\textcolor{gray}{±0.3} & 26.4& \,\textcolor{gray}{±0.2} & 31.7& \,\textcolor{gray}{±0.2} & 29.9& \,\textcolor{gray}{±0.2} \\
DecompX & 25.3& \,\textcolor{gray}{±0.3} & 30.7& \,\textcolor{gray}{±0.3} & 19.4& \,\textcolor{gray}{±0.2} & 20.7& \,\textcolor{gray}{±0.2} & 35.7& \,\textcolor{gray}{±0.2} & 23.5& \,\textcolor{gray}{±0.2} & 35.9& \,\textcolor{gray}{±0.2} & 27.3& \,\textcolor{gray}{±0.2} \\
Integrated Gradients & 21.9& \,\textcolor{gray}{±0.2} & 19.3& \,\textcolor{gray}{±0.2} & 11.9& \,\textcolor{gray}{±0.1} & 9.4& \,\textcolor{gray}{±0.2} & 28.8& \,\textcolor{gray}{±0.2} & 15.0& \,\textcolor{gray}{±0.2} & 22.8& \,\textcolor{gray}{±0.2} & 18.4& \,\textcolor{gray}{±0.2} \\
\midrule
\IxG{}  & 19.6& \,\textcolor{gray}{±0.2} & 17.0& \,\textcolor{gray}{±0.2} & 10.3& \,\textcolor{gray}{±0.1} & 6.5& \,\textcolor{gray}{±0.2} & 26.0& \,\textcolor{gray}{±0.2} & 15.2& \,\textcolor{gray}{±0.2} & 25.1& \,\textcolor{gray}{±0.2} & 17.1& \,\textcolor{gray}{±0.2} \\
\textbf{Libra \IxG{} } & 26.1& \,\textcolor{gray}{±0.3} & 44.4& \,\textcolor{gray}{±0.3} & 20.2& \,\textcolor{gray}{±0.2} & 21.3& \,\textcolor{gray}{±0.2} & 35.6& \,\textcolor{gray}{±0.2} & 24.0& \,\textcolor{gray}{±0.2} & 36.3& \,\textcolor{gray}{±0.2} & 29.7& \,\textcolor{gray}{±0.2} \\
\midrule
AttCAT & 29.0& \,\textcolor{gray}{±0.3} & 35.3& \,\textcolor{gray}{±0.3} & 21.0& \,\textcolor{gray}{±0.2} & 22.6& \,\textcolor{gray}{±0.3} & 30.9& \,\textcolor{gray}{±0.2} & 21.3& \,\textcolor{gray}{±0.1} & 32.3& \,\textcolor{gray}{±0.3} & 27.5& \,\textcolor{gray}{±0.2} \\
\textbf{Libra AttCAT} & \underline{44.5}& \,\textcolor{gray}{±0.3} & \underline{48.7}& \,\textcolor{gray}{±0.2} & \underline{34.6}& \,\textcolor{gray}{±0.2} & \underline{39.6}& \,\textcolor{gray}{±0.3} & \textbf{59.7}& \,\textcolor{gray}{±0.2} & \underline{34.7}& \,\textcolor{gray}{±0.2} & \underline{52.8}& \,\textcolor{gray}{±0.2} & \underline{44.9}& \,\textcolor{gray}{±0.2} \\
\midrule
GenAtt & 36.5& \,\textcolor{gray}{±0.3} & 24.3& \,\textcolor{gray}{±0.2} & 19.2& \,\textcolor{gray}{±0.2} & 35.1& \,\textcolor{gray}{±0.3} & -& & 29.6& \,\textcolor{gray}{±0.2} & 48.1& \,\textcolor{gray}{±0.2} & 32.1& \,\textcolor{gray}{±0.2} \\
\textbf{Libra GenAtt} & 39.6& \,\textcolor{gray}{±0.3} & 25.6& \,\textcolor{gray}{±0.2} & 20.7& \,\textcolor{gray}{±0.3} & 36.7& \,\textcolor{gray}{±0.3} & -& & 34.5& \,\textcolor{gray}{±0.2} & 49.7& \,\textcolor{gray}{±0.2} & 34.5& \,\textcolor{gray}{±0.3} \\
\midrule
TokenTM & 34.9& \,\textcolor{gray}{±0.3} & 28.3& \,\textcolor{gray}{±0.3} & 26.8& \,\textcolor{gray}{±0.3} & 32.7& \,\textcolor{gray}{±0.3} & -& & 30.1& \,\textcolor{gray}{±0.2} & 47.2& \,\textcolor{gray}{±0.2} & 33.3& \,\textcolor{gray}{±0.3} \\
\textbf{Libra TokenTM} & 37.4& \,\textcolor{gray}{±0.3} & 28.8& \,\textcolor{gray}{±0.3} & 25.5& \,\textcolor{gray}{±0.3} & 34.4& \,\textcolor{gray}{±0.3} & -& & 34.1& \,\textcolor{gray}{±0.2} & 48.8& \,\textcolor{gray}{±0.2} & 34.8& \,\textcolor{gray}{±0.3} \\
\midrule
GradCAM+ & 33.0& \,\textcolor{gray}{±0.2} & 29.0& \,\textcolor{gray}{±0.3} & 20.1& \,\textcolor{gray}{±0.2} & 13.1& \,\textcolor{gray}{±0.2} & 28.1& \,\textcolor{gray}{±0.2} & 16.2& \,\textcolor{gray}{±0.2} & 31.8& \,\textcolor{gray}{±0.2} & 24.5& \,\textcolor{gray}{±0.2} \\
\textbf{Libra GradCAM+} & 40.1& \,\textcolor{gray}{±0.3} & 46.1& \,\textcolor{gray}{±0.2} & 24.3& \,\textcolor{gray}{±0.2} & 18.4& \,\textcolor{gray}{±0.3} & 31.9& \,\textcolor{gray}{±0.3} & 18.6& \,\textcolor{gray}{±0.2} & 35.5& \,\textcolor{gray}{±0.2} & 30.7& \,\textcolor{gray}{±0.3} \\
\midrule
HiResCAM & 12.2& \,\textcolor{gray}{±0.2} & 40.1& \,\textcolor{gray}{±0.2} & 22.3& \,\textcolor{gray}{±0.2} & 9.0& \,\textcolor{gray}{±0.2} & 17.5& \,\textcolor{gray}{±0.2} & 19.7& \,\textcolor{gray}{±0.2} & 17.4& \,\textcolor{gray}{±0.2} & 19.7& \,\textcolor{gray}{±0.2} \\
\textbf{Libra HiResCAM} & 33.2& \,\textcolor{gray}{±0.3} & 42.9& \,\textcolor{gray}{±0.2} & 23.6& \,\textcolor{gray}{±0.2} & 38.1& \,\textcolor{gray}{±0.3} & 30.4& \,\textcolor{gray}{±0.2} & 27.9& \,\textcolor{gray}{±0.2} & 39.7& \,\textcolor{gray}{±0.2} & 33.7& \,\textcolor{gray}{±0.2} \\
\midrule
XGradCAM+ & 30.5& \,\textcolor{gray}{±0.3} & 31.9& \,\textcolor{gray}{±0.2} & 17.9& \,\textcolor{gray}{±0.2} & 9.9& \,\textcolor{gray}{±0.2} & 37.8& \,\textcolor{gray}{±0.2} & 21.3& \,\textcolor{gray}{±0.2} & 31.8& \,\textcolor{gray}{±0.2} & 25.9& \,\textcolor{gray}{±0.2} \\
\textbf{Libra XGradCAM+} & 42.2& \,\textcolor{gray}{±0.3} & 48.1& \,\textcolor{gray}{±0.2} & 31.4& \,\textcolor{gray}{±0.3} & 27.2& \,\textcolor{gray}{±0.3} & 46.3& \,\textcolor{gray}{±0.3} & 34.1& \,\textcolor{gray}{±0.2} & 49.0& \,\textcolor{gray}{±0.2} & 39.8& \,\textcolor{gray}{±0.3} \\
\midrule
FullGrad+ & 28.9& \,\textcolor{gray}{±0.3} & 30.0& \,\textcolor{gray}{±0.2} & 16.6& \,\textcolor{gray}{±0.2} & 20.8& \,\textcolor{gray}{±0.3} & 29.0& \,\textcolor{gray}{±0.2} & 20.5& \,\textcolor{gray}{±0.2} & 30.0& \,\textcolor{gray}{±0.3} & 25.1& \,\textcolor{gray}{±0.2} \\
\textbf{Libra FullGrad+} & \textbf{45.3}& \,\textcolor{gray}{±0.3} & \textbf{50.5}& \,\textcolor{gray}{±0.2} & \textbf{35.5}& \,\textcolor{gray}{±0.3} & \textbf{39.8}& \,\textcolor{gray}{±0.3} & \underline{55.1}& \,\textcolor{gray}{±0.2} & \textbf{36.8}& \,\textcolor{gray}{±0.2} & \textbf{53.7}& \,\textcolor{gray}{±0.2} & \textbf{45.2}& \,\textcolor{gray}{±0.2} \\
\bottomrule
\end{tabular}
\caption{Most-Influential-First Deletion (MIF) AOPC evaluated using predicted labels across multiple models.}
\label{across_models_sel1_MIF_1p_AOPC_m_2}
\end{table}


==> files/tables_v1/across_models/sel1/MIF_gt_AOPC/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}l}
\toprule
Method & \multicolumn{2}{c}{ViT-L} & \multicolumn{2}{c}{EVA2-S} & \multicolumn{2}{c}{BEiT2-L} & \multicolumn{2}{c}{FlexiViT-L} & \multicolumn{2}{c}{SigLIP-L} & \multicolumn{2}{c}{CLIP-H} & \multicolumn{2}{c}{DeiT3-H} & \multicolumn{2}{c}{\textit{Avg.}} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-15}
\cmidrule(l){16-17}
Random & 14.1& \,\textcolor{gray}{±0.2} & 6.6& \,\textcolor{gray}{±0.2} & 5.6& \,\textcolor{gray}{±0.2} & 5.2& \,\textcolor{gray}{±0.2} & 17.3& \,\textcolor{gray}{±0.2} & 11.2& \,\textcolor{gray}{±0.2} & 16.6& \,\textcolor{gray}{±0.2} & 10.9& \,\textcolor{gray}{±0.2} \\
RawAtt & 22.9& \,\textcolor{gray}{±0.3} & 30.3& \,\textcolor{gray}{±0.3} & 15.3& \,\textcolor{gray}{±0.2} & 23.6& \,\textcolor{gray}{±0.3} & -& & 21.0& \,\textcolor{gray}{±0.2} & 33.3& \,\textcolor{gray}{±0.3} & 24.4& \,\textcolor{gray}{±0.3} \\
Attention Rollout & 16.5& \,\textcolor{gray}{±0.3} & 22.0& \,\textcolor{gray}{±0.4} & 7.2& \,\textcolor{gray}{±0.1} & 8.2& \,\textcolor{gray}{±0.2} & -& & 20.5& \,\textcolor{gray}{±0.3} & 19.0& \,\textcolor{gray}{±0.2} & 15.5& \,\textcolor{gray}{±0.3} \\
AliLRP & 17.2& \,\textcolor{gray}{±0.3} & 27.7& \,\textcolor{gray}{±0.4} & 12.4& \,\textcolor{gray}{±0.2} & 8.8& \,\textcolor{gray}{±0.2} & 36.6& \,\textcolor{gray}{±0.3} & 15.7& \,\textcolor{gray}{±0.2} & 37.3& \,\textcolor{gray}{±0.3} & 22.2& \,\textcolor{gray}{±0.3} \\
AttnLRP & 24.8& \,\textcolor{gray}{±0.3} & 39.6& \,\textcolor{gray}{±0.3} & 22.6& \,\textcolor{gray}{±0.3} & 6.6& \,\textcolor{gray}{±0.2} & 42.4& \,\textcolor{gray}{±0.3} & 24.0& \,\textcolor{gray}{±0.3} & 28.1& \,\textcolor{gray}{±0.3} & 26.9& \,\textcolor{gray}{±0.3} \\
DecompX & 22.6& \,\textcolor{gray}{±0.3} & 27.0& \,\textcolor{gray}{±0.4} & 17.3& \,\textcolor{gray}{±0.3} & 18.1& \,\textcolor{gray}{±0.2} & 32.6& \,\textcolor{gray}{±0.2} & 21.3& \,\textcolor{gray}{±0.2} & 32.2& \,\textcolor{gray}{±0.3} & 24.4& \,\textcolor{gray}{±0.3} \\
Integrated Gradients & 23.1& \,\textcolor{gray}{±0.3} & 21.0& \,\textcolor{gray}{±0.3} & 12.5& \,\textcolor{gray}{±0.2} & 8.3& \,\textcolor{gray}{±0.2} & 30.0& \,\textcolor{gray}{±0.2} & 13.5& \,\textcolor{gray}{±0.2} & 24.9& \,\textcolor{gray}{±0.3} & 19.1& \,\textcolor{gray}{±0.2} \\
\midrule
\IxG{}  & 17.5& \,\textcolor{gray}{±0.3} & 14.1& \,\textcolor{gray}{±0.2} & 9.0& \,\textcolor{gray}{±0.1} & 5.1& \,\textcolor{gray}{±0.2} & 23.2& \,\textcolor{gray}{±0.2} & 13.7& \,\textcolor{gray}{±0.2} & 21.9& \,\textcolor{gray}{±0.3} & 14.9& \,\textcolor{gray}{±0.2} \\
\textbf{Libra \IxG{} } & 23.4& \,\textcolor{gray}{±0.3} & 39.6& \,\textcolor{gray}{±0.3} & 18.0& \,\textcolor{gray}{±0.2} & 18.6& \,\textcolor{gray}{±0.2} & 32.4& \,\textcolor{gray}{±0.2} & 21.8& \,\textcolor{gray}{±0.2} & 32.4& \,\textcolor{gray}{±0.3} & 26.6& \,\textcolor{gray}{±0.3} \\
\midrule
AttCAT & 25.7& \,\textcolor{gray}{±0.3} & 30.9& \,\textcolor{gray}{±0.2} & 18.9& \,\textcolor{gray}{±0.2} & 18.9& \,\textcolor{gray}{±0.3} & 27.4& \,\textcolor{gray}{±0.3} & 18.8& \,\textcolor{gray}{±0.2} & 28.6& \,\textcolor{gray}{±0.3} & 24.2& \,\textcolor{gray}{±0.3} \\
\textbf{Libra AttCAT} & \underline{40.5}& \,\textcolor{gray}{±0.3} & \underline{43.8}& \,\textcolor{gray}{±0.3} & \underline{31.6}& \,\textcolor{gray}{±0.3} & \underline{35.5}& \,\textcolor{gray}{±0.3} & \textbf{55.0}& \,\textcolor{gray}{±0.3} & \underline{31.7}& \,\textcolor{gray}{±0.3} & \underline{47.6}& \,\textcolor{gray}{±0.3} & \underline{40.8}& \,\textcolor{gray}{±0.3} \\
\midrule
GenAtt & 33.2& \,\textcolor{gray}{±0.3} & 21.2& \,\textcolor{gray}{±0.2} & 17.0& \,\textcolor{gray}{±0.3} & 31.4& \,\textcolor{gray}{±0.3} & -& & 26.8& \,\textcolor{gray}{±0.2} & 43.3& \,\textcolor{gray}{±0.3} & 28.8& \,\textcolor{gray}{±0.3} \\
\textbf{Libra GenAtt} & 36.2& \,\textcolor{gray}{±0.3} & 22.5& \,\textcolor{gray}{±0.3} & 18.4& \,\textcolor{gray}{±0.3} & 32.9& \,\textcolor{gray}{±0.3} & -& & 31.5& \,\textcolor{gray}{±0.3} & 45.0& \,\textcolor{gray}{±0.3} & 31.1& \,\textcolor{gray}{±0.3} \\
\midrule
TokenTM & 31.8& \,\textcolor{gray}{±0.3} & 25.1& \,\textcolor{gray}{±0.3} & 24.3& \,\textcolor{gray}{±0.3} & 29.3& \,\textcolor{gray}{±0.3} & -& & 27.4& \,\textcolor{gray}{±0.3} & 42.6& \,\textcolor{gray}{±0.3} & 30.1& \,\textcolor{gray}{±0.3} \\
\textbf{Libra TokenTM} & 34.2& \,\textcolor{gray}{±0.3} & 25.6& \,\textcolor{gray}{±0.3} & 23.1& \,\textcolor{gray}{±0.3} & 30.9& \,\textcolor{gray}{±0.3} & -& & 31.2& \,\textcolor{gray}{±0.3} & 44.1& \,\textcolor{gray}{±0.3} & 31.5& \,\textcolor{gray}{±0.3} \\
\midrule
GradCAM+ & 30.0& \,\textcolor{gray}{±0.3} & 25.1& \,\textcolor{gray}{±0.3} & 18.2& \,\textcolor{gray}{±0.2} & 10.9& \,\textcolor{gray}{±0.2} & 25.4& \,\textcolor{gray}{±0.3} & 14.5& \,\textcolor{gray}{±0.2} & 28.3& \,\textcolor{gray}{±0.3} & 21.8& \,\textcolor{gray}{±0.2} \\
\textbf{Libra GradCAM+} & 36.7& \,\textcolor{gray}{±0.3} & 41.4& \,\textcolor{gray}{±0.3} & 22.0& \,\textcolor{gray}{±0.2} & 15.7& \,\textcolor{gray}{±0.2} & 28.8& \,\textcolor{gray}{±0.3} & 16.8& \,\textcolor{gray}{±0.2} & 31.4& \,\textcolor{gray}{±0.3} & 27.5& \,\textcolor{gray}{±0.3} \\
\midrule
HiResCAM & 10.6& \,\textcolor{gray}{±0.2} & 36.1& \,\textcolor{gray}{±0.2} & 20.1& \,\textcolor{gray}{±0.2} & 7.2& \,\textcolor{gray}{±0.2} & 15.7& \,\textcolor{gray}{±0.2} & 17.6& \,\textcolor{gray}{±0.2} & 15.0& \,\textcolor{gray}{±0.2} & 17.5& \,\textcolor{gray}{±0.2} \\
\textbf{Libra HiResCAM} & 30.2& \,\textcolor{gray}{±0.3} & 38.6& \,\textcolor{gray}{±0.3} & 21.2& \,\textcolor{gray}{±0.2} & 34.2& \,\textcolor{gray}{±0.3} & 27.5& \,\textcolor{gray}{±0.3} & 25.4& \,\textcolor{gray}{±0.2} & 35.4& \,\textcolor{gray}{±0.3} & 30.4& \,\textcolor{gray}{±0.3} \\
\midrule
XGradCAM+ & 27.7& \,\textcolor{gray}{±0.3} & 27.9& \,\textcolor{gray}{±0.2} & 16.0& \,\textcolor{gray}{±0.2} & 7.8& \,\textcolor{gray}{±0.2} & 34.5& \,\textcolor{gray}{±0.3} & 19.2& \,\textcolor{gray}{±0.2} & 27.9& \,\textcolor{gray}{±0.3} & 23.0& \,\textcolor{gray}{±0.2} \\
\textbf{Libra XGradCAM+} & 38.6& \,\textcolor{gray}{±0.3} & 43.3& \,\textcolor{gray}{±0.3} & 28.6& \,\textcolor{gray}{±0.3} & 24.1& \,\textcolor{gray}{±0.3} & 42.5& \,\textcolor{gray}{±0.3} & 31.1& \,\textcolor{gray}{±0.2} & 44.2& \,\textcolor{gray}{±0.3} & 36.0& \,\textcolor{gray}{±0.3} \\
\midrule
FullGrad+ & 25.8& \,\textcolor{gray}{±0.3} & 25.7& \,\textcolor{gray}{±0.2} & 14.9& \,\textcolor{gray}{±0.2} & 17.5& \,\textcolor{gray}{±0.3} & 25.8& \,\textcolor{gray}{±0.3} & 18.1& \,\textcolor{gray}{±0.2} & 26.2& \,\textcolor{gray}{±0.3} & 22.0& \,\textcolor{gray}{±0.3} \\
\textbf{Libra FullGrad+} & \textbf{41.2}& \,\textcolor{gray}{±0.3} & \textbf{45.5}& \,\textcolor{gray}{±0.3} & \textbf{32.4}& \,\textcolor{gray}{±0.3} & \textbf{35.8}& \,\textcolor{gray}{±0.3} & \underline{50.7}& \,\textcolor{gray}{±0.3} & \textbf{33.6}& \,\textcolor{gray}{±0.3} & \textbf{48.5}& \,\textcolor{gray}{±0.3} & \textbf{41.1}& \,\textcolor{gray}{±0.3} \\
\bottomrule
\end{tabular}
\caption{Most-Influential-First Deletion (MIF) AOPC evaluated using ground-truth labels across multiple models.}
\label{across_models_sel1_MIF_gt_AOPC_m_2}
\end{table}


==> files/tables_v1/across_models/sel1/MIF_gt_accuracy/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}l}
\toprule
Method & \multicolumn{2}{c}{ViT-L} & \multicolumn{2}{c}{EVA2-S} & \multicolumn{2}{c}{BEiT2-L} & \multicolumn{2}{c}{FlexiViT-L} & \multicolumn{2}{c}{SigLIP-L} & \multicolumn{2}{c}{CLIP-H} & \multicolumn{2}{c}{DeiT3-H} & \multicolumn{2}{c}{\textit{Avg.}} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-15}
\cmidrule(l){16-17}
Random & 36.9& \,\textcolor{gray}{±0.1} & 29.9& \,\textcolor{gray}{±0.1} & 25.1& \,\textcolor{gray}{±0.1} & 28.8& \,\textcolor{gray}{±0.1} & 39.0& \,\textcolor{gray}{±0.1} & 34.3& \,\textcolor{gray}{±0.1} & 35.6& \,\textcolor{gray}{±0.1} & 32.8& \,\textcolor{gray}{±0.1} \\
RawAtt & 45.4& \,\textcolor{gray}{±0.1} & 55.4& \,\textcolor{gray}{±0.1} & 34.2& \,\textcolor{gray}{±0.1} & 47.3& \,\textcolor{gray}{±0.1} & -& & 46.9& \,\textcolor{gray}{±0.1} & 56.1& \,\textcolor{gray}{±0.1} & 47.6& \,\textcolor{gray}{±0.1} \\
Attention Rollout & 39.0& \,\textcolor{gray}{±0.1} & 47.0& \,\textcolor{gray}{±0.1} & 26.0& \,\textcolor{gray}{±0.1} & 31.7& \,\textcolor{gray}{±0.1} & -& & 46.4& \,\textcolor{gray}{±0.1} & 37.1& \,\textcolor{gray}{±0.1} & 37.9& \,\textcolor{gray}{±0.1} \\
AliLRP & 39.8& \,\textcolor{gray}{±0.1} & 52.8& \,\textcolor{gray}{±0.1} & 31.9& \,\textcolor{gray}{±0.1} & 32.5& \,\textcolor{gray}{±0.1} & 58.8& \,\textcolor{gray}{±0.1} & 40.0& \,\textcolor{gray}{±0.1} & 59.6& \,\textcolor{gray}{±0.1} & 45.1& \,\textcolor{gray}{±0.1} \\
AttnLRP & 47.1& \,\textcolor{gray}{±0.1} & 66.6& \,\textcolor{gray}{±0.1} & 42.1& \,\textcolor{gray}{±0.1} & 30.3& \,\textcolor{gray}{±0.1} & 64.7& \,\textcolor{gray}{±0.1} & 50.8& \,\textcolor{gray}{±0.1} & 45.4& \,\textcolor{gray}{±0.1} & 49.6& \,\textcolor{gray}{±0.1} \\
DecompX & 44.4& \,\textcolor{gray}{±0.1} & 51.6& \,\textcolor{gray}{±0.1} & 36.5& \,\textcolor{gray}{±0.1} & 42.0& \,\textcolor{gray}{±0.1} & 54.5& \,\textcolor{gray}{±0.1} & 46.7& \,\textcolor{gray}{±0.1} & 51.6& \,\textcolor{gray}{±0.1} & 46.8& \,\textcolor{gray}{±0.1} \\
Integrated Gradients & 46.3& \,\textcolor{gray}{±0.1} & 46.2& \,\textcolor{gray}{±0.1} & 31.7& \,\textcolor{gray}{±0.1} & 31.4& \,\textcolor{gray}{±0.1} & 52.7& \,\textcolor{gray}{±0.1} & 37.1& \,\textcolor{gray}{±0.1} & 43.7& \,\textcolor{gray}{±0.1} & 41.3& \,\textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 40.1& \,\textcolor{gray}{±0.1} & 37.9& \,\textcolor{gray}{±0.1} & 28.2& \,\textcolor{gray}{±0.1} & 28.5& \,\textcolor{gray}{±0.1} & 44.4& \,\textcolor{gray}{±0.1} & 37.5& \,\textcolor{gray}{±0.1} & 40.4& \,\textcolor{gray}{±0.1} & 36.7& \,\textcolor{gray}{±0.1} \\
\textbf{Libra \IxG{} } & 45.9& \,\textcolor{gray}{±0.1} & 67.0& \,\textcolor{gray}{±0.1} & 37.7& \,\textcolor{gray}{±0.1} & 42.6& \,\textcolor{gray}{±0.1} & 54.7& \,\textcolor{gray}{±0.1} & 47.5& \,\textcolor{gray}{±0.1} & 52.1& \,\textcolor{gray}{±0.1} & 49.7& \,\textcolor{gray}{±0.1} \\
\midrule
AttCAT & 48.7& \,\textcolor{gray}{±0.1} & 56.9& \,\textcolor{gray}{±0.1} & 38.4& \,\textcolor{gray}{±0.1} & 45.3& \,\textcolor{gray}{±0.1} & 48.3& \,\textcolor{gray}{±0.1} & 42.5& \,\textcolor{gray}{±0.1} & 48.2& \,\textcolor{gray}{±0.1} & 46.9& \,\textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \underline{64.7}& \,\textcolor{gray}{±0.1} & \underline{72.1}& \,\textcolor{gray}{±0.1} & \underline{52.5}& \,\textcolor{gray}{±0.1} & \underline{61.8}& \,\textcolor{gray}{±0.1} & \textbf{79.0}& \,\textcolor{gray}{±0.1} & \underline{61.5}& \,\textcolor{gray}{±0.1} & \underline{72.6}& \,\textcolor{gray}{±0.1} & \underline{66.3}& \,\textcolor{gray}{±0.1} \\
\midrule
GenAtt & 56.4& \,\textcolor{gray}{±0.1} & 46.3& \,\textcolor{gray}{±0.1} & 35.6& \,\textcolor{gray}{±0.1} & 57.2& \,\textcolor{gray}{±0.1} & -& & 54.4& \,\textcolor{gray}{±0.1} & 67.2& \,\textcolor{gray}{±0.1} & 52.9& \,\textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 59.7& \,\textcolor{gray}{±0.1} & 47.7& \,\textcolor{gray}{±0.1} & 37.6& \,\textcolor{gray}{±0.1} & 58.3& \,\textcolor{gray}{±0.1} & -& & 61.0& \,\textcolor{gray}{±0.1} & 69.1& \,\textcolor{gray}{±0.1} & 55.6& \,\textcolor{gray}{±0.1} \\
\midrule
TokenTM & 54.9& \,\textcolor{gray}{±0.1} & 50.4& \,\textcolor{gray}{±0.1} & 43.9& \,\textcolor{gray}{±0.1} & 54.3& \,\textcolor{gray}{±0.1} & -& & 55.4& \,\textcolor{gray}{±0.1} & 66.2& \,\textcolor{gray}{±0.1} & 54.2& \,\textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 57.3& \,\textcolor{gray}{±0.1} & 51.6& \,\textcolor{gray}{±0.1} & 42.6& \,\textcolor{gray}{±0.1} & 55.7& \,\textcolor{gray}{±0.1} & -& & 60.6& \,\textcolor{gray}{±0.1} & 68.1& \,\textcolor{gray}{±0.1} & 56.0& \,\textcolor{gray}{±0.1} \\
\midrule
GradCAM+ & 53.4& \,\textcolor{gray}{±0.1} & 50.6& \,\textcolor{gray}{±0.1} & 38.4& \,\textcolor{gray}{±0.1} & 35.8& \,\textcolor{gray}{±0.1} & 47.6& \,\textcolor{gray}{±0.1} & 38.6& \,\textcolor{gray}{±0.1} & 49.5& \,\textcolor{gray}{±0.1} & 44.8& \,\textcolor{gray}{±0.1} \\
\textbf{Libra GradCAM+} & 60.9& \,\textcolor{gray}{±0.1} & 69.9& \,\textcolor{gray}{±0.1} & 42.3& \,\textcolor{gray}{±0.1} & 40.2& \,\textcolor{gray}{±0.1} & 51.0& \,\textcolor{gray}{±0.1} & 41.8& \,\textcolor{gray}{±0.1} & 52.6& \,\textcolor{gray}{±0.1} & 51.3& \,\textcolor{gray}{±0.1} \\
\midrule
HiResCAM & 32.7& \,\textcolor{gray}{±0.1} & 63.1& \,\textcolor{gray}{±0.1} & 40.3& \,\textcolor{gray}{±0.1} & 31.2& \,\textcolor{gray}{±0.1} & 37.1& \,\textcolor{gray}{±0.1} & 42.3& \,\textcolor{gray}{±0.1} & 32.5& \,\textcolor{gray}{±0.1} & 39.9& \,\textcolor{gray}{±0.1} \\
\textbf{Libra HiResCAM} & 54.0& \,\textcolor{gray}{±0.1} & 65.9& \,\textcolor{gray}{±0.1} & 41.5& \,\textcolor{gray}{±0.1} & 60.1& \,\textcolor{gray}{±0.1} & 50.0& \,\textcolor{gray}{±0.1} & 52.8& \,\textcolor{gray}{±0.1} & 57.4& \,\textcolor{gray}{±0.1} & 54.5& \,\textcolor{gray}{±0.1} \\
\midrule
XGradCAM+ & 50.9& \,\textcolor{gray}{±0.1} & 53.7& \,\textcolor{gray}{±0.1} & 35.6& \,\textcolor{gray}{±0.1} & 33.4& \,\textcolor{gray}{±0.1} & 54.8& \,\textcolor{gray}{±0.1} & 44.2& \,\textcolor{gray}{±0.1} & 49.1& \,\textcolor{gray}{±0.1} & 46.0& \,\textcolor{gray}{±0.1} \\
\textbf{Libra XGradCAM+} & 63.0& \,\textcolor{gray}{±0.1} & 71.9& \,\textcolor{gray}{±0.1} & 49.5& \,\textcolor{gray}{±0.1} & 49.7& \,\textcolor{gray}{±0.1} & 66.3& \,\textcolor{gray}{±0.1} & 60.8& \,\textcolor{gray}{±0.1} & 68.8& \,\textcolor{gray}{±0.1} & 61.4& \,\textcolor{gray}{±0.1} \\
\midrule
FullGrad+ & 49.1& \,\textcolor{gray}{±0.1} & 50.9& \,\textcolor{gray}{±0.1} & 34.4& \,\textcolor{gray}{±0.1} & 43.0& \,\textcolor{gray}{±0.1} & 46.6& \,\textcolor{gray}{±0.1} & 41.4& \,\textcolor{gray}{±0.1} & 45.8& \,\textcolor{gray}{±0.1} & 44.4& \,\textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & \textbf{65.5}& \,\textcolor{gray}{±0.1} & \textbf{74.1}& \,\textcolor{gray}{±0.1} & \textbf{53.4}& \,\textcolor{gray}{±0.1} & \textbf{62.4}& \,\textcolor{gray}{±0.1} & \underline{75.3}& \,\textcolor{gray}{±0.1} & \textbf{63.8}& \,\textcolor{gray}{±0.1} & \textbf{73.5}& \,\textcolor{gray}{±0.1} & \textbf{66.9}& \,\textcolor{gray}{±0.1} \\
\bottomrule
\end{tabular}
\caption{Most-Influential-First Deletion (MIF) Accuracy evaluated using ground-truth labels across multiple models.}
\label{across_models_sel1_MIF_gt_accuracy_m_2}
\end{table}


==> files/tables_v1/across_models/sel1/SRG_1p_AOPC/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}l}
\toprule
Method & \multicolumn{2}{c}{ViT-L} & \multicolumn{2}{c}{EVA2-S} & \multicolumn{2}{c}{BEiT2-L} & \multicolumn{2}{c}{FlexiViT-L} & \multicolumn{2}{c}{SigLIP-L} & \multicolumn{2}{c}{CLIP-H} & \multicolumn{2}{c}{DeiT3-H} & \multicolumn{2}{c}{\textit{Avg.}} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-15}
\cmidrule(l){16-17}
Random & 49.8& \,\textcolor{gray}{±0.2} & 50.2& \,\textcolor{gray}{±0.2} & 50.0& \,\textcolor{gray}{±0.1} & 50.0& \,\textcolor{gray}{±0.2} & 50.0& \,\textcolor{gray}{±0.2} & 50.1& \,\textcolor{gray}{±0.2} & 50.1& \,\textcolor{gray}{±0.2} & 50.0& \,\textcolor{gray}{±0.2} \\
RawAtt & 53.4& \,\textcolor{gray}{±0.2} & 64.8& \,\textcolor{gray}{±0.2} & 56.2& \,\textcolor{gray}{±0.2} & 60.9& \,\textcolor{gray}{±0.2} & -& & 56.7& \,\textcolor{gray}{±0.2} & 60.7& \,\textcolor{gray}{±0.2} & 58.8& \,\textcolor{gray}{±0.2} \\
Attention Rollout & 50.1& \,\textcolor{gray}{±0.2} & 58.4& \,\textcolor{gray}{±0.3} & 48.0& \,\textcolor{gray}{±0.2} & 48.0& \,\textcolor{gray}{±0.2} & -& & 55.9& \,\textcolor{gray}{±0.2} & 48.3& \,\textcolor{gray}{±0.2} & 51.5& \,\textcolor{gray}{±0.2} \\
AliLRP & 52.5& \,\textcolor{gray}{±0.2} & 66.1& \,\textcolor{gray}{±0.2} & 54.7& \,\textcolor{gray}{±0.1} & 54.2& \,\textcolor{gray}{±0.1} & 64.9& \,\textcolor{gray}{±0.2} & 53.6& \,\textcolor{gray}{±0.2} & 68.8& \,\textcolor{gray}{±0.2} & 59.3& \,\textcolor{gray}{±0.2} \\
AttnLRP & 59.5& \,\textcolor{gray}{±0.2} & 73.1& \,\textcolor{gray}{±0.2} & 60.9& \,\textcolor{gray}{±0.2} & 49.6& \,\textcolor{gray}{±0.2} & 70.6& \,\textcolor{gray}{±0.2} & 61.3& \,\textcolor{gray}{±0.2} & 62.0& \,\textcolor{gray}{±0.2} & 62.4& \,\textcolor{gray}{±0.2} \\
DecompX & 57.3& \,\textcolor{gray}{±0.2} & 65.1& \,\textcolor{gray}{±0.2} & 57.8& \,\textcolor{gray}{±0.2} & 60.1& \,\textcolor{gray}{±0.1} & 63.1& \,\textcolor{gray}{±0.2} & 58.9& \,\textcolor{gray}{±0.2} & 64.7& \,\textcolor{gray}{±0.2} & 61.0& \,\textcolor{gray}{±0.2} \\
Integrated Gradients & 55.1& \,\textcolor{gray}{±0.2} & 59.6& \,\textcolor{gray}{±0.2} & 54.2& \,\textcolor{gray}{±0.2} & 50.7& \,\textcolor{gray}{±0.2} & 60.0& \,\textcolor{gray}{±0.2} & 50.3& \,\textcolor{gray}{±0.1} & 53.8& \,\textcolor{gray}{±0.2} & 54.8& \,\textcolor{gray}{±0.2} \\
\midrule
\IxG{}  & 53.2& \,\textcolor{gray}{±0.2} & 57.9& \,\textcolor{gray}{±0.2} & 51.9& \,\textcolor{gray}{±0.1} & 48.9& \,\textcolor{gray}{±0.2} & 56.8& \,\textcolor{gray}{±0.2} & 50.1& \,\textcolor{gray}{±0.1} & 56.4& \,\textcolor{gray}{±0.2} & 53.6& \,\textcolor{gray}{±0.2} \\
\textbf{Libra \IxG{} } & 58.2& \,\textcolor{gray}{±0.2} & 73.4& \,\textcolor{gray}{±0.2} & 58.5& \,\textcolor{gray}{±0.2} & 60.8& \,\textcolor{gray}{±0.1} & 63.1& \,\textcolor{gray}{±0.2} & 59.4& \,\textcolor{gray}{±0.2} & 65.1& \,\textcolor{gray}{±0.2} & 62.7& \,\textcolor{gray}{±0.2} \\
\midrule
AttCAT & 60.8& \,\textcolor{gray}{±0.2} & 70.3& \,\textcolor{gray}{±0.2} & 60.5& \,\textcolor{gray}{±0.1} & 63.5& \,\textcolor{gray}{±0.3} & 61.7& \,\textcolor{gray}{±0.2} & 58.1& \,\textcolor{gray}{±0.2} & 61.5& \,\textcolor{gray}{±0.2} & 62.3& \,\textcolor{gray}{±0.2} \\
\textbf{Libra AttCAT} & \underline{70.8}& \,\textcolor{gray}{±0.2} & \underline{75.7}& \,\textcolor{gray}{±0.2} & \underline{66.3}& \,\textcolor{gray}{±0.2} & \underline{71.3}& \,\textcolor{gray}{±0.2} & \textbf{79.0}& \,\textcolor{gray}{±0.2} & \underline{65.5}& \,\textcolor{gray}{±0.2} & \underline{75.7}& \,\textcolor{gray}{±0.2} & \underline{72.0}& \,\textcolor{gray}{±0.2} \\
\midrule
GenAtt & 64.0& \,\textcolor{gray}{±0.2} & 59.1& \,\textcolor{gray}{±0.2} & 56.8& \,\textcolor{gray}{±0.2} & 67.4& \,\textcolor{gray}{±0.2} & -& & 62.0& \,\textcolor{gray}{±0.2} & 70.8& \,\textcolor{gray}{±0.2} & 63.3& \,\textcolor{gray}{±0.2} \\
\textbf{Libra GenAtt} & 65.8& \,\textcolor{gray}{±0.3} & 60.0& \,\textcolor{gray}{±0.2} & 57.5& \,\textcolor{gray}{±0.2} & 68.0& \,\textcolor{gray}{±0.2} & -& & 64.5& \,\textcolor{gray}{±0.2} & 71.9& \,\textcolor{gray}{±0.2} & 64.6& \,\textcolor{gray}{±0.2} \\
\midrule
TokenTM & 62.6& \,\textcolor{gray}{±0.2} & 61.7& \,\textcolor{gray}{±0.2} & 61.2& \,\textcolor{gray}{±0.2} & 65.6& \,\textcolor{gray}{±0.2} & -& & 61.8& \,\textcolor{gray}{±0.2} & 70.1& \,\textcolor{gray}{±0.2} & 63.8& \,\textcolor{gray}{±0.2} \\
\textbf{Libra TokenTM} & 64.1& \,\textcolor{gray}{±0.3} & 61.8& \,\textcolor{gray}{±0.2} & 60.0& \,\textcolor{gray}{±0.2} & 66.5& \,\textcolor{gray}{±0.2} & -& & 63.9& \,\textcolor{gray}{±0.2} & 71.0& \,\textcolor{gray}{±0.2} & 64.6& \,\textcolor{gray}{±0.2} \\
\midrule
GradCAM+ & 62.0& \,\textcolor{gray}{±0.2} & 63.8& \,\textcolor{gray}{±0.2} & 58.6& \,\textcolor{gray}{±0.2} & 49.4& \,\textcolor{gray}{±0.2} & 44.4& \,\textcolor{gray}{±0.3} & 50.9& \,\textcolor{gray}{±0.2} & 58.1& \,\textcolor{gray}{±0.2} & 55.3& \,\textcolor{gray}{±0.2} \\
\textbf{Libra GradCAM+} & 66.4& \,\textcolor{gray}{±0.2} & 73.2& \,\textcolor{gray}{±0.2} & 59.9& \,\textcolor{gray}{±0.2} & 56.1& \,\textcolor{gray}{±0.2} & 56.4& \,\textcolor{gray}{±0.3} & 52.5& \,\textcolor{gray}{±0.2} & 62.6& \,\textcolor{gray}{±0.2} & 61.0& \,\textcolor{gray}{±0.2} \\
\midrule
HiResCAM & 43.2& \,\textcolor{gray}{±0.2} & 70.6& \,\textcolor{gray}{±0.2} & 59.6& \,\textcolor{gray}{±0.2} & 50.1& \,\textcolor{gray}{±0.2} & 41.9& \,\textcolor{gray}{±0.2} & 56.2& \,\textcolor{gray}{±0.2} & 50.8& \,\textcolor{gray}{±0.2} & 53.2& \,\textcolor{gray}{±0.2} \\
\textbf{Libra HiResCAM} & 60.6& \,\textcolor{gray}{±0.2} & 71.7& \,\textcolor{gray}{±0.2} & 60.4& \,\textcolor{gray}{±0.2} & 69.8& \,\textcolor{gray}{±0.2} & 56.5& \,\textcolor{gray}{±0.2} & 61.0& \,\textcolor{gray}{±0.2} & 63.3& \,\textcolor{gray}{±0.2} & 63.3& \,\textcolor{gray}{±0.2} \\
\midrule
XGradCAM+ & 60.3& \,\textcolor{gray}{±0.2} & 65.8& \,\textcolor{gray}{±0.2} & 57.2& \,\textcolor{gray}{±0.1} & 47.3& \,\textcolor{gray}{±0.3} & 56.5& \,\textcolor{gray}{±0.2} & 56.0& \,\textcolor{gray}{±0.2} & 59.6& \,\textcolor{gray}{±0.2} & 57.5& \,\textcolor{gray}{±0.2} \\
\textbf{Libra XGradCAM+} & 68.0& \,\textcolor{gray}{±0.3} & 74.2& \,\textcolor{gray}{±0.2} & 64.0& \,\textcolor{gray}{±0.2} & 63.1& \,\textcolor{gray}{±0.2} & 67.3& \,\textcolor{gray}{±0.2} & 64.0& \,\textcolor{gray}{±0.2} & 72.2& \,\textcolor{gray}{±0.2} & 67.5& \,\textcolor{gray}{±0.2} \\
\midrule
FullGrad+ & 60.4& \,\textcolor{gray}{±0.2} & 67.2& \,\textcolor{gray}{±0.2} & 57.3& \,\textcolor{gray}{±0.2} & 62.0& \,\textcolor{gray}{±0.2} & 59.2& \,\textcolor{gray}{±0.2} & 57.0& \,\textcolor{gray}{±0.2} & 60.1& \,\textcolor{gray}{±0.3} & 60.4& \,\textcolor{gray}{±0.2} \\
\textbf{Libra FullGrad+} & \textbf{71.3}& \,\textcolor{gray}{±0.2} & \textbf{76.8}& \,\textcolor{gray}{±0.2} & \textbf{66.8}& \,\textcolor{gray}{±0.2} & \textbf{71.4}& \,\textcolor{gray}{±0.2} & \underline{76.7}& \,\textcolor{gray}{±0.2} & \textbf{66.8}& \,\textcolor{gray}{±0.2} & \textbf{76.3}& \,\textcolor{gray}{±0.2} & \textbf{72.3}& \,\textcolor{gray}{±0.2} \\
\bottomrule
\end{tabular}
\caption{Symmetric Relevance Gain (SRG) AOPC evaluated using predicted labels across multiple models.}
\label{across_models_sel1_SRG_1p_AOPC_m_2}
\end{table}


==> files/tables_v1/across_models/sel1/SRG_1p_accuracy/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}l}
\toprule
Method & \multicolumn{2}{c}{ViT-L} & \multicolumn{2}{c}{EVA2-S} & \multicolumn{2}{c}{BEiT2-L} & \multicolumn{2}{c}{FlexiViT-L} & \multicolumn{2}{c}{SigLIP-L} & \multicolumn{2}{c}{CLIP-H} & \multicolumn{2}{c}{DeiT3-H} & \multicolumn{2}{c}{\textit{Avg.}} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-15}
\cmidrule(l){16-17}
Random & 49.8& \,\textcolor{gray}{±0.1} & 50.1& \,\textcolor{gray}{±0.1} & 50.0& \,\textcolor{gray}{±0.1} & 49.9& \,\textcolor{gray}{±0.1} & 50.0& \,\textcolor{gray}{±0.1} & 50.2& \,\textcolor{gray}{±0.1} & 49.8& \,\textcolor{gray}{±0.1} & 50.0& \,\textcolor{gray}{±0.1} \\
RawAtt & 53.3& \,\textcolor{gray}{±0.1} & 66.8& \,\textcolor{gray}{±0.1} & 56.6& \,\textcolor{gray}{±0.1} & 62.1& \,\textcolor{gray}{±0.1} & -& & 59.2& \,\textcolor{gray}{±0.1} & 65.2& \,\textcolor{gray}{±0.1} & 60.6& \,\textcolor{gray}{±0.1} \\
Attention Rollout & 49.9& \,\textcolor{gray}{±0.1} & 59.9& \,\textcolor{gray}{±0.1} & 47.7& \,\textcolor{gray}{±0.1} & 48.0& \,\textcolor{gray}{±0.1} & -& & 58.0& \,\textcolor{gray}{±0.1} & 47.8& \,\textcolor{gray}{±0.1} & 51.9& \,\textcolor{gray}{±0.1} \\
AliLRP & 52.8& \,\textcolor{gray}{±0.1} & 67.6& \,\textcolor{gray}{±0.1} & 55.3& \,\textcolor{gray}{±0.1} & 54.8& \,\textcolor{gray}{±0.1} & 66.2& \,\textcolor{gray}{±0.1} & 54.8& \,\textcolor{gray}{±0.1} & 71.2& \,\textcolor{gray}{±0.1} & 60.4& \,\textcolor{gray}{±0.1} \\
AttnLRP & 59.7& \,\textcolor{gray}{±0.1} & 75.5& \,\textcolor{gray}{±0.1} & 61.7& \,\textcolor{gray}{±0.1} & 49.9& \,\textcolor{gray}{±0.1} & 72.2& \,\textcolor{gray}{±0.1} & 65.0& \,\textcolor{gray}{±0.1} & 60.8& \,\textcolor{gray}{±0.1} & 63.5& \,\textcolor{gray}{±0.1} \\
DecompX & 57.4& \,\textcolor{gray}{±0.1} & 66.3& \,\textcolor{gray}{±0.1} & 58.3& \,\textcolor{gray}{±0.1} & 60.9& \,\textcolor{gray}{±0.1} & 64.6& \,\textcolor{gray}{±0.1} & 62.1& \,\textcolor{gray}{±0.1} & 65.1& \,\textcolor{gray}{±0.1} & 62.1& \,\textcolor{gray}{±0.1} \\
Integrated Gradients & 54.7& \,\textcolor{gray}{±0.1} & 59.2& \,\textcolor{gray}{±0.1} & 53.7& \,\textcolor{gray}{±0.1} & 50.0& \,\textcolor{gray}{±0.1} & 59.8& \,\textcolor{gray}{±0.1} & 50.2& \,\textcolor{gray}{±0.1} & 53.9& \,\textcolor{gray}{±0.1} & 54.5& \,\textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 53.3& \,\textcolor{gray}{±0.1} & 58.2& \,\textcolor{gray}{±0.1} & 51.9& \,\textcolor{gray}{±0.1} & 49.1& \,\textcolor{gray}{±0.1} & 56.2& \,\textcolor{gray}{±0.1} & 50.1& \,\textcolor{gray}{±0.1} & 56.4& \,\textcolor{gray}{±0.1} & 53.6& \,\textcolor{gray}{±0.1} \\
\textbf{Libra \IxG{} } & 58.6& \,\textcolor{gray}{±0.1} & 76.2& \,\textcolor{gray}{±0.1} & 59.3& \,\textcolor{gray}{±0.1} & 61.6& \,\textcolor{gray}{±0.1} & 64.7& \,\textcolor{gray}{±0.1} & 62.6& \,\textcolor{gray}{±0.1} & 65.7& \,\textcolor{gray}{±0.1} & 64.1& \,\textcolor{gray}{±0.1} \\
\midrule
AttCAT & 61.2& \,\textcolor{gray}{±0.1} & 71.0& \,\textcolor{gray}{±0.1} & 60.7& \,\textcolor{gray}{±0.1} & 65.1& \,\textcolor{gray}{±0.1} & 61.2& \,\textcolor{gray}{±0.1} & 58.0& \,\textcolor{gray}{±0.1} & 62.3& \,\textcolor{gray}{±0.1} & 62.8& \,\textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \underline{71.8}& \,\textcolor{gray}{±0.1} & \underline{78.9}& \,\textcolor{gray}{±0.1} & \underline{67.9}& \,\textcolor{gray}{±0.1} & \underline{73.4}& \,\textcolor{gray}{±0.1} & \textbf{81.6}& \,\textcolor{gray}{±0.1} & \underline{71.2}& \,\textcolor{gray}{±0.1} & \underline{79.1}& \,\textcolor{gray}{±0.1} & \underline{74.9}& \,\textcolor{gray}{±0.1} \\
\midrule
GenAtt & 65.0& \,\textcolor{gray}{±0.1} & 60.7& \,\textcolor{gray}{±0.1} & 57.0& \,\textcolor{gray}{±0.1} & 70.0& \,\textcolor{gray}{±0.1} & -& & 65.9& \,\textcolor{gray}{±0.1} & 75.2& \,\textcolor{gray}{±0.1} & 65.6& \,\textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 67.1& \,\textcolor{gray}{±0.1} & 61.9& \,\textcolor{gray}{±0.1} & 58.1& \,\textcolor{gray}{±0.1} & 70.4& \,\textcolor{gray}{±0.1} & -& & 70.3& \,\textcolor{gray}{±0.1} & 76.2& \,\textcolor{gray}{±0.1} & 67.3& \,\textcolor{gray}{±0.1} \\
\midrule
TokenTM & 63.6& \,\textcolor{gray}{±0.1} & 63.4& \,\textcolor{gray}{±0.1} & 62.1& \,\textcolor{gray}{±0.1} & 67.6& \,\textcolor{gray}{±0.1} & -& & 66.2& \,\textcolor{gray}{±0.1} & 74.2& \,\textcolor{gray}{±0.1} & 66.2& \,\textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 65.2& \,\textcolor{gray}{±0.1} & 63.9& \,\textcolor{gray}{±0.1} & 61.0& \,\textcolor{gray}{±0.1} & 68.4& \,\textcolor{gray}{±0.1} & -& & 69.5& \,\textcolor{gray}{±0.1} & 75.3& \,\textcolor{gray}{±0.1} & 67.2& \,\textcolor{gray}{±0.1} \\
\midrule
GradCAM+ & 62.7& \,\textcolor{gray}{±0.1} & 65.0& \,\textcolor{gray}{±0.1} & 59.2& \,\textcolor{gray}{±0.1} & 50.5& \,\textcolor{gray}{±0.1} & 46.2& \,\textcolor{gray}{±0.1} & 51.2& \,\textcolor{gray}{±0.1} & 60.1& \,\textcolor{gray}{±0.1} & 56.4& \,\textcolor{gray}{±0.1} \\
\textbf{Libra GradCAM+} & 67.8& \,\textcolor{gray}{±0.1} & 76.7& \,\textcolor{gray}{±0.1} & 60.9& \,\textcolor{gray}{±0.1} & 57.2& \,\textcolor{gray}{±0.1} & 57.4& \,\textcolor{gray}{±0.1} & 53.5& \,\textcolor{gray}{±0.1} & 64.7& \,\textcolor{gray}{±0.1} & 62.6& \,\textcolor{gray}{±0.1} \\
\midrule
HiResCAM & 42.5& \,\textcolor{gray}{±0.1} & 72.6& \,\textcolor{gray}{±0.1} & 60.6& \,\textcolor{gray}{±0.1} & 51.2& \,\textcolor{gray}{±0.1} & 41.7& \,\textcolor{gray}{±0.1} & 57.8& \,\textcolor{gray}{±0.1} & 50.7& \,\textcolor{gray}{±0.1} & 53.9& \,\textcolor{gray}{±0.1} \\
\textbf{Libra HiResCAM} & 61.4& \,\textcolor{gray}{±0.1} & 74.5& \,\textcolor{gray}{±0.1} & 61.6& \,\textcolor{gray}{±0.1} & 71.9& \,\textcolor{gray}{±0.1} & 57.2& \,\textcolor{gray}{±0.1} & 64.9& \,\textcolor{gray}{±0.1} & 67.2& \,\textcolor{gray}{±0.1} & 65.5& \,\textcolor{gray}{±0.1} \\
\midrule
XGradCAM+ & 60.8& \,\textcolor{gray}{±0.1} & 67.0& \,\textcolor{gray}{±0.1} & 57.4& \,\textcolor{gray}{±0.1} & 49.4& \,\textcolor{gray}{±0.1} & 56.0& \,\textcolor{gray}{±0.1} & 57.4& \,\textcolor{gray}{±0.1} & 61.1& \,\textcolor{gray}{±0.1} & 58.5& \,\textcolor{gray}{±0.1} \\
\textbf{Libra XGradCAM+} & 69.4& \,\textcolor{gray}{±0.1} & 78.0& \,\textcolor{gray}{±0.1} & 65.6& \,\textcolor{gray}{±0.1} & 64.8& \,\textcolor{gray}{±0.1} & 70.0& \,\textcolor{gray}{±0.1} & 69.3& \,\textcolor{gray}{±0.1} & 76.3& \,\textcolor{gray}{±0.1} & 70.5& \,\textcolor{gray}{±0.1} \\
\midrule
FullGrad+ & 60.9& \,\textcolor{gray}{±0.1} & 67.4& \,\textcolor{gray}{±0.1} & 57.5& \,\textcolor{gray}{±0.1} & 63.3& \,\textcolor{gray}{±0.1} & 58.4& \,\textcolor{gray}{±0.1} & 56.9& \,\textcolor{gray}{±0.1} & 60.9& \,\textcolor{gray}{±0.1} & 60.8& \,\textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & \textbf{72.5}& \,\textcolor{gray}{±0.1} & \textbf{80.1}& \,\textcolor{gray}{±0.1} & \textbf{68.5}& \,\textcolor{gray}{±0.1} & \textbf{73.7}& \,\textcolor{gray}{±0.1} & \underline{79.6}& \,\textcolor{gray}{±0.1} & \textbf{73.0}& \,\textcolor{gray}{±0.1} & \textbf{79.6}& \,\textcolor{gray}{±0.1} & \textbf{75.3}& \,\textcolor{gray}{±0.1} \\
\bottomrule
\end{tabular}
\caption{Symmetric Relevance Gain (SRG) Accuracy evaluated using predicted labels across multiple models.}
\label{across_models_sel1_SRG_1p_accuracy_m_2}
\end{table}


==> files/tables_v1/across_models/sel1/SRG_gt_AOPC/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}l}
\toprule
Method & \multicolumn{2}{c}{ViT-L} & \multicolumn{2}{c}{EVA2-S} & \multicolumn{2}{c}{BEiT2-L} & \multicolumn{2}{c}{FlexiViT-L} & \multicolumn{2}{c}{SigLIP-L} & \multicolumn{2}{c}{CLIP-H} & \multicolumn{2}{c}{DeiT3-H} & \multicolumn{2}{c}{\textit{Avg.}} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-15}
\cmidrule(l){16-17}
Random & 49.7& \,\textcolor{gray}{±0.2} & 50.0& \,\textcolor{gray}{±0.2} & 49.8& \,\textcolor{gray}{±0.1} & 50.0& \,\textcolor{gray}{±0.2} & 50.0& \,\textcolor{gray}{±0.2} & 50.0& \,\textcolor{gray}{±0.2} & 50.0& \,\textcolor{gray}{±0.2} & 49.9& \,\textcolor{gray}{±0.2} \\
RawAtt & 53.1& \,\textcolor{gray}{±0.2} & 63.6& \,\textcolor{gray}{±0.2} & 55.6& \,\textcolor{gray}{±0.2} & 60.1& \,\textcolor{gray}{±0.2} & -& & 56.1& \,\textcolor{gray}{±0.2} & 59.8& \,\textcolor{gray}{±0.2} & 58.0& \,\textcolor{gray}{±0.2} \\
Attention Rollout & 50.3& \,\textcolor{gray}{±0.3} & 57.8& \,\textcolor{gray}{±0.3} & 48.1& \,\textcolor{gray}{±0.2} & 48.2& \,\textcolor{gray}{±0.2} & -& & 55.6& \,\textcolor{gray}{±0.3} & 48.4& \,\textcolor{gray}{±0.3} & 51.4& \,\textcolor{gray}{±0.2} \\
AliLRP & 52.4& \,\textcolor{gray}{±0.2} & 65.1& \,\textcolor{gray}{±0.3} & 54.6& \,\textcolor{gray}{±0.2} & 53.9& \,\textcolor{gray}{±0.1} & 63.9& \,\textcolor{gray}{±0.3} & 53.5& \,\textcolor{gray}{±0.2} & 67.4& \,\textcolor{gray}{±0.2} & 58.7& \,\textcolor{gray}{±0.2} \\
AttnLRP & 58.8& \,\textcolor{gray}{±0.3} & 71.3& \,\textcolor{gray}{±0.2} & 60.2& \,\textcolor{gray}{±0.2} & 49.4& \,\textcolor{gray}{±0.2} & 69.2& \,\textcolor{gray}{±0.3} & 60.6& \,\textcolor{gray}{±0.2} & 61.2& \,\textcolor{gray}{±0.3} & 61.5& \,\textcolor{gray}{±0.2} \\
DecompX & 56.8& \,\textcolor{gray}{±0.3} & 63.7& \,\textcolor{gray}{±0.3} & 57.3& \,\textcolor{gray}{±0.2} & 59.3& \,\textcolor{gray}{±0.2} & 62.2& \,\textcolor{gray}{±0.2} & 58.3& \,\textcolor{gray}{±0.2} & 63.7& \,\textcolor{gray}{±0.2} & 60.2& \,\textcolor{gray}{±0.2} \\
Integrated Gradients & 58.2& \,\textcolor{gray}{±0.3} & 63.1& \,\textcolor{gray}{±0.2} & 55.7& \,\textcolor{gray}{±0.2} & 51.1& \,\textcolor{gray}{±0.2} & 63.5& \,\textcolor{gray}{±0.3} & 50.3& \,\textcolor{gray}{±0.2} & 58.1& \,\textcolor{gray}{±0.3} & 57.1& \,\textcolor{gray}{±0.2} \\
\midrule
\IxG{}  & 53.0& \,\textcolor{gray}{±0.2} & 57.1& \,\textcolor{gray}{±0.2} & 51.7& \,\textcolor{gray}{±0.1} & 49.0& \,\textcolor{gray}{±0.2} & 56.4& \,\textcolor{gray}{±0.3} & 50.1& \,\textcolor{gray}{±0.2} & 56.2& \,\textcolor{gray}{±0.2} & 53.3& \,\textcolor{gray}{±0.2} \\
\textbf{Libra \IxG{} } & 57.7& \,\textcolor{gray}{±0.3} & 72.2& \,\textcolor{gray}{±0.3} & 58.1& \,\textcolor{gray}{±0.2} & 60.1& \,\textcolor{gray}{±0.2} & 62.2& \,\textcolor{gray}{±0.3} & 59.0& \,\textcolor{gray}{±0.2} & 64.1& \,\textcolor{gray}{±0.2} & 61.9& \,\textcolor{gray}{±0.2} \\
\midrule
AttCAT & 60.0& \,\textcolor{gray}{±0.2} & 69.0& \,\textcolor{gray}{±0.2} & 60.0& \,\textcolor{gray}{±0.2} & 62.5& \,\textcolor{gray}{±0.3} & 61.4& \,\textcolor{gray}{±0.3} & 57.5& \,\textcolor{gray}{±0.2} & 61.1& \,\textcolor{gray}{±0.3} & 61.6& \,\textcolor{gray}{±0.2} \\
\textbf{Libra AttCAT} & \underline{69.5}& \,\textcolor{gray}{±0.3} & \underline{74.4}& \,\textcolor{gray}{±0.2} & \underline{65.4}& \,\textcolor{gray}{±0.2} & \underline{70.0}& \,\textcolor{gray}{±0.2} & \textbf{77.3}& \,\textcolor{gray}{±0.3} & \underline{64.9}& \,\textcolor{gray}{±0.2} & \underline{73.8}& \,\textcolor{gray}{±0.2} & \underline{70.8}& \,\textcolor{gray}{±0.2} \\
\midrule
GenAtt & 63.0& \,\textcolor{gray}{±0.2} & 58.2& \,\textcolor{gray}{±0.2} & 56.1& \,\textcolor{gray}{±0.2} & 66.1& \,\textcolor{gray}{±0.2} & -& & 61.1& \,\textcolor{gray}{±0.2} & 69.1& \,\textcolor{gray}{±0.2} & 62.3& \,\textcolor{gray}{±0.2} \\
\textbf{Libra GenAtt} & 64.7& \,\textcolor{gray}{±0.3} & 59.2& \,\textcolor{gray}{±0.2} & 56.8& \,\textcolor{gray}{±0.2} & 66.7& \,\textcolor{gray}{±0.2} & -& & 63.5& \,\textcolor{gray}{±0.2} & 70.2& \,\textcolor{gray}{±0.2} & 63.5& \,\textcolor{gray}{±0.2} \\
\midrule
TokenTM & 61.7& \,\textcolor{gray}{±0.3} & 60.9& \,\textcolor{gray}{±0.2} & 60.3& \,\textcolor{gray}{±0.2} & 64.4& \,\textcolor{gray}{±0.2} & -& & 60.9& \,\textcolor{gray}{±0.2} & 68.4& \,\textcolor{gray}{±0.2} & 62.8& \,\textcolor{gray}{±0.2} \\
\textbf{Libra TokenTM} & 63.1& \,\textcolor{gray}{±0.3} & 61.0& \,\textcolor{gray}{±0.3} & 59.3& \,\textcolor{gray}{±0.3} & 65.3& \,\textcolor{gray}{±0.2} & -& & 62.9& \,\textcolor{gray}{±0.2} & 69.3& \,\textcolor{gray}{±0.2} & 63.5& \,\textcolor{gray}{±0.2} \\
\midrule
GradCAM+ & 61.5& \,\textcolor{gray}{±0.3} & 62.9& \,\textcolor{gray}{±0.3} & 58.3& \,\textcolor{gray}{±0.2} & 49.2& \,\textcolor{gray}{±0.2} & 44.9& \,\textcolor{gray}{±0.3} & 51.0& \,\textcolor{gray}{±0.2} & 57.5& \,\textcolor{gray}{±0.2} & 55.0& \,\textcolor{gray}{±0.2} \\
\textbf{Libra GradCAM+} & 65.5& \,\textcolor{gray}{±0.3} & 72.0& \,\textcolor{gray}{±0.2} & 59.6& \,\textcolor{gray}{±0.2} & 55.6& \,\textcolor{gray}{±0.2} & 55.9& \,\textcolor{gray}{±0.3} & 52.6& \,\textcolor{gray}{±0.2} & 61.6& \,\textcolor{gray}{±0.2} & 60.4& \,\textcolor{gray}{±0.2} \\
\midrule
HiResCAM & 43.6& \,\textcolor{gray}{±0.2} & 69.6& \,\textcolor{gray}{±0.2} & 59.2& \,\textcolor{gray}{±0.2} & 49.9& \,\textcolor{gray}{±0.2} & 42.5& \,\textcolor{gray}{±0.3} & 55.9& \,\textcolor{gray}{±0.2} & 50.6& \,\textcolor{gray}{±0.2} & 53.1& \,\textcolor{gray}{±0.2} \\
\textbf{Libra HiResCAM} & 60.1& \,\textcolor{gray}{±0.2} & 70.5& \,\textcolor{gray}{±0.2} & 59.8& \,\textcolor{gray}{±0.2} & 68.8& \,\textcolor{gray}{±0.3} & 56.1& \,\textcolor{gray}{±0.3} & 60.5& \,\textcolor{gray}{±0.2} & 62.6& \,\textcolor{gray}{±0.3} & 62.6& \,\textcolor{gray}{±0.2} \\
\midrule
XGradCAM+ & 59.9& \,\textcolor{gray}{±0.3} & 64.9& \,\textcolor{gray}{±0.3} & 56.9& \,\textcolor{gray}{±0.2} & 47.2& \,\textcolor{gray}{±0.3} & 56.4& \,\textcolor{gray}{±0.3} & 55.7& \,\textcolor{gray}{±0.2} & 58.9& \,\textcolor{gray}{±0.3} & 57.1& \,\textcolor{gray}{±0.3} \\
\textbf{Libra XGradCAM+} & 66.9& \,\textcolor{gray}{±0.3} & 72.9& \,\textcolor{gray}{±0.2} & 63.3& \,\textcolor{gray}{±0.2} & 62.3& \,\textcolor{gray}{±0.2} & 66.2& \,\textcolor{gray}{±0.3} & 63.4& \,\textcolor{gray}{±0.2} & 70.6& \,\textcolor{gray}{±0.2} & 66.5& \,\textcolor{gray}{±0.2} \\
\midrule
FullGrad+ & 59.8& \,\textcolor{gray}{±0.2} & 66.2& \,\textcolor{gray}{±0.3} & 56.9& \,\textcolor{gray}{±0.2} & 60.9& \,\textcolor{gray}{±0.3} & 59.0& \,\textcolor{gray}{±0.3} & 56.5& \,\textcolor{gray}{±0.2} & 59.5& \,\textcolor{gray}{±0.3} & 59.8& \,\textcolor{gray}{±0.2} \\
\textbf{Libra FullGrad+} & \textbf{70.0}& \,\textcolor{gray}{±0.3} & \textbf{75.4}& \,\textcolor{gray}{±0.3} & \textbf{65.8}& \,\textcolor{gray}{±0.2} & \textbf{70.1}& \,\textcolor{gray}{±0.2} & \underline{75.0}& \,\textcolor{gray}{±0.3} & \textbf{66.0}& \,\textcolor{gray}{±0.2} & \textbf{74.4}& \,\textcolor{gray}{±0.2} & \textbf{71.0}& \,\textcolor{gray}{±0.2} \\
\bottomrule
\end{tabular}
\caption{Symmetric Relevance Gain (SRG) AOPC evaluated using ground-truth labels across multiple models.}
\label{across_models_sel1_SRG_gt_AOPC_m_2}
\end{table}


==> files/tables_v1/across_models/sel1/SRG_gt_accuracy/m_2.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}l}
\toprule
Method & \multicolumn{2}{c}{ViT-L} & \multicolumn{2}{c}{EVA2-S} & \multicolumn{2}{c}{BEiT2-L} & \multicolumn{2}{c}{FlexiViT-L} & \multicolumn{2}{c}{SigLIP-L} & \multicolumn{2}{c}{CLIP-H} & \multicolumn{2}{c}{DeiT3-H} & \multicolumn{2}{c}{\textit{Avg.}} \\
\cmidrule(r){1-1}
\cmidrule(lr){2-15}
\cmidrule(l){16-17}
Random & 49.9& \,\textcolor{gray}{±0.1} & 50.0& \,\textcolor{gray}{±0.1} & 49.8& \,\textcolor{gray}{±0.1} & 49.8& \,\textcolor{gray}{±0.1} & 50.0& \,\textcolor{gray}{±0.1} & 50.0& \,\textcolor{gray}{±0.1} & 49.9& \,\textcolor{gray}{±0.1} & 49.9& \,\textcolor{gray}{±0.1} \\
RawAtt & 52.9& \,\textcolor{gray}{±0.1} & 64.3& \,\textcolor{gray}{±0.1} & 55.4& \,\textcolor{gray}{±0.1} & 60.1& \,\textcolor{gray}{±0.1} & -& & 57.8& \,\textcolor{gray}{±0.1} & 63.5& \,\textcolor{gray}{±0.1} & 59.0& \,\textcolor{gray}{±0.1} \\
Attention Rollout & 50.4& \,\textcolor{gray}{±0.1} & 58.5& \,\textcolor{gray}{±0.1} & 47.9& \,\textcolor{gray}{±0.1} & 48.3& \,\textcolor{gray}{±0.1} & -& & 57.2& \,\textcolor{gray}{±0.1} & 48.1& \,\textcolor{gray}{±0.1} & 51.8& \,\textcolor{gray}{±0.1} \\
AliLRP & 52.6& \,\textcolor{gray}{±0.1} & 66.2& \,\textcolor{gray}{±0.1} & 55.0& \,\textcolor{gray}{±0.1} & 54.1& \,\textcolor{gray}{±0.1} & 64.8& \,\textcolor{gray}{±0.1} & 54.5& \,\textcolor{gray}{±0.1} & 69.6& \,\textcolor{gray}{±0.1} & 59.5& \,\textcolor{gray}{±0.1} \\
AttnLRP & 58.7& \,\textcolor{gray}{±0.1} & 72.7& \,\textcolor{gray}{±0.1} & 60.3& \,\textcolor{gray}{±0.1} & 49.6& \,\textcolor{gray}{±0.1} & 69.8& \,\textcolor{gray}{±0.1} & 63.8& \,\textcolor{gray}{±0.1} & 59.7& \,\textcolor{gray}{±0.1} & 62.1& \,\textcolor{gray}{±0.1} \\
DecompX & 56.6& \,\textcolor{gray}{±0.1} & 64.0& \,\textcolor{gray}{±0.1} & 57.0& \,\textcolor{gray}{±0.1} & 59.3& \,\textcolor{gray}{±0.1} & 62.9& \,\textcolor{gray}{±0.1} & 60.8& \,\textcolor{gray}{±0.1} & 63.7& \,\textcolor{gray}{±0.1} & 60.6& \,\textcolor{gray}{±0.1} \\
Integrated Gradients & 58.7& \,\textcolor{gray}{±0.1} & 64.1& \,\textcolor{gray}{±0.1} & 55.6& \,\textcolor{gray}{±0.1} & 50.8& \,\textcolor{gray}{±0.1} & 64.3& \,\textcolor{gray}{±0.1} & 50.2& \,\textcolor{gray}{±0.1} & 57.6& \,\textcolor{gray}{±0.1} & 57.3& \,\textcolor{gray}{±0.1} \\
\midrule
\IxG{}  & 53.0& \,\textcolor{gray}{±0.1} & 57.2& \,\textcolor{gray}{±0.1} & 51.9& \,\textcolor{gray}{±0.1} & 49.0& \,\textcolor{gray}{±0.1} & 55.9& \,\textcolor{gray}{±0.1} & 50.1& \,\textcolor{gray}{±0.1} & 56.1& \,\textcolor{gray}{±0.1} & 53.3& \,\textcolor{gray}{±0.1} \\
\textbf{Libra \IxG{} } & 58.0& \,\textcolor{gray}{±0.1} & 74.5& \,\textcolor{gray}{±0.1} & 58.4& \,\textcolor{gray}{±0.1} & 60.4& \,\textcolor{gray}{±0.1} & 63.3& \,\textcolor{gray}{±0.1} & 61.7& \,\textcolor{gray}{±0.1} & 64.6& \,\textcolor{gray}{±0.1} & 63.0& \,\textcolor{gray}{±0.1} \\
\midrule
AttCAT & 60.2& \,\textcolor{gray}{±0.1} & 69.8& \,\textcolor{gray}{±0.1} & 60.1& \,\textcolor{gray}{±0.1} & 64.2& \,\textcolor{gray}{±0.1} & 61.0& \,\textcolor{gray}{±0.1} & 57.4& \,\textcolor{gray}{±0.1} & 61.8& \,\textcolor{gray}{±0.1} & 62.1& \,\textcolor{gray}{±0.1} \\
\textbf{Libra AttCAT} & \underline{70.5}& \,\textcolor{gray}{±0.1} & \underline{77.2}& \,\textcolor{gray}{±0.1} & \underline{66.6}& \,\textcolor{gray}{±0.1} & \underline{71.6}& \,\textcolor{gray}{±0.1} & \textbf{79.5}& \,\textcolor{gray}{±0.1} & \underline{69.8}& \,\textcolor{gray}{±0.1} & \underline{77.1}& \,\textcolor{gray}{±0.1} & \underline{73.2}& \,\textcolor{gray}{±0.1} \\
\midrule
GenAtt & 63.2& \,\textcolor{gray}{±0.1} & 59.1& \,\textcolor{gray}{±0.1} & 55.6& \,\textcolor{gray}{±0.1} & 67.3& \,\textcolor{gray}{±0.1} & -& & 63.9& \,\textcolor{gray}{±0.1} & 72.1& \,\textcolor{gray}{±0.1} & 63.5& \,\textcolor{gray}{±0.1} \\
\textbf{Libra GenAtt} & 65.3& \,\textcolor{gray}{±0.1} & 60.2& \,\textcolor{gray}{±0.1} & 56.6& \,\textcolor{gray}{±0.1} & 67.6& \,\textcolor{gray}{±0.1} & -& & 68.0& \,\textcolor{gray}{±0.1} & 73.2& \,\textcolor{gray}{±0.1} & 65.2& \,\textcolor{gray}{±0.1} \\
\midrule
TokenTM & 61.9& \,\textcolor{gray}{±0.1} & 61.8& \,\textcolor{gray}{±0.1} & 60.3& \,\textcolor{gray}{±0.1} & 65.2& \,\textcolor{gray}{±0.1} & -& & 64.3& \,\textcolor{gray}{±0.1} & 71.2& \,\textcolor{gray}{±0.1} & 64.1& \,\textcolor{gray}{±0.1} \\
\textbf{Libra TokenTM} & 63.4& \,\textcolor{gray}{±0.1} & 62.2& \,\textcolor{gray}{±0.1} & 59.4& \,\textcolor{gray}{±0.1} & 65.7& \,\textcolor{gray}{±0.1} & -& & 67.3& \,\textcolor{gray}{±0.1} & 72.3& \,\textcolor{gray}{±0.1} & 65.0& \,\textcolor{gray}{±0.1} \\
\midrule
GradCAM+ & 62.0& \,\textcolor{gray}{±0.1} & 64.0& \,\textcolor{gray}{±0.1} & 58.8& \,\textcolor{gray}{±0.1} & 50.2& \,\textcolor{gray}{±0.1} & 46.7& \,\textcolor{gray}{±0.1} & 51.2& \,\textcolor{gray}{±0.1} & 59.4& \,\textcolor{gray}{±0.1} & 56.0& \,\textcolor{gray}{±0.1} \\
\textbf{Libra GradCAM+} & 66.7& \,\textcolor{gray}{±0.1} & 75.0& \,\textcolor{gray}{±0.1} & 60.3& \,\textcolor{gray}{±0.1} & 56.6& \,\textcolor{gray}{±0.1} & 56.9& \,\textcolor{gray}{±0.1} & 53.7& \,\textcolor{gray}{±0.1} & 63.4& \,\textcolor{gray}{±0.1} & 61.8& \,\textcolor{gray}{±0.1} \\
\midrule
HiResCAM & 43.2& \,\textcolor{gray}{±0.1} & 71.2& \,\textcolor{gray}{±0.1} & 59.9& \,\textcolor{gray}{±0.1} & 50.6& \,\textcolor{gray}{±0.1} & 42.6& \,\textcolor{gray}{±0.1} & 57.3& \,\textcolor{gray}{±0.1} & 50.3& \,\textcolor{gray}{±0.1} & 53.6& \,\textcolor{gray}{±0.1} \\
\textbf{Libra HiResCAM} & 60.7& \,\textcolor{gray}{±0.1} & 72.6& \,\textcolor{gray}{±0.1} & 60.8& \,\textcolor{gray}{±0.1} & 70.4& \,\textcolor{gray}{±0.1} & 56.8& \,\textcolor{gray}{±0.1} & 63.8& \,\textcolor{gray}{±0.1} & 66.3& \,\textcolor{gray}{±0.1} & 64.5& \,\textcolor{gray}{±0.1} \\
\midrule
XGradCAM+ & 60.2& \,\textcolor{gray}{±0.1} & 66.0& \,\textcolor{gray}{±0.1} & 57.3& \,\textcolor{gray}{±0.1} & 49.2& \,\textcolor{gray}{±0.1} & 56.0& \,\textcolor{gray}{±0.1} & 56.9& \,\textcolor{gray}{±0.1} & 60.2& \,\textcolor{gray}{±0.1} & 58.0& \,\textcolor{gray}{±0.1} \\
\textbf{Libra XGradCAM+} & 68.2& \,\textcolor{gray}{±0.1} & 76.0& \,\textcolor{gray}{±0.1} & 64.5& \,\textcolor{gray}{±0.1} & 63.6& \,\textcolor{gray}{±0.1} & 68.4& \,\textcolor{gray}{±0.1} & 68.2& \,\textcolor{gray}{±0.1} & 74.2& \,\textcolor{gray}{±0.1} & 69.0& \,\textcolor{gray}{±0.1} \\
\midrule
FullGrad+ & 60.3& \,\textcolor{gray}{±0.1} & 66.5& \,\textcolor{gray}{±0.1} & 57.1& \,\textcolor{gray}{±0.1} & 62.2& \,\textcolor{gray}{±0.1} & 58.5& \,\textcolor{gray}{±0.1} & 56.4& \,\textcolor{gray}{±0.1} & 60.2& \,\textcolor{gray}{±0.1} & 60.2& \,\textcolor{gray}{±0.1} \\
\textbf{Libra FullGrad+} & \textbf{71.2}& \,\textcolor{gray}{±0.1} & \textbf{78.3}& \,\textcolor{gray}{±0.1} & \textbf{67.1}& \,\textcolor{gray}{±0.1} & \textbf{71.9}& \,\textcolor{gray}{±0.1} & \underline{77.6}& \,\textcolor{gray}{±0.1} & \textbf{71.5}& \,\textcolor{gray}{±0.1} & \textbf{77.6}& \,\textcolor{gray}{±0.1} & \textbf{73.6}& \,\textcolor{gray}{±0.1} \\
\bottomrule
\end{tabular}
\caption{Symmetric Relevance Gain (SRG) Accuracy evaluated using ground-truth labels across multiple models.}
\label{across_models_sel1_SRG_gt_accuracy_m_2}
\end{table}

